QuadraNet: Improving High-Order Neural Interaction Efficiency with Hardware-Aware Quadratic Neural Networks

Recent progress in computer vision-oriented neural network designs is mostly driven by capturing high-order neural interactions among inputs and features. And there emerged a variety of approaches to accomplish this, such as Transformers and its variants. However, these interactions generate a large amount of intermediate state and/or strong data dependency, leading to considerable memory consumption and computing cost, and therefore compromising the overall runtime performance. To address this challenge, we rethink the high-order interactive neural network design with a quadratic computing approach. Specifically, we propose QuadraNet -- a comprehensive model design methodology from neuron reconstruction to structural block and eventually to the overall neural network implementation. Leveraging quadratic neurons' intrinsic high-order advantages and dedicated computation optimization schemes, QuadraNet could effectively achieve optimal cognition and computation performance. Incorporating state-of-the-art hardware-aware neural architecture search and system integration techniques, QuadraNet could also be well generalized in different hardware constraint settings and deployment scenarios. The experiment shows thatQuadraNet achieves up to 1.5$\times$ throughput, 30% less memory footprint, and similar cognition performance, compared with the state-of-the-art high-order approaches.

==> _hist/0-Abstract_v1-JX.tex <==
\begin{abstract}
It has been observed that recent progress in Computer Vision is mostly driven by {capturing} high-order spatial {interactions among inputs and features}. {There are, however, a variety of approaches to accomplish this with most of them suffering}
%\sout{it current high-order interactive neural networks suffer} 
from {high computation cost}
%\sout{bottlenecks} 
because of {the} large intermediate state space {and/}or strong data dependency. It's challenging to design efficient high-order interactive neural networks because it is hard to solve such problems and lacks hardware-optimized operators. To address this challenge, we propose a neural-level approach, namely \textit{QuadraNet}, using the quadratic neuron and an effective and efficient network design. \textit{QuadraNet} becomes hardware-friendly by optimizing the intermediate state space and eliminating recursive design, while it only uses a well-optimized operator\CX{\sout{library}}. To achieve maximum utilization proposed \textit{QuadraNet}'s hardware-friendliness, we also conduct Hardware-aware Neural Architecture Search to find out the best-suited network architecture for different hardware. The experiment shows that \textit{QuadraNet} achieves upto 1.5$\times$ throughput and 30\% less memory footprint compared with state-of-the-art high-order interactive model with similar performance.
\end{abstract}

==> _hist/0-Abstract_v2-XC.tex <==
\begin{abstract}
Recent progress in computer vision-oriented neural network designs is mostly driven by capturing high-order neural interactions among inputs and features.
	And there emerged a variety of approaches to accomplish this, such as Transformers and its variants.
%
However, these interactions generate a large amount of intermediate state and/or strong data dependency, leading to considerable memory consumption and computing cost, and therefore compromising the overall runtime performance.
%
To address this challenge, we rethink the high-order interactive neural network design with a quadratic computing approach.
	Specifically, we propose \textit{QuadraNet} --- a comprehensive model design methodology from neuron reconstruction to module design and eventually to the overall neural network implementation.
	Leveraging quadratic neuron's intrinsic high-order advantages and dedicated computation optimization schemes, \textit{QuadraNet} could effectively achieve optimal cognition and computation performance.
	Incorporating with state-of-the-art hardware-aware neural architecture search and system integration techniques, \textit{QuadraNet} could be also well generalized in different hardware constraint settings and deployment scenarios.
	The experiment shows that \textit{QuadraNet} achieves upto 1.5$\times$ throughput and 30\% less memory footprint compared with state-of-the-art high-order interactive model with similar performance.
\end{abstract}



==> _hist/1-Introduction_v1.tex <==
\section{Introduction}
Over the past decade, convolutional neural networks (CNN) have achieved great success in deep learning-based computer vision methods. The introduction of AlexNet \cite{NIPS2012_c399862d} attracts the attention of many researchers in the field of computer vision to the convolutional neural network. The ingenious design of convolutional operator introduces serviceable inductive bias: \emph{locality} and \emph{translation equivalence}. Locality is inspired by a biological finding that neurons in certain areas of the visual cortex are sensitive only to certain areas of the visual field \cite{hubel1962receptive}, which is important to delineating structures such as lines, edges, shapes and objects \cite{li2021localvit}. Translation equivalence ensures that the information of region of interest can be equally preserved in the information iterative transmission of a neural network. A large number of CNN-based models \cite{he2016deep,zhang2018residual,ren2015faster,xie2017aggregated} have then subsequently been proposed by the community and have been successful in a wide variety of computer vision tasks such as image classification, object detection, and semantic segmentation.

The emergence of Vision Transformer (ViT) \cite{dosovitskiy2020image} breaks the long-term monopoly of CNNs in computer vision. Vit and its variants \cite{liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit} have shown that with the powerful representation capacity of self-attention mechanism, they can achieve reasonable performance on image classification and other downstream tasks. But when it comes to the question of why Transformer-based models work, there is a contention of a hundred schools of thought. Some works \cite{dosovitskiy2020image,ding2022scaling} proposed that \emph{global receptive field} of self-attention helps catch the long-term spatial dependencies. Although this global receptive field considerably improve the representation capacity of neural networks, it results a tremendous number of parameters and FLOPs, and thus a requirement of large-scale training datasets. An intuitive solution is introducing locality or pyramid network structure to restrict the amount of parameters and computation \cite{liu2021swin,wang2021pyramid,chu2021twins}. Some other works \cite{liu2022convnet,tolstikhin2021mlp} focus on the \emph{macroscopical network architecture} of Vision Transformer, and substitute self-attention with convolution operations or multi layer perceptrons. Meanwhile, some works \cite{han2021connection,rao2022hornet} point out that the implicit \emph{input adaptive weights} of self-attention is one of the key component to build a powerful neural networks. Some works \cite{rao2022hornet,hu2018squeeze,chrysos2020p} take notice of \emph{high-order spatial interaction} exploited by self-attention mechanism , but the designed models in their works which achieve high-order spatial interaction suffer from low throughput due to complex network structures.

\begin{figure}[thbp]
\centerline{\includegraphics[width = 0.5\textwidth]{_fig/Problem_1.pdf}fig/2-order-noTanh.png}}
\caption{A perceptron with single quadratic neuron can solve Generalized XOR problem.}
\label{single perceptron}
\end{figure}

This derives a question: How to leverage convolution operator and self-attention's respective strengths to design a neural network? An intuitive way to combine the above-mentioned advantages of CNNs and Transformer-based models is to integrate convolution and self-attention \cite{dai2021coatnet,pan2022integration}. However, these approaches still suffer from tremendous amount of computation in self-attention mechanism. While there are potential high-order interaction among the spatial locations in a feature map, the existing dynamic \cite{chen2020dynamic} and high-order \cite{rao2022hornet,hu2018squeeze} convolutions' success suggests that high-order interaction does not necessarily accompanied with self-attention mechanism, instead, a choreographed network block architecture can also possess ability to capture high-order spatial interaction. Different from these hybrid models and architecture-base approaches, we aim at neuron-level implementation of high-order interaction among feature maps.

%In this work, we summarize that the success of previous vision backbone models lies in the \emph{locality}, \emph{translation equivalence}, \emph{long-term receptive field},\emph{multi-stage network architecture},\emph{input-adaptive weight}, and \emph{high-order interactions}. While previous 
Some previous works \cite{chrysos2020p,mantini2021cqnn,fan2018new} concentrate on quadratic or polynomial neural networks to discover the non-linearity in data. A quadratic neuron has a stronger ability of information self-reinforcement, while it can better find the correlation between various dimensions of data. Figure \ref{single perceptron} shows that a perceptron with a single quadratic neural can solve a generalized XOR problem, while data points farther from the decision boundary have greater activation, indicating that a quadratic neuron can generate nonlinear cross-dimensional feature self-reinforcement. Therefore, leveraging these characteristics, a shallower neural network can be designed with equivalent capacity to conventional deep neural networks. However, a quadratic neuron also bring a extra overhead compared with a conventional neuron. Consequently, inappropriate neural architecture design extremely hurts the sufficient utilization of intrinsic high-order interaction representation capacity and causes unnecessary overheads. We argue that an appropriate co-design of quadratic neuron and neural architecture can not only leverage the above-mentioned advantages of existing models but also the powerful information superposition ability.

In this paper, we propose the QuadraBlock that performs spatial-level high-order interaction using quadratic depth-width convolution and fully-connected layer.


==> _hist/1-Introduction_v2.tex <==
\section{Introduction}
During the past decade, the development of backbone neural networks in computer vision tasks have gone through two stages, the first stage is characterized by CNN-based models \cite{NIPS2012_c399862d,he2016deep,zhang2018residual}, while the second is featured by Transformer-based models \cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}.
%Over the past decade, convolutional neural networks (CNN) have achieved great success in learning-based computer vision tasks. 
%    The introduction of AlexNet \cite{NIPS2012_c399862d} attracts the attention of many researchers in the field of computer vision to CNNs. 
%    A large number of CNN-based models \cite{he2016deep,zhang2018residual,ren2015faster,xie2017aggregated} have then subsequently been proposed by the community and have been successful in a wide variety of computer vision tasks such as image classification, object detection, and semantic segmentation. 
%The emergence of Vision Transformer (ViT) \cite{dosovitskiy2020image} breaks the long-term monopoly of CNNs in computer vision. 
%    Vit and its variants \cite{liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit} have shown that with the powerful representation capacity of self-attention mechanism, they can achieve reasonable performance on image classification and other downstream tasks.
%    However, such high presentation ability comes at the cost of significant computing and memory overhead.
        The attention mechanism requires a lot of intermediate state parameters where exists a quadratic space complexity relation with the input. 
            The linear projection used to generate query, key and value leads to a huge computation complexity, and thus a huge amount of occupancy of computation and memory resources on GPU. 
            Also, in a vision task, the Q, K, and V's number of tokens will be $input\_size^2/patch\_size^2$. Consider a multi-head self attention (MHSA), the computation of $Softmax(QK^T/\sqrt{d_k})$ would take $2 \times input\_size^4 \times num\_heads \times 4Byte / patch\_size^4 $ memory. 
            The huge computational overhead of MHSA strongly impairs its feasibility of deployment on mobile devices.
    \cite{keles2022computational} shows that there is no better algorithm than the naive $O(n^2)$ approach for calculating softmax dot-product self-attention. 
        That means, in order to build a more concise neural networks of equal representation performance as ViT, we need give a carefully analysis of what makes a transformer-based model so powerful in vision tasks.
        
%\red{Maybe lack a summary sentence}
    Some works \cite{dosovitskiy2020image,ding2022scaling} proposed that \emph{global receptive field} of self-attention helps catch the long-term spatial dependencies. 
    Although this global receptive field considerably improve the representation capacity of neural networks, it results a tremendous number of parameters and FLOPs, and thus a requirement of large-scale training datasets. 
        An intuitive solution is introducing locality or pyramid network structure to restrict the amount of parameters and computation \cite{liu2021swin,wang2021pyramid,chu2021twins}. 
    Some other works \cite{liu2022convnet,tolstikhin2021mlp} focus on the \emph{macroscopical network architecture} of Vision Transformer, and substitute self-attention with convolution operations or multi layer perceptrons. 
    Meanwhile, some works \cite{han2021connection,rao2022hornet} point out that the implicit \emph{input adaptive weights} of self-attention is one of the key component to build a powerful neural networks. 
    Some works \cite{rao2022hornet,hu2018squeeze,chrysos2020p} take notice of \emph{high-order spatial interaction} exploited by self-attention mechanism , but the designed models in their works which achieve high-order spatial interaction still suffer from low throughput due to data hazards caused by the recursive design.
        While there are potential high-order interaction among the spatial locations in a feature map, the existing dynamic \cite{chen2020dynamic} and high-order \cite{rao2022hornet,hu2018squeeze} convolutions' success suggests that high-order interaction does not necessarily accompanied with self-attention mechanism, instead, a choreographed network block architecture can also possess ability to capture high-order spatial interaction. 
            Different from these hybrid models and architecture-base approaches, we aim at neuron-level implementation of high-order interaction among feature maps.
            
A quadratic neuron has a stronger ability of information self-reinforcement, while it can better find the correlation between various dimensions of data.
%Figure unfinished
    A perceptron with a single quadratic neural can solve a generalized XOR problem, which can only solved by a multi-layer perceptron with at least four conventional neurons, indicating that a quadratic neuron can generate nonlinear cross-dimensional feature self-reinforcement. 
        Therefore, leveraging these characteristics, a shallower neural network can be designed with equivalent capacity to conventional deep neural networks. 
    However, a quadratic neuron also bring a extra overhead compared with a conventional neuron. 
        Some previous works \cite{chrysos2020p,mantini2021cqnn,fan2018new} concentrate on quadratic or polynomial neural networks to discover the non-linearity in data.
            However, inappropriate neural architecture design extremely hurts the sufficient utilization of intrinsic high-order interaction representation capacity and causes unnecessary overheads.
        We argue that an appropriate co-design of quadratic neuron and neural architecture can not only leverage the above-mentioned advantages of existing models but also the powerful information superposition ability.
        
        
%Unfinished
%What we design? (QuadraBlock, Manually designed QuadraNet, hardware-aware NAS QuadraNet)
%Highlighted Experiment Result (accuracy, computation efficient, memory overhead)
%Main Contribution (1. deconstructing the success of self attention. 
%                   2. Rethinking the Format of Quadratic neuron
%                   3. Quadratic Neuron and Network Architecture Co-design
%                   4. Hardware-friendly compared with ViT)

==> _hist/1-Introduction_v3-XC.tex <==
\section{\textbf{Introduction}}
\begin{comment}
	% During the past decade, the designing philosophy of backbone neural networks in computer vision tasks have gone through two stages, the first stage is characterized by CNN-based models \cite{NIPS2012_c399862d,he2016deep,zhang2018residual}, while the second is featured by Transformer-based models \cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}.
\end{comment}

\FN{During the past decade, backbone neural networks for computer vision tasks have evolved from straightforward convolution-based information extraction~\cite{NIPS2012_c399862d,he2016deep,zhang2018residual} into Transformer-based interactive semantic representation that well leverages self-attention mechanisms for information superposition~\cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}.
	However, such an advanced mechanism brings huge costs as shown in  Fig.~\ref{fig:problem}.
	Specifically, interactive information iteration in self-attention requires more computation density than flattened convolution operations.
	Meanwhile, significant memory overheads are introduced due to intensive data transmission from sparse intermediate states.
	Therefore, even an extremely lightweight MobileViT model~\cite{mehta2021mobilevit} for edge devices still suffers a 10$\times$ latency compared with CNN-based MobileNetV2 \cite{sandler2018mobilenetv2}, and more than 60\% latency is caused by self-attention computing.}

\begin{comment}
	% As illustrated in Figure \ref{fig:problem}(a), due to the sparse intermediate state, self-attention cause a huge memory overhead.
	% For example, an extremely lightweight MobileViT  \cite{mehta2021mobilevit} for edge devices still suffer a 10$\times$ latency compared with CNN-based MobileNetV2 \cite{sandler2018mobilenetv2}.
\end{comment}

\begin{comment}
	% During the past decade, the designing philosophy of back- bone neural networks in computer vision tasks have gone from simple one-order information extraction (i.e. Convolution Neural Networks\cite{NIPS2012_c399862d,he2016deep,zhang2018residual}), to a complex high-order information superposition (i.e. Transformer-based models \cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}).
	% The reason why Transformer-based models performs well is powerful representation capacity of self-attention mechanism.
	% However, complex computation pattern of self-attention results in tremendous computing and memory overhead. As illustrated in Figure \ref{fig:problem}(a), due to the sparse intermediate state, self-attention cause a huge memory overhead.
	% For example, an extremely lightweight MobileViT  \cite{mehta2021mobilevit} for edge devices still suffer a 10$\times$ latency compared with CNN-based MobileNetV2 \cite{sandler2018mobilenetv2}.
	% Of such a long latency, more than 60\% is spent on self-attention.
	% The huge overhead of self-attention strongly impairs its feasibility of deployment on mobile devices.
\end{comment}

\begin{comment}
	%% In a vision task, the computation of $Softmax(QK^T)$ on an image with a resolution of 224 and patch size of 4 takes about 38MB memory.
	%% In consideration of the multi-heads, multi-layers structure, and linear projection used to generate Q,K and V, the overall computation and memory overhead will be enormous.
	%% The linear projection used to generate query, key and value leads to a huge computation complexity, and thus a huge amount of occupancy of computation resources.
\end{comment}


\FN{As the self-attention mechanism emerges as a new computing optimization bottleneck for Transformer-like neural networks, we need to carefully examine its in-depth mechanism:
%
From the algorithm perspective, self-attention operations are achieved by iterative point products across multiple feature dimensions (i.e., Q-K-V as shown in Fig.~\ref{fig:problem}).
	The nature of such a mechanism is \textit{high-order neural interactions} that generating an input-adaptive weight including information from input and multiplying this weight to the input itself.
	And~\cite{keles2022computational} also proves that such interactions might be the best approach for constructing an non-liner quadratic space for optimal cognition performance.}
%
\XC{From the computing perspective, given this algorithmic nature, there are some works emerging to achieve high-order neural interactions instead of existing self-attention operations, and therefore relieve the huge computational costs as mentioned above.}
	\CX{For example,~\cite{wang2020linformer} bypassed softmax operation to approximate self-attention as associative multiplication to avoid non-linear intermediate state space.~\cite{rao2022hornet} also devolve high-order production to gated recursive convolution for lower computation density.
	However, such approaches still suffer from certain problems.~\cite{wang2020linformer} with a strong assumptions can not be directly adapted to vision tasks, and it just provides a sub-optimal approximation to the self-attention.~\cite{rao2022hornet} introduces additional computational costs for its recursive design that extremely restricts the inference throughput.}

\begin{comment}
	% Unfortunately,~\cite{keles2022computational} shows that there is no better algorithm than the naive quadratic space-complexity approach for calculating softmax dot-product self-attention.
	% That means, in order to build a more hardware-friednly neural networks of equal representation performance as Vision Transformer (ViT), we need give a carefully analysis of what makes a transformer-based model so powerful in vision tasks.
	% Research efforts have been made to analyze the key factors of the success of ViT.
	%% Some works \cite{dosovitskiy2020image,ding2022scaling} proposed that \emph{global receptive field} of self-attention helps catch the long-term spatial dependencies.
	%% Although this global receptive field considerably improve the representation capacity of neural networks, it results a tremendous number of parameters and FLOPs, and thus a requirement of large-scale training datasets.
	%% An intuitive solution is introducing locality or pyramid network structure to restrict the amount of parameters and computation \cite{liu2021swin,wang2021pyramid,chu2021twins}.
\end{comment}
\begin{comment}
	Some works \cite{liu2022convnet,tolstikhin2021mlp} focus on the \emph{macroscopical network architecture} of Vision Transformer, and substitute self-attention with convolution operations or multi layer perceptrons.
	Meanwhile, some works \cite{han2021connection,rao2022hornet} point out that the implicit \emph{input adaptive weights} of self-attention is one of the key component to build a powerful neural networks.
	% But most importantly, the self-attention mechanism exploits \textbf{high-order neural interaction} among different dimension of data. The point product of Q, K and V is essentially a cross-dimensional high-order information superposition.
	%% \cite{rao2022hornet,hu2018squeeze,chrysos2020p} take notice of \emph{high-order spatial interaction} exploited by self-attention mechanism , but the designed models in their works which achieve high-order spatial interaction still suffer from low throughput due to data hazards caused by the recursive design.挪到related work讲
\end{comment}


\newpage
\begin{figure}[t]
	\centerline{\includegraphics[width=1.75in]{Problem}}
	\caption{Huge Costs of High-Order Neural Interaction in Self-Attention}
	% \caption{Huge memory overhead and latency caused by large intermediate state space and strong data dependencies, has become the main bottleneck of efficient high-order interactive neural networks. We come up with using quadratic neuron to realize efficient high-order interactive neural network}
    \label{fig:problem}
	\vspace{-3.2mm}
\end{figure}

\begin{comment}
	% While there are potential high-order interaction among the spatial locations in a feature map, the existing dynamic \cite{chen2020dynamic} and high-order \cite{rao2022hornet,hu2018squeeze} convolutions' success suggests that high-order interaction does not necessarily accompanied with self-attention mechanism, instead, a choreographed network block architecture can also possess ability to capture high-order spatial interaction.
	% Although there have been various works \cite{rao2022hornet,hu2018squeeze,chrysos2020p} take notice of high-order spatial interaction, the designed models in their works still suffer from low throughput due to data hazards caused by the recursive design.
    % In a word, the memory overhead and data dependency have been a significant bottleneck of the efficient high-order interaction computation.}
\end{comment}

\FN{Different from these state of arts that explored alternative model architectures to embody high-order neural interactions with certain drawbacks, we would dive into the neuron designs in this work, and fundamentally rethink Transformer-like neural network constructions.}
	\CX{Inspired by xxxxxx xxxx xxxxxx xxxx (we found that the high-order xxxx computation could be directly embedded into neuron designs).
	And such neuron implementations are usually referred to \textit{quadratic neurons}.}
	\FN{Quadratic neurons possess strong ability of information self-reinforcement across feature dimensions and relatively simple computation pattern, eliminating the data dependency and sparse intermediate states from conventional self-attention operations.
	Thus, quadratic neurons eventually serves as the key to fundamental Transformer-like model design revolution.}

\begin{comment}
	% Different from these architecture-based approaches, we aim at a neuron-level implementation of high-order interaction among dimensions, and thus eliminate data dependence and quadratic intermediate state space which result in a large latency and memory overhead.
	% Quadratic Neuron with strong ability of information self-reinforcement across dimensions and relatively simple computation pattern provides a good opportunity to attain this goal.
\end{comment}
\begin{comment}
	However, inappropriate neural architecture design extremely hurts the sufficient utilization of quadratic neuron's intrinsic high-order interaction representation capacity and causes unnecessary overheads.
   	This brings new opportunities and challenges to the co-design of efficient high-order interactive neural networks and quadratic neuron.
\end{comment}

\FN{Following such an approach, in this paper, we propose a novel quadratic neural network architecture --- \textit{QuadraNet}, which performs high-order neural interactions and adapts to different hardware computing constraints.
	From the inspiration of quadratic neuron designs to the comprehensive \textit{QuadraNet} architecture, we tackled a series of challenges, including:}
	

In this paper, we propose a novel hardware-friendly Quadratic interaction neural block with quadratic neuron, namely QuadraBlock.
    QuadraBlock achieves acceleration of high-order spatial interactive neural networks by leveraging hardware-optimized convolution and eliminating time consuming recursive computations.
    Based on QuadraBlock, we design a family of generic vision backbone networks named QuadraNet.
    For mobile devices implementation, we use the proposed QuadraBlock for hardware-aware neural architecture search (HW-NAS) that enables efficient deployment of high-order interactive neural networks.
    With the support of QuadraLib \cite{xu2022quadralib}, the memory overhead in the training stage of QuadraNet reduced also significantly compared with Transformer-based model.

The main contributions of this paper are as follows.
\begin{itemize}
\item We deconstruct the success of the Transformer-based vision model, and summarize high-order spatial interaction could be one of the key point of the self-attention. Then, we analyze the computational bottleneck of the high-order interactive neural networks in memory consumption and data dependency.
\item In neuron level, based on summarized key point, we propose a quadratic neural network approach, to leverage hardware-optimized operators and eliminate recursive computations.
\item In network level, we propose a quadratic neuron and network co-design, namely QuadraBlock, to minimize the overhead of quadratic neurons while achieve a powerful presentation ability. Using QuadraBlock, we propose QuadraNet with comparable accuracy to existing state-of-the-art Transformer-based models while achieve a higher throughput.
\item In system level, incorporating HW-NAS, we obtain customized quadratic neural networks on different computing platforms with low latency and high accuracy.
\end{itemize}

Experiment shows that the proposed QuadraNet get a good balance in the trade-off between Convolution's efficiency and Self-attention's representation capacity. QuadraNet can provide 1.5$\times$ throughput without any accuracy reduction.
%NAS experiment result
%Intro部分缺一幅图！放1.neuron->block->{Manul Design and NAS}的整个framework 2.accuracy/throughput的折线图


==> _hist/1-Introduction_v3.tex <==
\section{\textbf{Introduction}}
%During the past decade, the designing philosophy of backbone neural networks in computer vision tasks have gone through two stages, the first stage is characterized by CNN-based models \cite{NIPS2012_c399862d,he2016deep,zhang2018residual}, while the second is featured by Transformer-based models \cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}.
During the past decade, the designing philosophy of backbone neural networks in computer vision tasks have gone from simple one-order information extraction (i.e. Convolution Neural Networks\cite{NIPS2012_c399862d,he2016deep,zhang2018residual}), to a complex high-order information superposition (i.e. Transformer-based models \cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}).
    The reason why Transformer-based models performs well is powerful representation capacity of self-attention mechanism. 
        However, complex computation pattern of self-attention results in tremendous computing and memory overhead. As illustrated in Figure \ref{fig:problem}(a), due to the sparse intermediate state, self-attention cause a huge memory overhead.
            For example, an extremely lightweight MobileViT  \cite{mehta2021mobilevit} for edge devices still suffer a 10$\times$ latency compared with CNN-based MobileNetV2 \cite{sandler2018mobilenetv2}.
                Of such a long latency, more than 60\% is spent on self-attention.
%            In a vision task, the computation of $Softmax(QK^T)$ on an image with a resolution of 224 and patch size of 4 takes about 38MB memory.
%           In consideration of the multi-heads, multi-layers structure, and linear projection used to generate Q,K and V, the overall computation and memory overhead will be enormous.
%        The linear projection used to generate query, key and value leads to a huge computation complexity, and thus a huge amount of occupancy of computation resources.
            The huge overhead of self-attention strongly impairs its feasibility of deployment on mobile devices.
    
\begin{figure}
    \centerline{\includegraphics[width = 3 in]{Problem}}
    \caption{Huge memory overhead and latency caused by large intermediate state space and strong data dependencies, has become the main bottleneck of efficient high-order interactive neural networks. We come up with using quadratic neuron to realize efficient high-order interactive neural network}
    \label{fig:problem}
\end{figure}

Unfortunately, \cite{keles2022computational} shows that there is no better algorithm than the naive quadratic space-complexity approach for calculating softmax dot-product self-attention. 
    That means, in order to build a more hardware-friednly neural networks of equal representation performance as Vision Transformer (ViT), we need give a carefully analysis of what makes a transformer-based model so powerful in vision tasks.
%\red{Maybe lack a summary sentence}
Research efforts have been made to analyze the key factors of the success of ViT.
%    Some works \cite{dosovitskiy2020image,ding2022scaling} proposed that \emph{global receptive field} of self-attention helps catch the long-term spatial dependencies. 
%    Although this global receptive field considerably improve the representation capacity of neural networks, it results a tremendous number of parameters and FLOPs, and thus a requirement of large-scale training datasets. 
%        An intuitive solution is introducing locality or pyramid network structure to restrict the amount of parameters and computation \cite{liu2021swin,wang2021pyramid,chu2021twins}. 
    Some works \cite{liu2022convnet,tolstikhin2021mlp} focus on the \emph{macroscopical network architecture} of Vision Transformer, and substitute self-attention with convolution operations or multi layer perceptrons. 
    Meanwhile, some works \cite{han2021connection,rao2022hornet} point out that the implicit \emph{input adaptive weights} of self-attention is one of the key component to build a powerful neural networks. 
    But most importantly, the self-attention mechanism exploits \textbf{high-order neural interaction} among different dimension of data. The point product of Q, K and V is essentially a cross-dimensional high-order information superposition. %\cite{rao2022hornet,hu2018squeeze,chrysos2020p} take notice of \emph{high-order spatial interaction} exploited by self-attention mechanism , but the designed models in their works which achieve high-order spatial interaction still suffer from low throughput due to data hazards caused by the recursive design.挪到related work讲
        While there are potential high-order interaction among the spatial locations in a feature map, the existing dynamic \cite{chen2020dynamic} and high-order \cite{rao2022hornet,hu2018squeeze} convolutions' success suggests that high-order interaction does not necessarily accompanied with self-attention mechanism, instead, a choreographed network block architecture can also possess ability to capture high-order spatial interaction. 

Although there have been various works \cite{rao2022hornet,hu2018squeeze,chrysos2020p} take notice of high-order spatial interaction, the designed models in their works still suffer from low throughput due to data hazards caused by the recursive design. 
    In a word, the memory overhead and data dependency have been a significant bottleneck of the efficient high-order interaction computation. 
    Different from these architecture-based approaches, we aim at a neuron-level implementation of high-order interaction among dimensions, and thus eliminate data dependence and quadratic intermediate state space which result in a large latency and memory overhead.
        Quadratic Neuron with strong ability of information self-reinforcement across dimensions and relatively simple computation pattern provides a good opportunity to attain this goal.
    However, inappropriate neural architecture design extremely hurts the sufficient utilization of quadratic neuron's intrinsic high-order interaction representation capacity and causes unnecessary overheads.
    This brings new opportunities and challenges to the co-design of efficient high-order interactive neural networks and quadratic neuron.
    
In this paper, we propose a novel hardware-friendly Quadratic interaction neural block with quadratic neuron, namely QuadraBlock.
    QuadraBlock achieves acceleration of high-order spatial interactive neural networks by leveraging hardware-optimized convolution and eliminating time consuming recursive computations. 
    Based on QuadraBlock, we design a family of generic vision backbone networks named QuadraNet.
    For mobile devices implementation, we use the proposed QuadraBlock for hardware-aware neural architecture search (HW-NAS) that enables efficient deployment of high-order interactive neural networks.
    With the support of QuadraLib \cite{xu2022quadralib}, the memory overhead in the training stage of QuadraNet reduced also significantly compared with Transformer-based model.
    
The main contributions of this paper are as follows.
\begin{itemize}
\item We deconstruct the success of the Transformer-based vision model, and summarize high-order spatial interaction could be one of the key point of the self-attention. Then, we analyze the computational bottleneck of the high-order interactive neural networks in memory consumption and data dependency. 
\item In neuron level, based on summarized key point, we propose a quadratic neural network approach, to leverage hardware-optimized operators and eliminate recursive computations.
\item In network level, we propose a quadratic neuron and network co-design, namely QuadraBlock, to minimize the overhead of quadratic neurons while achieve a powerful presentation ability. Using QuadraBlock, we propose QuadraNet with comparable accuracy to existing state-of-the-art Transformer-based models while achieve a higher throughput.
\item In system level, incorporating HW-NAS, we obtain customized quadratic neural networks on different computing platforms with low latency and high accuracy.
\end{itemize}

Experiment shows that the proposed QuadraNet get a good balance in the trade-off between Convolution's efficiency and Self-attention's representation capacity. QuadraNet can provide 1.5$\times$ throughput without any accuracy reduction. 
%NAS experiment result
%Intro部分缺一幅图！放1.neuron->block->{Manul Design and NAS}的整个framework 2.accuracy/throughput的折线图


==> _hist/1-Introduction_v4-JX.tex <==
\section{\textbf{Introduction}}
\begin{comment}
	% During the past decade, the designing philosophy of backbone neural networks in computer vision tasks have gone through two stages, the first stage is characterized by CNN-based models \cite{NIPS2012_c399862d,he2016deep,zhang2018residual}, while the second is featured by Transformer-based models \cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}.
\end{comment}

\FN{During the past decade, backbone neural networks for computer vision tasks have evolved from straightforward convolution-based information extraction~\cite{NIPS2012_c399862d,he2016deep,zhang2018residual} into Transformer-based \JX{is ``Interactive semantic representation'' a term we coined in this paper or is this a term already being used by others?} interactive semantic representation that well leverages self-attention mechanisms for information superposition~\cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}.
	However, such an advanced mechanism brings huge costs as shown in  Fig.~\ref{fig:problem}.
	Specifically, \JX{another new term: ``interactive information iteration''?} interactive information iteration in self-attention requires more computation density \JX{needs to define: flops per byte or simply number of flops?} than flattened convolution operations.
	Meanwhile, significant memory overheads are introduced due to intensive data \JX{movement resulting}\sout{transmission} from \JX{large and} sparse intermediate states.
	Therefore, even an extremely lightweight MobileViT model~\cite{mehta2021mobilevit} for edge devices still suffers a 10$\times$ latency \JX{slow-down than} \sout{compared with} CNN-based MobileNetV2 \cite{sandler2018mobilenetv2}, \JX{among which} more than 60\% \JX{slowdown}\sout{latency} is caused by self-attention computing.}

\begin{comment}
	% As illustrated in Figure \ref{fig:problem}(a), due to the sparse intermediate state, self-attention cause a huge memory overhead.
	% For example, an extremely lightweight MobileViT  \cite{mehta2021mobilevit} for edge devices still suffer a 10$\times$ latency compared with CNN-based MobileNetV2 \cite{sandler2018mobilenetv2}.
\end{comment}

\begin{comment}
	% During the past decade, the designing philosophy of back- bone neural networks in computer vision tasks have gone from simple one-order information extraction (i.e. Convolution Neural Networks\cite{NIPS2012_c399862d,he2016deep,zhang2018residual}), to a complex high-order information superposition (i.e. Transformer-based models \cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}).
	% The reason why Transformer-based models performs well is powerful representation capacity of self-attention mechanism.
	% However, complex computation pattern of self-attention results in tremendous computing and memory overhead. As illustrated in Figure \ref{fig:problem}(a), due to the sparse intermediate state, self-attention cause a huge memory overhead.
	% For example, an extremely lightweight MobileViT  \cite{mehta2021mobilevit} for edge devices still suffer a 10$\times$ latency compared with CNN-based MobileNetV2 \cite{sandler2018mobilenetv2}.
	% Of such a long latency, more than 60\% is spent on self-attention.
	% The huge overhead of self-attention strongly impairs its feasibility of deployment on mobile devices.
\end{comment}

\begin{comment}
	%% In a vision task, the computation of $Softmax(QK^T)$ on an image with a resolution of 224 and patch size of 4 takes about 38MB memory.
	%% In consideration of the multi-heads, multi-layers structure, and linear projection used to generate Q,K and V, the overall computation and memory overhead will be enormous.
	%% The linear projection used to generate query, key and value leads to a huge computation complexity, and thus a huge amount of occupancy of computation resources.
\end{comment}


\FN{As the self-attention mechanism emerges as a new computing optimization bottleneck for Transformer-like neural networks, \JX{an open question is how to better understand its working mechanism and the impact of attention layer's depth.}\sout{we need to carefully examine its in-depth mechanism:}
%
From the algorithm perspective, self-attention operations are achieved by iterative point products across multiple feature dimensions (i.e., Q-K-V as shown in Fig.~\ref{fig:problem}).
	The nature of such a mechanism is \JX{the  effects of} \textit{high-order neural interactions} \JX{among inputs resulting from the multiplication of inputs and inputs-dependent weights.}\sout{that generating an input-adaptive weight including information from input and multiplying this weight to the input itself.}
	\JX{the following sentence is not clear to me. Maybe better like this: ``Such a high-order neural interaction may best be captured at the cost of quadratic time and space complexity~\cite{keles2022computational}, which further poses limits on its efficient implementation.''} \sout{And~\cite{keles2022computational} also proves that such interactions might be the best approach for constructing an non-liner quadratic space for optimal cognition performance.}}
%
\JX{From the computing perspective, to avoid the high computation cost of self-attention, some recent works propose other means to achieve a similar high-order neural interactions.}
\sout{
\XC{From the computing perspective, given this algorithmic nature, there are some works emerging to achieve high-order neural interactions instead of existing self-attention operations, and therefore relieve the huge computational costs as mentioned above.}}
\JX{need to define or explain ``non-linear intermediate state space''}
	\CX{For example,~\cite{wang2020linformer} bypassed softmax operation to approximate self-attention as associative multiplication to avoid non-linear intermediate state space.~\cite{rao2022hornet} also devolve high-order production to gated recursive convolution for lower computation density.
	However, such approaches still suffer from certain problems.~\cite{wang2020linformer} with a strong assumptions can not be directly adapted to vision tasks, and it just provides a sub-optimal approximation to the self-attention.~\cite{rao2022hornet} introduces additional computational costs for its recursive design that extremely restricts the inference throughput.}

\begin{comment}
	% Unfortunately,~\cite{keles2022computational} shows that there is no better algorithm than the naive quadratic space-complexity approach for calculating softmax dot-product self-attention.
	% That means, in order to build a more hardware-friednly neural networks of equal representation performance as Vision Transformer (ViT), we need give a carefully analysis of what makes a transformer-based model so powerful in vision tasks.
	% Research efforts have been made to analyze the key factors of the success of ViT.
	%% Some works \cite{dosovitskiy2020image,ding2022scaling} proposed that \emph{global receptive field} of self-attention helps catch the long-term spatial dependencies.
	%% Although this global receptive field considerably improve the representation capacity of neural networks, it results a tremendous number of parameters and FLOPs, and thus a requirement of large-scale training datasets.
	%% An intuitive solution is introducing locality or pyramid network structure to restrict the amount of parameters and computation \cite{liu2021swin,wang2021pyramid,chu2021twins}.
\end{comment}
\begin{comment}
	Some works \cite{liu2022convnet,tolstikhin2021mlp} focus on the \emph{macroscopical network architecture} of Vision Transformer, and substitute self-attention with convolution operations or multi layer perceptrons.
	Meanwhile, some works \cite{han2021connection,rao2022hornet} point out that the implicit \emph{input adaptive weights} of self-attention is one of the key component to build a powerful neural networks.
	% But most importantly, the self-attention mechanism exploits \textbf{high-order neural interaction} among different dimension of data. The point product of Q, K and V is essentially a cross-dimensional high-order information superposition.
	%% \cite{rao2022hornet,hu2018squeeze,chrysos2020p} take notice of \emph{high-order spatial interaction} exploited by self-attention mechanism , but the designed models in their works which achieve high-order spatial interaction still suffer from low throughput due to data hazards caused by the recursive design.挪到related work讲
\end{comment}


\newpage
\begin{figure}[t]
	\centerline{\includegraphics[width=1.75in]{Problem}}
	\caption{Huge Costs of High-Order Neural Interaction in Self-Attention}
	% \caption{Huge memory overhead and latency caused by large intermediate state space and strong data dependencies, has become the main bottleneck of efficient high-order interactive neural networks. We come up with using quadratic neuron to realize efficient high-order interactive neural network}
    \label{fig:problem}
	\vspace{-3.2mm}
\end{figure}

\begin{comment}
	% While there are potential high-order interaction among the spatial locations in a feature map, the existing dynamic \cite{chen2020dynamic} and high-order \cite{rao2022hornet,hu2018squeeze} convolutions' success suggests that high-order interaction does not necessarily accompanied with self-attention mechanism, instead, a choreographed network block architecture can also possess ability to capture high-order spatial interaction.
	% Although there have been various works \cite{rao2022hornet,hu2018squeeze,chrysos2020p} take notice of high-order spatial interaction, the designed models in their works still suffer from low throughput due to data hazards caused by the recursive design.
    % In a word, the memory overhead and data dependency have been a significant bottleneck of the efficient high-order interaction computation.}
\end{comment}

\FN{Different from these state of arts that explored alternative model architectures to embody high-order neural interactions with certain drawbacks, we would dive into the neuron designs in this work, and fundamentally rethink Transformer-like neural network constructions.}
	\CX{Inspired by~\cite{chrysos2020p} which builds neural networks by polynomials without activation function, we found that the high-order interactive computation could be directly embedded into neuron designs.
	And such neuron implementations are usually referred to \textit{quadratic neurons}.}
	\FN{Quadratic neurons possess strong ability of information self-reinforcement across feature dimensions and relatively simple computation pattern, eliminating the data dependency and \CX{non-linear intermediate states from conventional architecture-level approaches.}
%\XC{sparse intermediate states from conventional self-attention operations.}
	Thus, quadratic neurons eventually serves as the key to fundamental Transformer-like model design revolution.}

\begin{comment}
	% Different from these architecture-based approaches, we aim at a neuron-level implementation of high-order interaction among dimensions, and thus eliminate data dependence and quadratic intermediate state space which result in a large latency and memory overhead.
	% Quadratic Neuron with strong ability of information self-reinforcement across dimensions and relatively simple computation pattern provides a good opportunity to attain this goal.
\end{comment}
\begin{comment}
	However, inappropriate neural architecture design extremely hurts the sufficient utilization of quadratic neuron's intrinsic high-order interaction representation capacity and causes unnecessary overheads.
   	This brings new opportunities and challenges to the co-design of efficient high-order interactive neural networks and quadratic neuron.
\end{comment}

\FN{Following such an approach, in this paper, we propose a novel quadratic neural network architecture --- \textit{QuadraNet}, which performs high-order neural interactions and adapts to different hardware computing constraints. 
	From the inspiration of quadratic neuron designs to the comprehensive \textit{QuadraNet} architecture, we tackled a series of challenges, including}
	
	\CX{large memory consumption coupled with non-linear intermediate state space and data dependency caused by recursive design.} \JX{recursive design was not explained before?}
	

In this paper, we propose a novel hardware-friendly Quadratic interaction neural block with quadratic neuron, namely QuadraBlock.
    QuadraBlock achieves acceleration of high-order spatial interactive neural networks by leveraging hardware-optimized convolution and eliminating time consuming recursive computations.
    Based on QuadraBlock, we design a family of generic vision backbone networks named QuadraNet.
    For mobile devices implementation, we use the proposed QuadraBlock for hardware-aware neural architecture search (HW-NAS) that enables efficient deployment of high-order interactive neural networks.
    With the support of QuadraLib \cite{xu2022quadralib}, the memory overhead in the training stage of QuadraNet reduced also significantly compared with Transformer-based model.
    
\CX{
The main contributions of this paper are as follows.
\begin{itemize}

\item We demystify and deconstruct the success of the Transformer-based vision model through comprehensive algorithm and computation analysis. We point out that the nature of Transformer-based methods is higher-order computation and explore the bottleneck of existing high-order interactive approaches.
%and summarize high-order spatial interaction could be one of the key point of the self-attention. Then, we analyze the computational bottleneck of the high-order interactive neural networks in memory consumption and data dependency.
%\item In neuron level, based on summarized key point, we propose a quadratic neural network approach, to leverage hardware-optimized operators and eliminate recursive computations.
\item This is the first quadratic neural network that achieves competitive performance with state-of-the-art while keeping computational efficiency. We bridges the quadratic neurons to modern neural network design to form high-order neural interaction by exploiting their features separately.
\item We breakthrough the design methodology for neural network design from the architecture design level to neuron-architecture codesign level.
%\item In network level, we propose a quadratic neuron and network co-design, namely QuadraBlock, to minimize the overhead of quadratic neurons while achieve a powerful presentation ability. Using QuadraBlock, we propose QuadraNet with comparable accuracy to existing state-of-the-art Transformer-based models while achieve a higher throughput.
%\item In system level, incorporating HW-NAS, we obtain customized quadratic neural networks on different computing platforms with low latency and high accuracy.

\end{itemize}
}
Experiment shows that the proposed QuadraNet get a good balance in the trade-off between Convolution's efficiency and Self-attention's representation capacity. QuadraNet can provide 1.5$\times$ throughput without any accuracy reduction and 30\% memory optimization compared with Swin-Transformer~\cite{liu2021swin}. 
%QuadraBlock also enriches the search space of NAS, helps us finding suitable high-order neural architecture for different devices.
%NAS experiment result
%Intro部分缺一幅图！放1.neuron->block->{Manul Design and NAS}的整个framework 2.accuracy/throughput的折线图


==> _hist/1-Introduction_v5-CX-XC.tex <==
\section{\textbf{Introduction}}

\begin{comment}
	% During the past decade, the designing philosophy of backbone neural networks in computer vision tasks have gone through two stages, the first stage is characterized by CNN-based models \cite{NIPS2012_c399862d,he2016deep,zhang2018residual}, while the second is featured by Transformer-based models \cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}.
\end{comment}

During the past decade, backbone neural networks for computer vision tasks have evolved from convolution-based information extraction~\cite{NIPS2012_c399862d,he2016deep,zhang2018residual} into Transformer-based semantic representation that well leverages self-attention mechanisms for information superposition~\cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}.
	However, such an advanced mechanism brings huge computation costs.
	Specifically, self-attention generation involves complex neural information interactions as shown in Fig.~\ref{fig:problem}~(a), resulting in more computing resources consumption and memory overheads.
	% Meanwhile, significant memory overheads are introduced due to intensive data movement resulting from large and sparse intermediate states.
	Therefore, even with supreme cognition performance, an extremely lightweight MobileViT model~\cite{mehta2021mobilevit} for edge devices still suffers a 10$\times$ latency slow-down than a CNN-based MobileNetV2~\cite{sandler2018mobilenetv2}, among which more than 60\% slow-down is caused by self-attention generation.

\begin{comment}
	% As illustrated in Figure \ref{fig:problem}(a), due to the sparse intermediate state, self-attention cause a huge memory overhead.
	% For example, an extremely lightweight MobileViT  \cite{mehta2021mobilevit} for edge devices still suffer a 10$\times$ latency compared with CNN-based MobileNetV2 \cite{sandler2018mobilenetv2}.
\end{comment}
\begin{comment}
	% During the past decade, the designing philosophy of back- bone neural networks in computer vision tasks have gone from simple one-order information extraction (i.e. Convolution Neural Networks\cite{NIPS2012_c399862d,he2016deep,zhang2018residual}), to a complex high-order information superposition (i.e. Transformer-based models \cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}).
	% The reason why Transformer-based models performs well is powerful representation capacity of self-attention mechanism.
	% However, complex computation pattern of self-attention results in tremendous computing and memory overhead. As illustrated in Figure \ref{fig:problem}(a), due to the sparse intermediate state, self-attention cause a huge memory overhead.
	% For example, an extremely lightweight MobileViT  \cite{mehta2021mobilevit} for edge devices still suffer a 10$\times$ latency compared with CNN-based MobileNetV2 \cite{sandler2018mobilenetv2}.
	% Of such a long latency, more than 60\% is spent on self-attention.
	% The huge overhead of self-attention strongly impairs its feasibility of deployment on mobile devices.
\end{comment}
\begin{comment}
	%% In a vision task, the computation of $Softmax(QK^T)$ on an image with a resolution of 224 and patch size of 4 takes about 38MB memory.
	%% In consideration of the multi-heads, multi-layers structure, and linear projection used to generate Q,K and V, the overall computation and memory overhead will be enormous.
	%% The linear projection used to generate query, key and value leads to a huge computation complexity, and thus a huge amount of occupancy of computation resources.
\end{comment}



As self-attention generation emerges as a new computing bottleneck for Transformer-like neural networks, an open question is how to better understand its in-depth working mechanism:
%
From the algorithm perspective, self-attention generations are achieved by \textit{high-order neural interactions} of iterative point products across multiple feature transformation dimensions, generating input-adaptive weight sets.
	% From the algorithm perspective, self-attention generations are achieved by iterative point products across multiple feature dimensions (i.e., Q-K-V as shown in Fig.~\ref{fig:problem} (a)).
	% The nature of such a mechanism is the  effects of \textit{high-order neural interactions} among inputs resulting from the multiplication of inputs and inputs-dependent weights.~%\sout{that generating an input-adaptive weight including information from input and multiplying this weight to the input itself.}
	% \JX{the following sentence is not clear to me. Maybe better like this: ``Such a high-order neural interaction may best be captured at the cost of quadratic time and space complexity~\cite{keles2022computational}, which further poses limits on its efficient implementation.''}
	Although such high-order neural interactions may best be captured at the cost of quadratic time and space complexity~\cite{keles2022computational}, a huge number of sparse intermediate states are introduced as shown in Fig.~\ref{fig:problem}~(b).
	Compared to regular convolution operations of linear feature complexity to the input size, these intermediate states consume a quadratic feature space, thus, the aforementioned computation costs.
	% \CX{As shown if Fig.~\ref{fig:problem} (b), self-attention forms an intermediate state space that is quadratic with the number of input dimensions.}
	% which further poses limits on its efficient implementation.
	%\sout{And~\cite{keles2022computational} also proves that such interactions might be the best approach for constructing an non-liner quadratic space for optimal cognition performance.}}
%
From the computing perspective, to avoid the self-attention costs, some recent works proposed other means to achieve similar high-order neural interactions.
	%\sout{
	%\XC{From the computing perspective, given this algorithmic nature, there are some works emerging to achieve high-order neural interactions instead of existing self-attention operations, and therefore relieve the huge computational costs as mentioned above.}}
	%\JX{need to define or explain ``non-linear intermediate state space''}
%
For example,~\cite{wang2020linformer} bypassed softmax operations to approximate self-attention as associative multiplication to avoid the quadratic intermediate states.~\cite{rao2022hornet} also devolved high-order production to gated recursive convolution for lower computation complexity.
%
However, such approaches still suffer from certain problems: many of self-attention approximations fell into a sub-optimal feature space, compromising the cognition performance~\cite{wang2020linformer}; or some of them achieved comparable cognition performance but introduced more intricate data dependency, which limited not only the inference throughput but also the model design generalization~\cite{rao2022hornet}.
	% However, such approaches still suffer from certain problems.~\cite{wang2020linformer} with a strong assumptions can not be directly adapted to vision tasks, and it just provides a sub-optimal approximation to the self-attention.~\cite{rao2022hornet} introduces additional computational costs for its recursive design that extremely restricts the inference throughput.

\begin{comment}
	% Unfortunately,~\cite{keles2022computational} shows that there is no better algorithm than the naive quadratic space-complexity approach for calculating softmax dot-product self-attention.
	% That means, in order to build a more hardware-friednly neural networks of equal representation performance as Vision Transformer (ViT), we need give a carefully analysis of what makes a transformer-based model so powerful in vision tasks.
	% Research efforts have been made to analyze the key factors of the success of ViT.
	%% Some works \cite{dosovitskiy2020image,ding2022scaling} proposed that \emph{global receptive field} of self-attention helps catch the long-term spatial dependencies.
	%% Although this global receptive field considerably improve the representation capacity of neural networks, it results a tremendous number of parameters and FLOPs, and thus a requirement of large-scale training datasets.
	%% An intuitive solution is introducing locality or pyramid network structure to restrict the amount of parameters and computation \cite{liu2021swin,wang2021pyramid,chu2021twins}.
\end{comment}
\begin{comment}
	Some works \cite{liu2022convnet,tolstikhin2021mlp} focus on the \emph{macroscopical network architecture} of Vision Transformer, and substitute self-attention with convolution operations or multi layer perceptrons.
	Meanwhile, some works \cite{han2021connection,rao2022hornet} point out that the implicit \emph{input adaptive weights} of self-attention is one of the key component to build a powerful neural networks.
	% But most importantly, the self-attention mechanism exploits \textbf{high-order neural interaction} among different dimension of data. The point product of Q, K and V is essentially a cross-dimensional high-order information superposition.
	%% \cite{rao2022hornet,hu2018squeeze,chrysos2020p} take notice of \emph{high-order spatial interaction} exploited by self-attention mechanism , but the designed models in their works which achieve high-order spatial interaction still suffer from low throughput due to data hazards caused by the recursive design.挪到related work讲
\end{comment}



\begin{figure}[t]
	\centerline{\includegraphics[width=2.6in]{_fig/Problem_1}}
	\caption{High-Order Neural Interactions in Self-Attention Generations }
	% \caption{Huge memory overhead and latency caused by large intermediate state space and strong data dependencies, has become the main bottleneck of efficient high-order interactive neural networks. We come up with using quadratic neuron to realize efficient high-order interactive neural network}
	\label{fig:problem}
	\vspace{-3.45mm}
\end{figure}

\begin{comment}
	% While there are potential high-order interaction among the spatial locations in a feature map, the existing dynamic \cite{chen2020dynamic} and high-order \cite{rao2022hornet,hu2018squeeze} convolutions' success suggests that high-order interaction does not necessarily accompanied with self-attention mechanism, instead, a choreographed network block architecture can also possess ability to capture high-order spatial interaction.
	% Although there have been various works \cite{rao2022hornet,hu2018squeeze,chrysos2020p} take notice of high-order spatial interaction, the designed models in their works still suffer from low throughput due to data hazards caused by the recursive design.
	% In a word, the memory overhead and data dependency have been a significant bottleneck of the efficient high-order interaction computation.}
\end{comment}

Different from these state of the arts that explored alternative means for high-order neural interactions with certain drawbacks~\cite{rao2022hornet,wang2020linformer}, we would like to dive into fundamental neuron designs and thoroughly rethink Transformer-like neural network constructions, while retaining cognition, computation, and generalization performance, simultaneously.
	Inspired by~\cite{chrysos2020p}, which builds neural networks by polynomials without activation functions, we found that high-order neural interactions could be directly embedded into high-order neuron designs.
	And such neuron implementations could be achieved by \textit{quadratic neurons}~\cite{fan2018new,xu2022quadralib}.
	Quadratic neurons possess strong ability of information self-reinforcement across multiple feature dimensions, as well as relatively simple computation patterns, therefore eliminating intermediate states from conventional self-attention generations.
	%\XC{sparse intermediate states from conventional self-attention operations.}
	\textit{Thus, we take quadratic neurons as the key to the revolution of fundamental Transformer-like model designs.}

\begin{comment}
	% Different from these architecture-based approaches, we aim at a neuron-level implementation of high-order interaction among dimensions, and thus eliminate data dependence and quadratic intermediate state space which result in a large latency and memory overhead.
	% Quadratic Neuron with strong ability of information self-reinforcement across dimensions and relatively simple computation pattern provides a good opportunity to attain this goal.
\end{comment}
\begin{comment}
	However, inappropriate neural architecture design extremely hurts the sufficient utilization of quadratic neuron's intrinsic high-order interaction representation capacity and causes unnecessary overheads.
	This brings new opportunities and challenges to the co-design of efficient high-order interactive neural networks and quadratic neuron.
\end{comment}



Following such an approach, in this paper, we establish a novel quadratic neural network architecture --- \textit{QuadraNet}, which masters high-order neural interactions and adapts to different hardware computing constraints.
	From the inspiration of quadratic neuron to the comprehensive \textit{QuadraNet} architecture, we tackled a series of challenges, including,
	designing a more efficient quadratic neuron and leveraging emerging compiling techniques to accelerate quadratic convolution;
	building basic model structural blocks by incorporating quadratic convolution into modern network models;
	and granting hardware awareness to comprehensive high-order interactive quadratic neural networks through neural architecture search.
	% \CX{large memory consumption coupled with non-linear intermediate state space and data dependency caused by recursive design.} \JX{recursive design was not explained before?}

\begin{comment}
	% In this paper, we propose a novel hardware-friendly Quadratic interaction neural block with quadratic neuron, namely QuadraBlock.
	% QuadraBlock achieves acceleration of high-order spatial interactive neural networks by leveraging hardware-optimized convolution and eliminating time consuming recursive computations.
	% Based on QuadraBlock, we design a family of generic vision backbone networks named QuadraNet.
	% For mobile devices implementation, we use the proposed QuadraBlock for hardware-aware neural architecture search (HW-NAS) that enables efficient deployment of high-order interactive neural networks.
	% With the support of QuadraLib \cite{xu2022quadralib}, the memory overhead in the training stage of QuadraNet reduced also significantly compared with Transformer-based model.
\end{comment}



The main contributions of this paper are as follows.
\begin{itemize}
	\item We demystify the high-order neural interactions in Transformer-like neural networks through comprehensive algorithm and computation analysis, and explore the bottleneck of existing optimization approaches.
	\item We breakthrough conventional Transformer-like model designs with a full-stack revolution from quadratic neuron to structural blocks and eventually to comprehensive neural networks.
	\item We further generalize the proposed revolutionary quadratic design methodology into various neural network architectures and hardware computing constraints.
\end{itemize}


\begin{comment}
	% \item We demystify and deconstruct the success of the Transformer-based vision model through comprehensive algorithm and computation analysis. We point out that the nature of Transformer-based methods is high-order computation and explore the bottleneck of existing high-order interactive approaches.
	% \item This is the first quadratic neural network that achieves competitive performance with state-of-the-art while keeping computational efficiency.
	% \item We breakthrough the design methodology for neural network design from the architecture design level to neuron-architecture codesign level.
\end{comment}
\begin{comment}
	% and summarize high-order spatial interaction could be one of the key point of the self-attention. Then, we analyze the computational bottleneck of the high-order interactive neural networks in memory consumption and data dependency.
	% \item In neuron level, based on summarized key point, we propose a quadratic neural network approach, to leverage hardware-optimized operators and eliminate recursive computations.
	% \item In network level, we propose a quadratic neuron and network co-design, namely QuadraBlock, to minimize the overhead of quadratic neurons while achieve a powerful presentation ability.
		% Using QuadraBlock, we propose QuadraNet with comparable accuracy to existing state-of-the-art Transformer-based models while achieve a higher throughput.
	% \item In system level, incorporating HW-NAS, we obtain customized quadratic neural networks on different computing platforms with low latency and high accuracy.
\end{comment}


\newpage
To the best of our knowledge, \textit{QuadraNet} is the very first quadratic neural network design methodology that achieves competitive cognition performance with state-of-the-art Transformer-like models, while achieving outstanding computation efficiency.
	Specifically, experiment shows that the proposed \textit{QuadraNet} performs exceptional high-order neural interactions in terms of comparative self-attention representation capacity and classification accuracy.
	Meanwhile, \textit{QuadraNet} can provide 1.5$\times$ throughput without any accuracy reduction and 30\% memory occupation optimization compared with representative Transformer-like models~\cite{liu2021swin}.

==> _hist/1-Introduction_v5-CX.tex <==
\section{\textbf{Introduction}}
\begin{comment}
	% During the past decade, the designing philosophy of backbone neural networks in computer vision tasks have gone through two stages, the first stage is characterized by CNN-based models \cite{NIPS2012_c399862d,he2016deep,zhang2018residual}, while the second is featured by Transformer-based models \cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}.
\end{comment}

\FN{During the past decade, backbone neural networks for computer vision tasks have evolved from straightforward convolution-based information extraction~\cite{NIPS2012_c399862d,he2016deep,zhang2018residual} into Transformer-based 
%\JX{is ``Interactive semantic representation'' a term we coined in this paper or is this a term already being used by others?} 
\CX{complex} semantic representation that well leverages self-attention mechanisms for information superposition~\cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}.
	However, such an advanced mechanism brings huge computation costs.
	Specifically, %\JX{another new term: ``interactive information iteration''?} 
	\CX{complex information interaction} in self-attention requires more computing \CX{resources due to the increase of computation amount} %\JX{needs to define: flops per byte or simply number of flops?} 
	than flattened convolution operations.
	Meanwhile, significant memory overheads are introduced due to intensive data movement resulting from large and sparse intermediate states. \CX{As shown if Fig. \ref{fig:problem} (b), self-attention forms an intermediate state space that is quadratic with the number of input dimensions.}
	Therefore, even an extremely lightweight MobileViT model~\cite{mehta2021mobilevit} for edge devices still suffers a 10$\times$ latency slow-down than CNN-based MobileNetV2 \cite{sandler2018mobilenetv2}, among which more than 60\% slowdown is caused by self-attention computing.}

\begin{comment}
	% As illustrated in Figure \ref{fig:problem}(a), due to the sparse intermediate state, self-attention cause a huge memory overhead.
	% For example, an extremely lightweight MobileViT  \cite{mehta2021mobilevit} for edge devices still suffer a 10$\times$ latency compared with CNN-based MobileNetV2 \cite{sandler2018mobilenetv2}.
\end{comment}

\begin{comment}
	% During the past decade, the designing philosophy of back- bone neural networks in computer vision tasks have gone from simple one-order information extraction (i.e. Convolution Neural Networks\cite{NIPS2012_c399862d,he2016deep,zhang2018residual}), to a complex high-order information superposition (i.e. Transformer-based models \cite{dosovitskiy2020image,liu2021swin,wang2021pyramid,chu2021twins,touvron2021training,zhou2021deepvit}).
	% The reason why Transformer-based models performs well is powerful representation capacity of self-attention mechanism.
	% However, complex computation pattern of self-attention results in tremendous computing and memory overhead. As illustrated in Figure \ref{fig:problem}(a), due to the sparse intermediate state, self-attention cause a huge memory overhead.
	% For example, an extremely lightweight MobileViT  \cite{mehta2021mobilevit} for edge devices still suffer a 10$\times$ latency compared with CNN-based MobileNetV2 \cite{sandler2018mobilenetv2}.
	% Of such a long latency, more than 60\% is spent on self-attention.
	% The huge overhead of self-attention strongly impairs its feasibility of deployment on mobile devices.
\end{comment}

\begin{comment}
	%% In a vision task, the computation of $Softmax(QK^T)$ on an image with a resolution of 224 and patch size of 4 takes about 38MB memory.
	%% In consideration of the multi-heads, multi-layers structure, and linear projection used to generate Q,K and V, the overall computation and memory overhead will be enormous.
	%% The linear projection used to generate query, key and value leads to a huge computation complexity, and thus a huge amount of occupancy of computation resources.
\end{comment}


\FN{As the self-attention mechanism emerges as a new computing optimization bottleneck for Transformer-like neural networks, \JX{an open question is how to better understand its \CX{in-depth} working mechanism \sout{and the impact of attention layer's depth.}}\sout{we need to carefully examine its in-depth mechanism:}
%
From the algorithm perspective, self-attention operations are achieved by iterative point products across multiple feature dimensions (i.e., Q-K-V as shown in Fig.~\ref{fig:problem} (a)).
	The nature of such a mechanism is the  effects of \textit{high-order neural interactions} among inputs resulting from the multiplication of inputs and inputs-dependent weights.~%\sout{that generating an input-adaptive weight including information from input and multiplying this weight to the input itself.}
%	\JX{the following sentence is not clear to me. Maybe better like this: ``Such a high-order neural interaction may best be captured at the cost of quadratic time and space complexity~\cite{keles2022computational}, which further poses limits on its efficient implementation.''}
Such a high-order neural interaction may best be captured at the cost of quadratic time and space complexity~\cite{keles2022computational}, which further poses limits on its efficient implementation.
%\sout{And~\cite{keles2022computational} also proves that such interactions might be the best approach for constructing an non-liner quadratic space for optimal cognition performance.}}
%
From the computing perspective, to avoid the high computation cost of self-attention, some recent works propose other means to achieve a similar high-order neural interactions.
%\sout{
%\XC{From the computing perspective, given this algorithmic nature, there are some works emerging to achieve high-order neural interactions instead of existing self-attention operations, and therefore relieve the huge computational costs as mentioned above.}}
%\JX{need to define or explain ``non-linear intermediate state space''}
	\CX{For example,~\cite{wang2020linformer} bypassed softmax operation to approximate self-attention as associative multiplication to avoid \FN{quadratic} \sout{non-linear} intermediate state space.~\cite{rao2022hornet} also devolve high-order production to gated recursive convolution for lower computation density.
	However, such approaches still suffer from certain problems.~\cite{wang2020linformer} with a strong assumptions can not be directly adapted to vision tasks, and it just provides a sub-optimal approximation to the self-attention.~\cite{rao2022hornet} introduces additional computational costs for its recursive design that extremely restricts the inference throughput.}}

\begin{comment}
	% Unfortunately,~\cite{keles2022computational} shows that there is no better algorithm than the naive quadratic space-complexity approach for calculating softmax dot-product self-attention.
	% That means, in order to build a more hardware-friednly neural networks of equal representation performance as Vision Transformer (ViT), we need give a carefully analysis of what makes a transformer-based model so powerful in vision tasks.
	% Research efforts have been made to analyze the key factors of the success of ViT.
	%% Some works \cite{dosovitskiy2020image,ding2022scaling} proposed that \emph{global receptive field} of self-attention helps catch the long-term spatial dependencies.
	%% Although this global receptive field considerably improve the representation capacity of neural networks, it results a tremendous number of parameters and FLOPs, and thus a requirement of large-scale training datasets.
	%% An intuitive solution is introducing locality or pyramid network structure to restrict the amount of parameters and computation \cite{liu2021swin,wang2021pyramid,chu2021twins}.
\end{comment}
\begin{comment}
	Some works \cite{liu2022convnet,tolstikhin2021mlp} focus on the \emph{macroscopical network architecture} of Vision Transformer, and substitute self-attention with convolution operations or multi layer perceptrons.
	Meanwhile, some works \cite{han2021connection,rao2022hornet} point out that the implicit \emph{input adaptive weights} of self-attention is one of the key component to build a powerful neural networks.
	% But most importantly, the self-attention mechanism exploits \textbf{high-order neural interaction} among different dimension of data. The point product of Q, K and V is essentially a cross-dimensional high-order information superposition.
	%% \cite{rao2022hornet,hu2018squeeze,chrysos2020p} take notice of \emph{high-order spatial interaction} exploited by self-attention mechanism , but the designed models in their works which achieve high-order spatial interaction still suffer from low throughput due to data hazards caused by the recursive design.挪到related work讲
\end{comment}



\begin{figure}[t]
	\centerline{\includegraphics[width=3.3in]{_fig/Problem_1}}
	\caption{The Process of High-Order Neural Interaction in Self-Attention generates }
	% \caption{Huge memory overhead and latency caused by large intermediate state space and strong data dependencies, has become the main bottleneck of efficient high-order interactive neural networks. We come up with using quadratic neuron to realize efficient high-order interactive neural network}
    \label{fig:problem}
	\vspace{-3.2mm}
\end{figure}

\begin{comment}
	% While there are potential high-order interaction among the spatial locations in a feature map, the existing dynamic \cite{chen2020dynamic} and high-order \cite{rao2022hornet,hu2018squeeze} convolutions' success suggests that high-order interaction does not necessarily accompanied with self-attention mechanism, instead, a choreographed network block architecture can also possess ability to capture high-order spatial interaction.
	% Although there have been various works \cite{rao2022hornet,hu2018squeeze,chrysos2020p} take notice of high-order spatial interaction, the designed models in their works still suffer from low throughput due to data hazards caused by the recursive design.
    % In a word, the memory overhead and data dependency have been a significant bottleneck of the efficient high-order interaction computation.}
\end{comment}

\FN{Different from these state-of-the-arts \cite{rao2022hornet,wang2020linformer} that explored alternative model architectures to embody high-order neural interactions with certain drawbacks, we would dive into the neuron designs in this work, and fundamentally rethink Transformer-like neural network constructions.}
	\CX{Inspired by~\cite{chrysos2020p} which builds neural networks by polynomials without activation function, we found that the high-order interactive computation could be directly embedded into neuron designs.
	And such neuron implementations are usually referred to \textit{quadratic neurons}.}
	\FN{Quadratic neurons possess strong ability of information self-reinforcement across feature dimensions and relatively simple computation pattern, eliminating the data dependency and \CX{non-linear intermediate states from conventional architecture-level approaches.}
%\XC{sparse intermediate states from conventional self-attention operations.}
	Thus, quadratic neurons eventually serves as the key to fundamental Transformer-like model design revolution.}

\begin{comment}
	% Different from these architecture-based approaches, we aim at a neuron-level implementation of high-order interaction among dimensions, and thus eliminate data dependence and quadratic intermediate state space which result in a large latency and memory overhead.
	% Quadratic Neuron with strong ability of information self-reinforcement across dimensions and relatively simple computation pattern provides a good opportunity to attain this goal.
\end{comment}
\begin{comment}
	However, inappropriate neural architecture design extremely hurts the sufficient utilization of quadratic neuron's intrinsic high-order interaction representation capacity and causes unnecessary overheads.
   	This brings new opportunities and challenges to the co-design of efficient high-order interactive neural networks and quadratic neuron.
\end{comment}

\FN{Following such an approach, in this paper, we propose a novel quadratic neural network architecture --- \textit{QuadraNet}, which performs high-order neural interactions and adapts to different hardware computing constraints. 
	From the inspiration of quadratic neuron designs to the comprehensive \textit{QuadraNet} architecture, we tackled a series of challenges, including \CX{designing a more efficient quadratic neuron, leveraging existing optimized operators to accelerate quadratic convolution, building \FN{QuadraBlock} to concurrently take advantage of both modern CNNs and quadratic neurons, exploring hardware-aware high-order interactive neural networks through neural architecture search.}}

%	\CX{large memory consumption coupled with non-linear intermediate state space and data dependency caused by recursive design.} \JX{recursive design was not explained before?}
	
\begin{comment}
    

In this paper, we propose a novel hardware-friendly Quadratic interaction neural block with quadratic neuron, namely QuadraBlock.
    QuadraBlock achieves acceleration of high-order spatial interactive neural networks by leveraging hardware-optimized convolution and eliminating time consuming recursive computations.
    Based on QuadraBlock, we design a family of generic vision backbone networks named QuadraNet.
    For mobile devices implementation, we use the proposed QuadraBlock for hardware-aware neural architecture search (HW-NAS) that enables efficient deployment of high-order interactive neural networks.
    With the support of QuadraLib \cite{xu2022quadralib}, the memory overhead in the training stage of QuadraNet reduced also significantly compared with Transformer-based model.
\end{comment}

\CX{
The main contributions of this paper are as follows.
\begin{itemize}

\item We demystify and deconstruct the success of the Transformer-based vision model through comprehensive algorithm and computation analysis. We point out that the nature of Transformer-based methods is high-order computation and explore the bottleneck of existing high-order interactive approaches.
%and summarize high-order spatial interaction could be one of the key point of the self-attention. Then, we analyze the computational bottleneck of the high-order interactive neural networks in memory consumption and data dependency.
%\item In neuron level, based on summarized key point, we propose a quadratic neural network approach, to leverage hardware-optimized operators and eliminate recursive computations.
\item This is the first quadratic neural network that achieves competitive performance with state-of-the-art while keeping computational efficiency. We bridges the quadratic neurons to modern neural network design to form high-order neural interaction by exploiting their characteristics separately.
\item We breakthrough the design methodology for neural network design from the architecture design level to neuron-architecture codesign level.
%\item In network level, we propose a quadratic neuron and network co-design, namely QuadraBlock, to minimize the overhead of quadratic neurons while achieve a powerful presentation ability. Using QuadraBlock, we propose QuadraNet with comparable accuracy to existing state-of-the-art Transformer-based models while achieve a higher throughput.
%\item In system level, incorporating HW-NAS, we obtain customized quadratic neural networks on different computing platforms with low latency and high accuracy.

\end{itemize}
}
Experiment shows that the proposed QuadraNet get a good balance in the trade-off between Convolution's efficiency and Self-attention's representation capacity. QuadraNet can provide 1.5$\times$ throughput without any accuracy reduction and 30\% memory optimization compared with Swin-Transformer~\cite{liu2021swin}. 
%QuadraBlock also enriches the search space of NAS, helps us finding suitable high-order neural architecture for different devices.
%NAS experiment result
%Intro部分缺一幅图！放1.neuron->block->{Manul Design and NAS}的整个framework 2.accuracy/throughput的折线图


==> _hist/2-Background_v1.tex <==
\section{\textbf{Background and Motivation}}
\subsection{\textbf{High-Order Interactive Neural Networks}}
\subsubsection{\textbf{Higher-Order Interaction}}
As aforementioned, the computing mechanism of neural networks has evolved from low-density convolution into high-density attention-like mechanisms (e.g., spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self-attention \cite{dosovitskiy2020image}).
    These mechanisms could be formulated as follows:
\begin{equation}
    Attention(x) = f(g(x),x),
\end{equation}
where $x$ denotes input data and $g(x)$ generate an input-adaptive weight, and compute the final output with rule $f(\cdot,\cdot)$.

In such a formulation, usually, a high-order neural interaction can be observed as multiplication of data with itself or its transformation.
Such an interaction represents leveraging the superposition of information between different dimensions of the data itself.
    
\subsubsection{\textbf{Existing Approaches}}

%In the past decade, researchers found the effectiveness of attention mechanism. The attention mechanism uses the data itself to generate a set of parameters, and then multiply them with the data itself or their transformation. So no matter what kinds of attention (spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self attention \cite{dosovitskiy2020image}) used, it can be formulated in a high-order computation:
To capture the high-order spatial interaction, the latest star models, ViT \cite{dosovitskiy2020image} and its variants \cite{liu2021swin,chu2021twins}, import self-attention as the high-order interaction routine.
    In a vision task, self-attention's spatial mixing computation of the $c$-th channel at location $i$ can therefore be formulated as:
\begin{equation}
    x_{MHSA}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(x)_{ij}\omega_V^{(c',c)}x^{(j,c')},
\end{equation}
where $\Omega_i$ denotes the receptive field, $g(x)$ is calculated by a dot-product of transfomation of input $x$, and then forms an interaction with another transformation of the input itself.
        
Different from the self-attention approach, HorNet \cite{rao2022hornet} performs high-order spatial interaction with a recursive convolution design. 
    HorNet \cite{rao2022hornet} comes up with a g$^n$Conv operator to perform high-order interaction computation. The output of g$^n$Conv can be formulated as:
\begin{equation}
    x_{g^nConv}^{(i,c)} = p_n^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(p_{n-1})w_{n-1,i\rightarrow j}^c\omega_{\phi_{in}}^{c',c}x^{(j,c')}.
\end{equation}
Instead of generating high-order interaction by $g(x)$, g$^n$Conv uses a channel decreasing recursive formulation $g(p_{n-1})$ to perform high-order iteration of information.

\subsubsection{\textbf{Computation Challenges}}
The computation of existing high-order interaction approaches face multiple challenges in \textbf{memory consumption} or \textbf{data dependency}.
The computational process of self-attention generate a $O(n^2)$ intermediate state space.
    When mapping to hardware, ViT suffer from excessive memory consumption. 
        In the training stage, all the intermediate state tensors must be saved for the backpropagation. This leads to a lot of memory usage on the accelerators (i.e. GPU), which limits the depth of trainable networks on accelerators or the batch size during training.
        In the inference stage, inconsistency and interval of memory consumption in time flow limits the parallelizability of models and sufficient usage of the computation resources.

The g$^n$Conv makes use of a recursive design to achieve higher-order spatial interactions.
 Although its channel decreasing design limits the FLOPs to an acceptable range, the recursive design brings a strong data dependency.
    When mapping to hardware, there exists a decreasing utilization rate of computation units in the g$^n$Conv operator due to the mandatory synchronization caused by the data dependencies.
    
Such excessive memory consumption and data hazards brings new opportunities and challenges to design a novel efficient high-order interactive neural network. In this work, we will show that, to build a hardware-friendly high-order neural network, quadratic neuron can play an important role.

\subsection{\textbf{Quadratic Neuron}}

\subsubsection{\textbf{Design Motivation}}
To avoid huge memory consumption caused by a $O(n^2)$ intermediate state space and data dependency caused by high-order interactive neural network architecture design, we try to reduce the granularity of high-order computation from the level of network architectures to the level of neurons.

A quadratic neuron brings more opportunities to discover nonlinear relations among data dimensions. 
    Therefore, with a shallower network, a quadratic neural network can learn a smoother and richer nonlinear representation than conventional neural networks.
        Figure \ref{fig:perceptron} shows that for a generalized XOR classification problem, a single layer perceptron with a quadratic neuron can solve it alone, and gives even a more clear classification boundary than a two-layer perceptron with 10 hidden neurons. 

\subsubsection{\textbf{Neural Format}}
In contrast to the conventional neuron represented by a inner product of weight vector $W \in \mathbb{R}^{1 \times n}$ and input vector $\mathbf{x} \in \mathbb{R}^{n \times 1}$ plus a bias $b$ and an activation, the quadratic neuron can be written by an quadratic polynomial of input $\mathbf{x}$:
\begin{equation}
    y = \mathbf{x}^TW_q\mathbf{x} + W_c\mathbf{x} + b,
    \label{equ:quadratic_neuron}
\end{equation}
where $W_q \in \mathbf{R}^{n \times n}$ denotes a quadratic term weight and $W_c \in \mathbf{R}^{1 \times n}$ denotes a linear term weight. 
%Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, and thus it will rise the dimension interaction in data to a mandatory high-order format. 
%Since the high-order interaction among dimension is potential, rise it to a mandatory high-order format will miss the. 
    While the linear term promise a non-weaker learning ability than conventional CNNs, since the quadratic neuron includes a conventional neural network.
        Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, 
            and thus rise the potential high-order interaction to mandatory, causing a performance deduction.
            


\begin{figure}
    \centerline{\includegraphics[width = 3 in]{_fig/quadratic_perceptron_2.pdf}}
    \caption{A perceptron with single quadratic neuron can solve a generalized XOR problem.}
    \label{fig:perceptron}
\end{figure}


However, the conventional quadratic neuron also brings a quadratic parameter space ($w_q$), an inappropriate implementation of quadratic neural networks will therefore cause unnecessary overhead. The optimization of quadratic neural network's computation will thus be a challenge. In this work, co-design of quadratic neuron and computation block we proposed makes a balance in the trade-off between the accuracy and throughput.

\subsection{Hardware-aware Neural Architecture Search}
Neural Architecture Search (NAS) has been extensively used in the computer vision tasks during past few years. 
    Although NAS has achieved a huge success in finding high-performance neural networks, directly deploying NAS-synthesized complex neural architecture in resource-limited mobile devices is infeasible. 
    HW-NAS considers execution latency, memory footprint or energy footprint as one of the optimization objectives in the algorithms, and thus synthesizing a model well balanced between performance and hardware-specific computational consumption.

\textbf{Implementation Approach:}

Earlier on, few attention on NAS is given to high-order interactive networks because complex search space and large evaluation cost. 
    Recently, Some works \cite{gong2021nasvit,chen2021glit} tries to build a NAS synthesized ViT. However, they aims at a state-of-the-art neural architecture, which ignores the feasibility of the deployment on various devices. Consider the conciseness and hardware-friendliness of our QuadraNet, combining HW-NAS and QuadraNet to search a customized high-order interactive neural network architecture for specific computation platform will therefore be much intuitive.

    In this work, we don't look for particular innovation in NAS methodology but utilize it for investigating....
    

==> _hist/2-Background_v2.tex <==
\section{\textbf{Background and Motivation}}
\subsection{\textbf{High-Order Interactive Neural Networks}}
\textbf{Higher-Order Interaction:}
As aforementioned, the computing mechanism of neural networks has evolved from low-density convolution into high-density attention-like mechanisms.
(e.g., spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self-attention \cite{dosovitskiy2020image})
    These mechanisms could be formulated as follows:
\begin{equation}
    Attention(x) = f(g(x),x),
\end{equation}
where $x$ denotes input data and $g(x)$ generate an input-adaptive weight, and compute the final output with rule $f(\cdot,\cdot)$.


In such a formulation, usually, a high-order neural interaction can be observed as multiplication of data with itself or its transformation.
Such an interaction represents leveraging the superposition of information between different dimensions of the data itself.
    
\textbf{Existing Approaches:}
%In the past decade, researchers found the effectiveness of attention mechanism. The attention mechanism uses the data itself to generate a set of parameters, and then multiply them with the data itself or their transformation. So no matter what kinds of attention (spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self attention \cite{dosovitskiy2020image}) used, it can be formulated in a high-order computation:
To capture the high-order spatial interaction, the latest star models, ViT \cite{dosovitskiy2020image} and its variants \cite{liu2021swin,chu2021twins}, import self-attention as the high-order interaction routine.
    In a vision task, self-attention's spatial mixing computation of the $c$-th channel at location $i$ can therefore be formulated as:
\begin{equation}
    x_{MHSA}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(x)_{ij}W_V^{(c',c)}x^{(j,c')},
    \label{equ:self}
\end{equation}
where $\Omega_i$ denotes the receptive field, $g(x)$ is calculated by a dot-product of transfomation of input $x$, and then forms an interaction with another transformation of the input itself.
        
Different from the self-attention approach, HorNet \cite{rao2022hornet} performs high-order spatial interaction with a recursive convolution design. 
    HorNet \cite{rao2022hornet} comes up with a g$^n$Conv operator to perform high-order interaction computation. The output of g$^n$Conv can be formulated as:
\begin{equation}
    x_{g^nConv}^{(i,c)} = p_n^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(p_{n-1})w_{n-1,i\rightarrow j}^cW_{\phi_{in}}^{(c',c)}x^{(j,c')}.
    \label{equ:gnconv}
\end{equation}
Instead of generating high-order interaction by $g(x)$, g$^n$Conv uses a channel decreasing recursive formulation $g(p_{n-1})$ to perform high-order iteration of information.

\textbf{Computation Challenges:}
The computation of existing high-order interaction approaches face multiple challenges in \textbf{memory consumption} or \textbf{data dependency}.
The computational process of self-attention generate a $O(n^2)$ intermediate state space.
    When mapping to hardware, ViT suffer from excessive memory consumption. 
        In the training stage, all the intermediate state tensors must be saved for the backpropagation. This leads to a lot of memory usage on the accelerators (i.e. GPU), which limits the depth of trainable networks on accelerators or the batch size during training.
        In the inference stage, inconsistency and interval of memory consumption in time flow limits the parallelizability of models and sufficient usage of the computation resources.

The g$^n$Conv makes use of a recursive design to achieve higher-order spatial interactions.
 Although its channel decreasing design limits the FLOPs to an acceptable range, the recursive design brings a strong data dependency.
    When mapping to hardware, there exists a decreasing utilization rate of computation units in the g$^n$Conv operator due to the mandatory synchronization caused by the data dependencies.
    
Such excessive memory consumption and data hazards brings new opportunities and challenges to design a novel efficient high-order interactive neural network. In this work, we will show that, to build a hardware-friendly high-order neural network, quadratic neuron can play an important role.




\subsection{\textbf{Quadratic Neuron}}
\textbf{Neural Format:}
In contrast to the conventional neuron represented by a inner product of weight vector $W \in \mathbb{R}^{1 \times n}$ and input vector $\mathbf{x} \in \mathbb{R}^{n \times 1}$ plus a bias $b$ and an activation, the quadratic neuron can be written by an quadratic polynomial of input $\mathbf{x}$:
\begin{equation}
    y = \mathbf{x}^TW_q\mathbf{x} + W_c\mathbf{x} + b,
    \label{equ:quadratic_neuron}
\end{equation}
where $W_q \in \mathbf{R}^{n \times n}$ denotes a quadratic term weight and $W_c \in \mathbf{R}^{1 \times n}$ denotes a linear term weight. 
%Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, and thus it will rise the dimension interaction in data to a mandatory high-order format. 
%Since the high-order interaction among dimension is potential, rise it to a mandatory high-order format will miss the. 
    While the linear term promise a non-weaker learning ability than conventional CNNs, since the quadratic neuron includes a conventional neural network.
        Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, 
            and thus rise the potential high-order interaction to mandatory, causing a performance deduction.
            


\begin{figure}
    \centerline{\includegraphics[width = 3 in]{fig/quadratic_perceptron_1.pdf}}
    \caption{A perceptron with single quadratic neuron can solve a generalized XOR problem.}
    \label{fig:perceptron}
\end{figure}

\textbf{Design Motivation:}
To avoid huge memory consumption caused by a $O(n^2)$ intermediate state space and data dependency caused by high-order interactive neural network architecture design, we try to reduce the granularity of high-order computation from the level of network architectures to the level of neurons. 

A quadratic neuron brings more opportunities to discover nonlinear relations among data dimensions, because it performs a high-order interaction within the neuron for its quadratic computation. 
    Therefore, with a shallower network, a quadratic neural network can learn a smoother and richer nonlinear representation than conventional neural networks.
        Figure \ref{fig:perceptron} shows that for a generalized XOR classification problem, a single layer perceptron with a quadratic neuron can solve it alone, and gives even a more clear classification boundary than a two-layer perceptron with 10 hidden neurons.
        
When embedding quadratic neurons into a network architecture that is well optimized for computation flow, we will no longer suffer from the computational bottleneck caused by network design, while performing high-order interaction.

\textbf{Neuron Design Challenges:}
Although with powerful representation capacity coming with high-order interaction, the conventional quadratic neuron also brings a quadratic parameter space ($w_q$), an inappropriate implementation of quadratic neural networks will therefore cause unnecessary overhead. The optimization of quadratic neural network's computation will thus be a challenge. Luckily, there is still room for improvement in the design of quadratic neurons. In this work, co-design of quadratic neuron and computation block we proposed endows quadratic neurons with powerful information representation ability with very limited parameter space dilation.

\subsection{\textbf{Hardware-aware Neural Architecture Search}}
Neural Architecture Search (NAS) has been extensively used in the computer vision tasks during past few years. 
    Although NAS has achieved a huge success in finding high-performance neural networks, directly deploying NAS-synthesized complex neural architecture in resource-limited mobile devices is infeasible. 
    HW-NAS considers execution latency, memory footprint or energy footprint as one of the optimization objectives in the algorithms, and thus synthesizing a model well balanced between performance and hardware-specific computational consumption.

\textbf{Implementation Approach:}
Earlier on, few attention on NAS is given to high-order interactive networks because complex search space and large evaluation cost. 
    Recently, Some works \cite{gong2021nasvit,chen2021glit} tries to build a NAS synthesized ViT. However, they aims at a state-of-the-art neural architecture, which ignores the feasibility of the deployment on various devices. Consider the conciseness and hardware-friendliness of our QuadraNet, combining HW-NAS and QuadraNet to search a customized high-order interactive neural network architecture for specific computation platform will therefore be much intuitive.

    In this work, we don't look for particular innovation in NAS methodology but utilize it for investigating hardware-specific optimized quadratic neural architecture.
    

==> _hist/2-Background_v3.tex <==
\section{\textbf{Background and Motivation}}
\subsection{\textbf{High-Order Interactive Neural Networks}}
\textbf{Higher-Order Interaction:}
As aforementioned, the computing mechanism of neural networks has evolved from low-density convolution into high-density attention-like mechanisms.
%(e.g., spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self-attention \cite{dosovitskiy2020image})
%    These mechanisms could be formulated as follows:
%\begin{equation}
%    Attention(x) = f(g(x),x),
%\end{equation}
%where $x$ denotes input data and $g(x)$ generate an input-adaptive weight, and compute the final output with rule $f(\cdot,\cdot)$.
\JX{Their working mechanism can be captured by the following unified formula for high-order interactions as}
\sout{
These mechanisms can be generalized into an uniform high-order interaction formulation as:}
\begin{equation}
    x_{highorder}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(x)_{ij}W^{(c',c)}x^{(j,c')},
    \label{equ:highorder}
\end{equation}
where $\Omega_i$ denotes mechanism's receptive field, $g(x)$ denotes an interactive weight which contains input's information, $W^{(c',c)}$ denotes a channel-wise information transformation from channel $c'$ to $c$. 

Therefore, the multiplication of $x$ and input-adaptive $g(x)$ forms the high-order neural interaction of data itself.
%In such a formulation, usually, a high-order neural interaction can be observed as multiplication of data with itself or its transformation.
    Such an interaction represents leveraging the superposition of information between different dimensions of the data itself.
    
\textbf{Existing Approaches:}
%In the past decade, researchers found the effectiveness of attention mechanism. The attention mechanism uses the data itself to generate a set of parameters, and then multiply them with the data itself or their transformation. So no matter what kinds of attention (spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self attention \cite{dosovitskiy2020image}) used, it can be formulated in a high-order computation:
To capture the high-order spatial interaction, the latest \JX{STOA}\sout{star} models, ViT \cite{dosovitskiy2020image} and its variants \cite{liu2021swin,chu2021twins}, \JX{adopt}\sout{import} self-attention as the high-order interaction routine.
    In a vision task, self-attention's spatial mixing computation of the $c$-th channel at location $i$ can therefore be formulated as:
\begin{equation}
    x_{MHSA}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^CA(x)_{ij}W_V^{(c',c)}x^{(j,c')},
    \label{equ:self}
\end{equation}
where receptive field $\Omega_i$ is instantiated to the attention window, $A(x)$ is calculated by a softmax dot-product of Query and Key transfomation of input $x$. And self-attention forms channel-wise information transportation through Value transformation $W_V$. 
    This formulation that unifies with Equation \ref{equ:highorder} indicates self-attention is substantially a high-order interaction computation.
        
Different from the self-attention approach, HorNet \cite{rao2022hornet} performs high-order spatial interaction with a recursive convolution design. 
    HorNet \cite{rao2022hornet} comes up with a g$^n$Conv operator to perform high-order interaction computation. The output of g$^n$Conv can be formulated as:
\begin{equation}
    x_{g^nConv}^{(i,c)} = p_n^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(p_{n-1})w_{n-1,i\rightarrow j}^cW_{\phi_{in}}^{(c',c)}x^{(j,c')}.
    \label{equ:gnconv}
\end{equation}
Instead of generating high-order interaction by $g(x)$, g$^n$Conv uses a channel increasing recursive formulation $g(p_{n-1})$ to perform high-order iteration of information.

\textbf{Computation Challenges:}
The computation of existing high-order interaction approaches face multiple challenges in \textbf{memory consumption} or \textbf{data dependency}.

 \textbf{1) Memory Consumption with Intermediate States:}
 The computational process of self-attention generates a $O(n^2)$ intermediate state space.
    When mapping to hardware, ViT suffers from excessive memory consumption. 
        In the training stage, all the intermediate state tensors must be saved for the backpropagation. This leads to a lot of memory usage on the accelerators (i.e. GPU), which limits the depth of trainable networks on accelerators or the batch size during training.
        In the inference stage, \JX{please explain} inconsistency and interval of memory consumption in time flow limits the parallelizability of models and sufficient usage of the computation resources.

\textbf{2) Computation Cost with Data Dependency:} The g$^n$Conv makes use of a recursive design to achieve higher-order spatial interactions.
 Although its channel increasing design limits the FLOPs to an acceptable range, the recursive design brings a strong data dependency.
    When mapping to hardware, there exists a insufficient utilization of computation units in the g$^n$Conv operator due to the mandatory synchronization caused by the data dependencies.
    
Such excessive memory consumption and data hazards brings new opportunities and challenges to design a novel efficient high-order interactive neural network. In this work, we will show that, to build a hardware-friendly high-order neural network, quadratic neuron can play an important role.

\subsection{\textbf{Quadratic Neuron}}

 

\textbf{Neural Format:}
In contrast to the conventional neuron represented by a inner product of weight vector $W \in \mathbb{R}^{1 \times n}$ and input vector $\mathbf{x} \in \mathbb{R}^{n \times 1}$ plus a bias $b$ and an activation, the quadratic neuron can be written by an quadratic polynomial of input $\mathbf{x}$:
\begin{equation}
    y = \mathbf{x}^TW_q\mathbf{x} + W_c\mathbf{x} + b,
    \label{equ:quadratic_neuron}
\end{equation}
where $W_q \in \mathbf{R}^{n \times n}$ denotes a quadratic term weight and $W_c \in \mathbf{R}^{1 \times n}$ denotes a linear term weight. 
%Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, and thus it will rise the dimension interaction in data to a mandatory high-order format. 
%Since the high-order interaction among dimension is potential, rise it to a mandatory high-order format will miss the. 
    While the linear term promise a non-weaker learning ability than conventional CNNs, since the quadratic neuron includes a conventional neural network.
        Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, 
            and thus rise the potential high-order interaction to mandatory, causing a performance deduction.
            


\begin{figure}
    \centerline{\includegraphics[width=3.3in]{quadratic_perceptron_1}}
    \caption{XOR Representation Capability of Different Neurons \newline(Different colors reprensts xxx, dots and crosses are xxx)}
    %A perceptron with single quadratic neuron can solve a generalized XOR problem.}
    \label{fig:perceptron}
\end{figure}

\textbf{Design Motivation:}
To avoid huge memory consumption caused by a $O(n^2)$ intermediate state space and data dependency caused by high-order interactive neural network architecture design, we try to reduce the granularity of high-order computation from the level of network architectures to the level of neurons. 

A quadratic neuron brings more opportunities to discover nonlinear relations among data dimensions, because it performs a high-order interaction within the neuron for its quadratic computation. 
    Therefore, with a shallower network, a quadratic neural network can learn a smoother and richer nonlinear representation than conventional neural networks.
        Figure \ref{fig:perceptron} shows that for a generalized XOR classification problem, a single layer perceptron with a quadratic neuron can solve it alone, and gives even a more clear classification boundary than a two-layer perceptron with 10 hidden neurons.
        
When embedding quadratic neurons into a network architecture that is well optimized for computation flow, we will no longer suffer from the computational bottleneck caused by network design, while performing high-order interaction.

\textbf{Neuron Design Challenges:}
Although with powerful representation capacity coming with high-order interaction, the conventional quadratic neuron also brings a quadratic parameter space ($w_q$), an inappropriate implementation of quadratic neural networks will therefore cause unnecessary overhead. The optimization of quadratic neural network's computation will thus be a challenge. Luckily, there is still room for improvement in the design of quadratic neurons. In this work, co-design of quadratic neuron and computation block we proposed endows quadratic neurons with powerful information representation ability with very limited parameter space dilation.

\subsection{\textbf{Hardware-aware Neural Architecture Search}}
Neural Architecture Search (NAS) has been extensively used in the computer vision tasks during past few years. 
    Although NAS has achieved a huge success in finding high-performance neural networks, directly deploying NAS-synthesized complex neural architecture in resource-limited mobile devices is infeasible. 
    HW-NAS considers execution latency, memory footprint or energy footprint as one of the optimization objectives in the algorithms, and thus synthesizing a model well balanced between performance and hardware-specific computational consumption.
    Earlier on, few attention on NAS is given to high-order interactive networks because complex search space and large evaluation cost. 
    Recently, Some works \cite{gong2021nasvit,chen2021glit} tries to build a NAS synthesized ViT. However, they aims at a state-of-the-art neural architecture, which ignores the feasibility of the deployment on various devices. 
    
    \textbf{Implementation Approach:}
Consider the conciseness and hardware-friendliness of our QuadraNet, combining HW-NAS and QuadraNet to search a customized high-order interactive neural network architecture for specific computation platform will therefore be much intuitive.
    In this work, we don't look for particular innovation in NAS methodology but utilize it for investigating hardware-specific optimized quadratic neural architecture.
    

==> _hist/2-Background_v4-CX-JX.tex <==
\section{\textbf{Background and Motivation}}
\subsection{\textbf{High-Order Interactive Neural Networks}}

    
\textbf{Existing Approaches:}
%In the past decade, researchers found the effectiveness of attention mechanism. The attention mechanism uses the data itself to generate a set of parameters, and then multiply them with the data itself or their transformation. So no matter what kinds of attention (spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self attention \cite{dosovitskiy2020image}) used, it can be formulated in a high-order computation:
To capture the high-order spatial interaction, the latest \CX{state-of-the-art} models, ViT \cite{dosovitskiy2020image} and its variants \cite{liu2021swin,chu2021twins}, adopt self-attention as  \JX{a key} high-order interaction \JX{operation}.
    In a vision task, self-attention's spatial mixing computation of the $c$-th output channel at location $i$, \JX{$y_{SA}^{(i,c)}$ can be written as}:
\begin{equation}
    y_{SA}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^CA(x)_{i\rightarrow j}W_V^{(c',c)}x^{(j,c')},
    \label{equ:self}
\end{equation}
where  $\Omega_i$ is \JX{ the receptive field as} instantiated to the attention window, $A(x)$ \CX{is the input-adaptive weight matrix} calculated by a softmax dot-product of Query and Key transformations of input $x$, \CX{and $i\rightarrow j$ denotes the relative position of location $i$ and $j$}. Self-attention \JX{performs} channel-wise information \JX{interaction}\sout{transportation} through \JX{its} Value transformation \JX{of} $W_V$ \JX{on $x^{(j,c')}$}, and $(c',c)$ denotes the information \JX{interaction as manifested}\sout{transportation} from input channel $c'$ to output channel $c$. As aforementioned, the multiplication of input-dependent weights $A(x)$ and input $x$ generates a high-order interaction.
\
    %This formulation that unifies with Equation \ref{equ:highorder} indicates self-attention is substantially a high-order interaction computation.
        
Different from the self-attention approach, HorNet \cite{rao2022hornet} performs high-order spatial interaction with a recursive convolution design. 
    HorNet \cite{rao2022hornet} \JX{proposes} a g$^n$Conv \JX{operation} to perform high-order interaction computation. The output of g$^n$Conv can be formulated as:
\begin{equation}
    y_{g^nConv}^{(i,c)} = p_n^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(p_{n-1})w_{n-1,i\rightarrow j}^cW_{\phi_{in}}^{(c',c)}x^{(j,c')}.
    \label{equ:gnconv}
\end{equation}
Instead of generating high-order interaction directly input $x$, g$^n$Conv uses a channel increasing recursive formulation $g(p_{n-1})$ to perform high-order iteration of information, and therefore getting an input-adaptive weight. $W_{\phi_{in}}^{(c',c)}$ is an input projection.

\textbf{Higher-Order Interaction:}
%As aforementioned, the computing mechanism of neural networks has evolved from low-density convolution into high-density attention-like mechanisms.
\CX{Summarizing the above work, we find that both of them adopt an input-dependent weight matrix, a channel-wise information transformation.}
%(e.g., spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self-attention \cite{dosovitskiy2020image})
%    These mechanisms could be formulated as follows:
%\begin{equation}
%    Attention(x) = f(g(x),x),
%\end{equation}
%where $x$ denotes input data and $g(x)$ generate an input-adaptive weight, and compute the final output with rule $f(\cdot,\cdot)$.
\JX{Therefore, their working mechanism can be captured by the following unified formula for high-order interactions as:}
%\sout{
%These mechanisms can be generalized into an uniform high-order interaction formulation as:}
\begin{equation}
    y_{highorder}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(x)_{ij}W^{(c',c)}x^{(j,c')},
    \label{equ:highorder}
\end{equation}
where $\Omega_i$ denotes mechanism's receptive field, $g(x)$ denotes an interactive weight which contains input's information, $W^{(c',c)}$ denotes a channel-wise information transformation from channel $c'$ to $c$. And the multiplication of $x$ and input-adaptive $g(x)$ forms the high-order neural interaction of data itself.
%In such a formulation, usually, a high-order neural interaction can be observed as multiplication of data with itself or its transformation.
    Such an interaction represents leveraging the superposition of information between different dimensions of the data itself.

\textbf{Computation Challenges:}
The computation of existing high-order interaction approaches face multiple challenges in \textbf{memory consumption} or \textbf{data dependency}.

 \textbf{1) Memory Consumption with Intermediate States:}
 The computational process of self-attention generates a \CX{quadratic} intermediate state space. \CX{To be specific, the the transformation of Q, K and V generates $3C^2HW$ intermediate states, and the $softmax(QK^T/\sqrt{d_k})$ takes $2(HW)^2C/Patch\_area$ intermediate states, where $H$, $W$and $C$ denote the height, width and channels of input. }
    When mapping to hardware, ViT suffers from excessive memory consumption. 
        In the training stage, all the intermediate state tensors must be saved for the backpropagation. This leads to a lot of memory usage on the accelerators (i.e. GPU), which limits the depth of trainable networks on accelerators or the batch size during training.
        In the inference stage, \JX{please explain}\CX{the continuous generation and release of intermediate states causes} inconsistency and interval of memory consumption in time flow, which limits the parallelizability \CX{(depends on the moment that intermediate state occupies the most memory)} of models and sufficient usage of the computation resources.

\textbf{2) Computation Cost with Data Dependency:} The g$^n$Conv makes use of a recursive design to achieve higher-order spatial interactions.
 Although its channel increasing design limits the FLOPs to an acceptable range, the recursive design brings a strong data dependency.
    When mapping to hardware, there exists a insufficient utilization of computation units in the g$^n$Conv operator due to the mandatory synchronization caused by the data dependencies.
    
Such excessive memory consumption and data hazards brings new opportunities and challenges to design a novel efficient high-order interactive neural network. In this work, we will show that, to build a hardware-friendly high-order neural network, quadratic neuron can play an important role.

\subsection{\textbf{Quadratic Neuron}}

 

\textbf{Neural Format:}
In contrast to the conventional neuron represented by a inner product of weight vector $W \in \mathbb{R}^{1 \times n}$ and input vector $\mathbf{x} \in \mathbb{R}^{n \times 1}$ plus a bias $b$ and an activation, the quadratic neuron can be written by an quadratic polynomial of input $\mathbf{x}$:
\begin{equation}
    y = \mathbf{x}^TW_q\mathbf{x} + W_c\mathbf{x} + b,
    \label{equ:quadratic_neuron}
\end{equation}
where $W_q \in \mathbf{R}^{n \times n}$ denotes a quadratic term weight and $W_c \in \mathbf{R}^{1 \times n}$ denotes a linear term weight. 
%Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, and thus it will rise the dimension interaction in data to a mandatory high-order format. 
%Since the high-order interaction among dimension is potential, rise it to a mandatory high-order format will miss the. 
    While the linear term promise a non-weaker learning ability than conventional CNNs, since the quadratic neuron includes a conventional neural network.
        Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, 
            and thus rise the potential high-order interaction to mandatory, causing a performance deduction.
            


\begin{figure}
    \centerline{\includegraphics[width=3.3in]{quadratic_perceptron_1}}
    \caption{XOR Representation Capability of Different Neurons \newline(Different colors reprensts xxx, dots and crosses are xxx)}
    %A perceptron with single quadratic neuron can solve a generalized XOR problem.}
    \label{fig:perceptron}
\end{figure}

\textbf{Design Motivation:}
To avoid huge memory consumption caused by a $O(n^2)$ intermediate state space and data dependency caused by high-order interactive neural network architecture design, we try to reduce the granularity of high-order computation from the level of network architectures to the level of neurons. 

A quadratic neuron brings more opportunities to discover nonlinear relations among data dimensions, because it performs a high-order interaction within the neuron for its quadratic computation. 
    Therefore, with a shallower network, a quadratic neural network can learn a smoother and richer nonlinear representation than conventional neural networks.
        Figure \ref{fig:perceptron} shows that for a generalized XOR classification problem, a single layer perceptron with a quadratic neuron can solve it alone, and gives even a more clear classification boundary than a two-layer perceptron with 10 hidden neurons.
        
When embedding quadratic neurons into a network architecture that is well optimized for computation flow, we will no longer suffer from the computational bottleneck caused by network design, while performing high-order interaction.

\textbf{Neuron Design Challenges:}
Although with powerful representation capacity coming with high-order interaction, the conventional quadratic neuron also brings a quadratic parameter space ($w_q$), an inappropriate implementation of quadratic neural networks will therefore cause unnecessary overhead. The optimization of quadratic neural network's computation will thus be a challenge. Luckily, there is still room for improvement in the design of quadratic neurons. In this work, co-design of quadratic neuron and computation block we proposed endows quadratic neurons with powerful information representation ability with very limited parameter space dilation.

\subsection{\textbf{Hardware-aware Neural Architecture Search}}
Neural Architecture Search (NAS) has been extensively used in the computer vision tasks during past few years. 
    Although NAS has achieved a huge success in finding high-performance neural networks, directly deploying NAS-synthesized complex neural architecture in resource-limited mobile devices is infeasible. 
    HW-NAS considers execution latency, memory footprint or energy footprint as one of the optimization objectives in the algorithms, and thus synthesizing a model well balanced between performance and hardware-specific computational consumption.
    Earlier on, few attention on NAS is given to high-order interactive networks because complex search space and large evaluation cost. 
    Recently, Some works \cite{gong2021nasvit,chen2021glit} tries to build a NAS synthesized ViT. However, they aims at a state-of-the-art neural architecture, which ignores the feasibility of the deployment on various devices. 
    
    \textbf{Implementation Approach:}
Consider the conciseness and hardware-friendliness of our QuadraNet, combining HW-NAS and QuadraNet to search a customized high-order interactive neural network architecture for specific computation platform will therefore be much intuitive.
    In this work, we don't look for particular innovation in NAS methodology but utilize it for investigating hardware-specific optimized quadratic neural architecture.

==> _hist/2-Background_v4-CX.tex <==
\section{\textbf{Background and Motivation}}
\subsection{\textbf{High-Order Interactive Neural Networks}}

    
\textbf{Existing Approaches:}
%In the past decade, researchers found the effectiveness of attention mechanism. The attention mechanism uses the data itself to generate a set of parameters, and then multiply them with the data itself or their transformation. So no matter what kinds of attention (spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self attention \cite{dosovitskiy2020image}) used, it can be formulated in a high-order computation:
To capture the high-order spatial interaction, the latest \CX{state-of-the-art} models, ViT \cite{dosovitskiy2020image} and its variants \cite{liu2021swin,chu2021twins}, adopt self-attention as the high-order interaction routine.
    In a vision task, self-attention's spatial mixing computation of the $c$-th output channel at location $i$ can therefore be formulated as:
\begin{equation}
    y_{SA}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^CA(x)_{i\rightarrow j}W_V^{(c',c)}x^{(j,c')},
    \label{equ:self}
\end{equation}
where receptive field $\Omega_i$ is instantiated to the attention window, $A(x)$ \CX{is an input-adaptive weight matrix} calculated by a softmax dot-product of Query and Key transfomation of input $x$, \CX{and $i\rightarrow j$ denotes the relative position of location $i$ and $j$}. Self-attention forms channel-wise information transportation through Value transformation $W_V$, and $(c',c)$ denotes the information transportation from input channel $c'$ to output channel $c$. As aforementioned, the multiplication of input-dependent weights $A(x)$ and input $x$ generate high-order interaction.
\
    %This formulation that unifies with Equation \ref{equ:highorder} indicates self-attention is substantially a high-order interaction computation.
        
Different from the self-attention approach, HorNet \cite{rao2022hornet} performs high-order spatial interaction with a recursive convolution design. 
    HorNet \cite{rao2022hornet} comes up with a g$^n$Conv operator to perform high-order interaction computation. The output of g$^n$Conv can be formulated as:
\begin{equation}
    y_{g^nConv}^{(i,c)} = p_n^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(p_{n-1})w_{n-1,i\rightarrow j}^cW_{\phi_{in}}^{(c',c)}x^{(j,c')}.
    \label{equ:gnconv}
\end{equation}
Instead of generating high-order interaction directly input $x$, g$^n$Conv uses a channel increasing recursive formulation $g(p_{n-1})$ to perform high-order iteration of information, and therefore getting an input-adaptive weight. $W_{\phi_{in}}^{(c',c)}$ is an input projection.

\textbf{Higher-Order Interaction:}
%As aforementioned, the computing mechanism of neural networks has evolved from low-density convolution into high-density attention-like mechanisms.
\CX{Summarizing the above work, we find that both of them adopt an input-dependent weight matrix, a channel-wise information transformation.}
%(e.g., spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self-attention \cite{dosovitskiy2020image})
%    These mechanisms could be formulated as follows:
%\begin{equation}
%    Attention(x) = f(g(x),x),
%\end{equation}
%where $x$ denotes input data and $g(x)$ generate an input-adaptive weight, and compute the final output with rule $f(\cdot,\cdot)$.
\JX{Therefore, their working mechanism can be captured by the following unified formula for high-order interactions as:}
%\sout{
%These mechanisms can be generalized into an uniform high-order interaction formulation as:}
\begin{equation}
    y_{highorder}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(x)_{ij}W^{(c',c)}x^{(j,c')},
    \label{equ:highorder}
\end{equation}
where $\Omega_i$ denotes mechanism's receptive field, $g(x)$ denotes an interactive weight which contains input's information, $W^{(c',c)}$ denotes a channel-wise information transformation from channel $c'$ to $c$. And the multiplication of $x$ and input-adaptive $g(x)$ forms the high-order neural interaction of data itself.
%In such a formulation, usually, a high-order neural interaction can be observed as multiplication of data with itself or its transformation.
    Such an interaction represents leveraging the superposition of information between different dimensions of the data itself.

\textbf{Computation Challenges:}
The computation of existing high-order interaction approaches face multiple challenges in \textbf{memory consumption} or \textbf{data dependency}.

 \textbf{1) Memory Consumption with Intermediate States:}
 The computational process of self-attention generates a quadratic intermediate state space.
    When mapping to hardware, ViT suffers from excessive memory consumption. 
        In the training stage, all the intermediate state tensors must be saved for the backpropagation. This leads to a lot of memory usage on the accelerators (i.e. GPU), which limits the depth of trainable networks on accelerators or the batch size during training.
        In the inference stage, \JX{please explain}\CX{the continuous generation and release of intermediate states causes} inconsistency and interval of memory consumption in time flow, which limits the parallelizability \CX{(depends on the moment that intermediate state occupies the most memory)} of models and sufficient usage of the computation resources.

\textbf{2) Computation Cost with Data Dependency:} The g$^n$Conv makes use of a recursive design to achieve higher-order spatial interactions.
 Although its channel increasing design limits the FLOPs to an acceptable range, the recursive design brings a strong data dependency.
    When mapping to hardware, there exists a insufficient utilization of computation units in the g$^n$Conv operator due to the mandatory synchronization caused by the data dependencies.
    
Such excessive memory consumption and data hazards brings new opportunities and challenges to design a novel efficient high-order interactive neural network. In this work, we will show that, to build a hardware-friendly high-order neural network, quadratic neuron can play an important role.

\subsection{\textbf{Quadratic Neuron}}

 

\textbf{Neural Format:}
In contrast to the conventional neuron represented by a inner product of weight vector $W \in \mathbb{R}^{1 \times n}$ and input vector $\mathbf{x} \in \mathbb{R}^{n \times 1}$ plus a bias $b$ and an activation, the quadratic neuron can be written by an quadratic polynomial of input $\mathbf{x}$:
\begin{equation}
    y = \mathbf{x}^TW_q\mathbf{x} + W_c\mathbf{x} + b,
    \label{equ:quadratic_neuron}
\end{equation}
where $W_q \in \mathbf{R}^{n \times n}$ denotes a quadratic term weight and $W_c \in \mathbf{R}^{1 \times n}$ denotes a linear term weight. 
%Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, and thus it will rise the dimension interaction in data to a mandatory high-order format. 
%Since the high-order interaction among dimension is potential, rise it to a mandatory high-order format will miss the. 
    While the linear term promise a non-weaker learning ability than conventional CNNs, since the quadratic neuron includes a conventional neural network.
        Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, 
            and thus rise the potential high-order interaction to mandatory, causing a performance deduction.
            


\begin{figure}
    \centerline{\includegraphics[width=3.3in]{quadratic_perceptron_1}}
    \caption{XOR Representation Capability of Different Neurons \newline(Different colors reprensts xxx, dots and crosses are xxx)}
    %A perceptron with single quadratic neuron can solve a generalized XOR problem.}
    \label{fig:perceptron}
\end{figure}

\textbf{Design Motivation:}
To avoid huge memory consumption caused by a $O(n^2)$ intermediate state space and data dependency caused by high-order interactive neural network architecture design, we try to reduce the granularity of high-order computation from the level of network architectures to the level of neurons. 

A quadratic neuron brings more opportunities to discover nonlinear relations among data dimensions, because it performs a high-order interaction within the neuron for its quadratic computation. 
    Therefore, with a shallower network, a quadratic neural network can learn a smoother and richer nonlinear representation than conventional neural networks.
        Figure \ref{fig:perceptron} shows that for a generalized XOR classification problem, a single layer perceptron with a quadratic neuron can solve it alone, and gives even a more clear classification boundary than a two-layer perceptron with 10 hidden neurons.
        
When embedding quadratic neurons into a network architecture that is well optimized for computation flow, we will no longer suffer from the computational bottleneck caused by network design, while performing high-order interaction.

\textbf{Neuron Design Challenges:}
Although with powerful representation capacity coming with high-order interaction, the conventional quadratic neuron also brings a quadratic parameter space ($w_q$), an inappropriate implementation of quadratic neural networks will therefore cause unnecessary overhead. The optimization of quadratic neural network's computation will thus be a challenge. Luckily, there is still room for improvement in the design of quadratic neurons. In this work, co-design of quadratic neuron and computation block we proposed endows quadratic neurons with powerful information representation ability with very limited parameter space dilation.

\subsection{\textbf{Hardware-aware Neural Architecture Search}}
Neural Architecture Search (NAS) has been extensively used in the computer vision tasks during past few years. 
    Although NAS has achieved a huge success in finding high-performance neural networks, directly deploying NAS-synthesized complex neural architecture in resource-limited mobile devices is infeasible. 
    HW-NAS considers execution latency, memory footprint or energy footprint as one of the optimization objectives in the algorithms, and thus synthesizing a model well balanced between performance and hardware-specific computational consumption.
    Earlier on, few attention on NAS is given to high-order interactive networks because complex search space and large evaluation cost. 
    Recently, Some works \cite{gong2021nasvit,chen2021glit} tries to build a NAS synthesized ViT. However, they aims at a state-of-the-art neural architecture, which ignores the feasibility of the deployment on various devices. 
    
    \textbf{Implementation Approach:}
Consider the conciseness and hardware-friendliness of our QuadraNet, combining HW-NAS and QuadraNet to search a customized high-order interactive neural network architecture for specific computation platform will therefore be much intuitive.
    In this work, we don't look for particular innovation in NAS methodology but utilize it for investigating hardware-specific optimized quadratic neural architecture.

==> _hist/2-Background_v5-XC-CX.tex <==
\section{\textbf{Background and Motivation}}

\subsection{\textbf{High-Order Interactive Neural Networks}}

\textbf{Existing Approaches:}
To capture high-order neural interactions, Transformer-like neural network models, such as ViT~\cite{dosovitskiy2020image} and its variants~\cite{liu2021swin,chu2021twins}, adopt the self-attention mechanism as aforementioned.
	In a vision task, self-attention performs spatial mixing computation $y_{SA}^{(i,c)}$ of $c^{th}$ output channel at location $i$, which can be written as:
	\begin{equation}
		y_{SA}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^CA(x)_{i\rightarrow j}W_V^{(c',c)}x^{(j,c')},
		\label{equ:self}
	\end{equation}
where $\Omega_i$ is the receptive field\CX{ (i.e. attention window in \cite{liu2021swin}) involving interaction}, $A(x)$ is the input-adaptive weight matrix calculated by a softmax dot-production of ``query'' ($Q$) and ``key'' ($K$) transformations of the input $x$, and $i$~$\rightarrow$~$j$ process denotes the relative position of location $i$ and $j$.
	Therefore, self-attention achieves channel-wise information interaction through its ``value'' ($V$) transformation of $W_V$ on $x^{(j,c')}$, and $(c',c)$ denotes the information interaction as manifested from input channel $c'$ to output channel $c$.
	As aforementioned, the multiplication of input-dependent weights $A(x)$ and input $x$ forms high-order interactions and thus corresponding expected cognition performance.

\begin{comment}
	% where  $\Omega_i$ is \JX{ the receptive field as} instantiated to the attention window, $A(x)$ \CX{is the input-adaptive weight matrix} calculated by a softmax dot-product of Query and Key transformations of input $x$, \CX{and $i\rightarrow j$ denotes the relative position of location $i$ and $j$}.
	%Self-attention \JX{performs} channel-wise information \JX{interaction}\sout{transportation} through \JX{its} Value transformation \JX{of} $W_V$ \JX{on $x^{(j,c')}$}, and $(c',c)$ denotes the information \JX{interaction as manifested}\sout{transportation} from input channel $c'$ to output channel $c$.
	%As aforementioned, the multiplication of input-dependent weights $A(x)$ and input $x$ generates a high-order interaction.
\end{comment}
\begin{comment}
	%In the past decade, researchers found the effectiveness of attention mechanism. The attention mechanism uses the data itself to generate a set of parameters, and then multiply them with the data itself or their transformation. So no matter what kinds of attention (spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self attention \cite{dosovitskiy2020image}) used, it can be formulated in a high-order computation:
	%This formulation that unifies with Equation \ref{equ:highorder} indicates self-attention is substantially a high-order interaction computation.
\end{comment}

Different from the self-attention approach shown in Eq.~\ref{equ:self}, HorNet \cite{rao2022hornet} performs high-order neural interactions with a recursive convolution design --- g$^n$Conv, which can be formulated as:
    % Specifically, HorNet proposes a g$^n$Conv operation to perform high-order interaction computation. The output of g$^n$Conv can be formulated as:
\begin{equation}
	\hspace{-3mm}y_{g^nConv}^{(i,c)} = p_n^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(p_{n-1})w_{n-1,i\rightarrow j}^cW_{\phi_{in}}^{(c',c)}x^{(j,c')}.
	\label{equ:gnconv}
\end{equation}
	Instead of generating high-order interaction directly \CX{from} input $x$, g$^n$Conv uses a channel increasing recursive formulation $g(p_{n-1})$ to perform high-order iteration of information, and therefore getting an input-adaptive weight. $W_{\phi_{in}}^{(c',c)}$ is an input projection.




\textbf{Higher-Order Interaction:}
Summarizing the above works, we find that both of them adopt an input-dependent weight matrix --- a channel-wise information transformation.
	Therefore, their working mechanism can be captured by the following unified formula for high-order interactions as:
\begin{equation}
	y_{highorder}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(x)_{ij}W^{(c',c)}x^{(j,c')},
	\label{equ:highorder}
\end{equation}
where $\Omega_i$ denotes mechanism's receptive field \CX{involving neural interaction}, $g(x)$ denotes an interactive weight which contains input's information, $W^{(c',c)}$ denotes a channel-wise information transformation from channel $c'$ to $c$.
	And the multiplication of $x$ and input-adaptive $g(x)$ forms the high-order neural interaction of data itself.
	Such an interaction represents leveraging the superposition of information between different feature dimensions of the input data itself.

\begin{comment}
	% As aforementioned, the computing mechanism of neural networks has evolved from low-density convolution into high-density attention-like mechanisms.
	% (e.g., spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self-attention \cite{dosovitskiy2020image})
	% These mechanisms could be formulated as follows:
	% \begin{equation}
		% Attention(x) = f(g(x),x),
	%\end{equation}
	%where $x$ denotes input data and $g(x)$ generate an input-adaptive weight, and compute the final output with rule $f(\cdot,\cdot)$.
	%\sout{These mechanisms can be generalized into an uniform high-order interaction formulation as:}
	%In such a formulation, usually, a high-order neural interaction can be observed as multiplication of data with itself or its transformation.
\end{comment}




\textbf{Computation Challenges:}
The computation of existing high-order interaction approaches (esp., self-attention) face multiple challenges in terms of memory consumption and computation cost.

\textbf{(1) \textit{Memory Consumption with Intermediate States:}}
As aforementioned, self-attention generation introduces a quadratic intermediate state space.
% ATTENTION!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
% 尽管你后面分作training 和inference讲了很多heavy load，但是你会发现橙色字段跟后面没有一根毛的联系啊。。。你给的公式并没有利用好啊。你需要一方面把橙色字写清楚。另一方面把这些公式用到后面的描述中。
	\TD{Specifically, the transformation process of $Q$, $K$, and $V$ parameters in Transformer-like models generates $3HWC$ intermediate states, and the $softmax(QK^T)V$ takes intermediate states as many as $(HW)^2+(HW)^2C$, where $H$, $W$and $C$ denote the height, width, and channels of the input in this layer.}
	\CX{Compared with widely-used depthwise separable convolution (depthwise convolution + pointwise convolution) which generates only $HWC$ intermediate states, self-attention needs $(HW+3) \times$ intermediate states to finish its computation. Even if attention is restricted to a local window as in \cite{liu2021swin}, the computation of self-attention still yields $(M^2+3)\times$ intermediate states, where $M$ denotes the window size (usually 7 or larger).} 
	%CX:\sqrt(d_k)的对intermediate space 没有影响，删除了这个概念。
	Due to such a huge amount of data movement across intermediate states, conventional Transformer-like models usually suffer from excessive memory consumption.
	In the training stage, all the data in intermediate states must be saved for the backpropagation, leading considerable memory costs and design limits of model architecture volumes or batch tuning flexibility.
	In the inference stage, frequent and continuous generation and release of intermediate states during the forward propagation also cast inconsistency and interval of memory consumption in time flow.
\begin{comment}
	% When mapping to hardware, ViT suffers from excessive memory consumption.
	% This leads to a lot of memory usage on the accelerators (i.e. GPU), which limits the depth of trainable networks on accelerators or the batch size during training.
	% In the inference stage, \JX{please explain}\CX{the continuous generation and release of intermediate states causes} inconsistency and interval of memory consumption in time flow, which limits the parallelizability \CX{(depends on the moment that intermediate state occupies the most memory)} of models and sufficient usage of the computation resources.
\end{comment}


\textbf{\textit{(2) Computation Cost with Data Dependency:}}
In addition to the memory consumption, the complex computing logistic in self-attention also introduces considerable costs.
	For example, the computation of g$^n$Conv in HorNet makes use of a recursive design to achieve higher-order spatial interactions.
	\GR{Although its \sout{\TD{channel} increasing} \CX{ingenious} design limits the FLOPs to an acceptable range, the recursive design brings a strong data dependency.
	% 这里channel的用法跟上面接不上。我不确认channel这个词是对的。总之我改到这里，channel这个词在我脑海里没啥感觉。
	\CX{The next order of interaction in g$^n$Conv must wait for the previous order of interaction to complete before it can proceed, in other words, $n$ times interactions means $n$ times synchronizations.}
	When mapping to hardware, there exists a insufficient utilization of computation units in the g$^n$Conv operator due to the mandatory synchronization caused by the data dependencies.}
	% 这一段话，写的也不清楚，问题跟上面的差不多，就只是一些general 的描述。不太清楚到底是多少。

Such excessive intermediate states and data dependency bring new opportunities and challenges to design a novel efficient high-order interactive neural network.
	In this work, we will show that, quadratic neuron can play an important role.

\begin{figure}
	\centerline{\includegraphics[width=3.5in]{quadratic_perceptron_1}}
	\caption{XOR Representation Capability of Different Neurons \newline(Different colors reprensts xxx, dots and crosses are xxx)}
	%A perceptron with single quadratic neuron can solve a generalized XOR problem.}
	\label{fig:perceptron}
	\vspace{-3.4mm}
\end{figure}



\subsection{\textbf{\TD{Quadratic Neuron}}}
A quadratic neuron brings more opportunities to discover nonlinear relations among data dimensions, because it performs a high-order interaction within the neuron for its quadratic computation.
	Therefore, with a shallower network, a quadratic neural network can learn a smoother and richer nonlinear representation than conventional neural networks.
	Fig.~\ref{fig:perceptron} shows that for a generalized XOR classification problem, a single layer perceptron with a quadratic neuron can solve it alone, and gives even a more clear classification boundary than a two-layer perceptron with 10 hidden neurons.
	
\textbf{Neural Format:}
In contrast to the conventional neuron represented by a inner product of weight vector $W \in \mathbb{R}^{1 \times n}$ and input vector $\mathbf{x} \in \mathbb{R}^{n \times 1}$ plus a bias $b$ and an activation, the quadratic neuron can be written by an quadratic polynomial of input $\mathbf{x}$:
	\begin{equation}
		\mathbf{y} = \mathbf{x}^TW_q\mathbf{x} + W_c\mathbf{x} + b,
		\label{equ:quadratic_neuron}
	\end{equation}
where $W_q \in \mathbb{R}^{n \times n}$ denotes a quadratic term weight and $W_c \in \mathbb{R}^{1 \times n}$ denotes a linear term weight.

\CX{\sout{While}} The linear term promise a non-weaker learning ability than a conventional neural network, since it is included in the quadratic neural network.
	Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, and thus rise the potential high-order interaction to mandatory, causing a performance deduction.
\begin{comment}


	%Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, and thus it will rise the dimension interaction in data to a mandatory high-order format.
	%Since the high-order interaction among dimension is potential, rise it to a mandatory high-order format will miss the.
\end{comment}



\textbf{Design Motivation:}
To avoid huge memory consumption caused by a large intermediate state space and data dependency caused by high-order interactive neural network architecture design, we try to reduce the granularity of high-order interaction computation from the level of network architectures to the level of neurons. Interaction within the quadratic neuron makes it possible. When embedding quadratic neurons into a network architecture that is well optimized for computation flow, we will no longer suffer from the computational bottleneck caused by network design, while performing high-order neural interaction.


\textbf{Neuron Design Challenges:}
\FN{Although embedding high-order interactions into neuron-level, conventional quadratic neurons also generate a quadratic parameter space ($W_q \in \mathbb{R}^{n\times n}$)}\CX{, which means we now have $n^2$, instead of $n$ in conventional neuron, learnable parameters need updating.}
	\TD{Therefore, an inappropriate implementation of quadratic neural networks would still cause certain computing issues.}
	% 到底是个什么parameter space？这个问题其实非常重要，而不是一句话打法了。因为他是你后面设计的motivation。
	\FN{In this work, we will carefully examine the quadratic neural network from neuron to structural blocks and eventually to the overall model design to comprehensively optimize the parameter space dilation issue whiling maintaining quadratic neurons with powerful high-order neural interaction ability.}
	% The optimization of quadratic neural network's computation will thus be a challenge.
	% Luckily, there is still room for improvement in the design of quadratic neurons.




\subsection{\textbf{Hardware-aware Neural Architecture Search}}
\FN{Neural Architecture Search (NAS) has been extensively used in the computer vision tasks during past few years.
	% Although NAS has achieved a huge success in finding high-performance neural networks, directly deploying NAS-synthesized complex neural architecture in resource-limited mobile devices is infeasible.
	Particularly, hardware-aware NAS considers system execution latency, memory footprint, or energy footprint as one of the optimization objectives in algorithms, and thus synthesizing a model that is well balanced between cognition and computing performance.}

\FN{Earlier on, few attention from NAS area is given to high-order interactive neural networks due to complex search space and large evaluation cost.
	Only very recently, the popularity of Transformer-like modleds triggered some works to build a NAS synthesized ViT~\cite{gong2021nasvit,chen2021glit}.
	However, even these works only focused on the cognition performance without considering hardware awareness, not to mention the breakthrough to high-order neuron designs.}

\FN{In this work, we target to endorse hardware-awareness into the proposed \textit{QuadraNet} and expand its generalization capability.
	Therefore, we will incorporate mature NAS techniques into our design methodology to search adaptive high-order interactive neural network architecture for various deployment scenarios.}


==> _hist/2-Background_v5-XC.tex <==
\section{\textbf{Background and Motivation}}

\subsection{\textbf{High-Order Interactive Neural Networks}}

\textbf{Existing Approaches:}
To capture high-order neural interactions, Transformer-like neural network models, such as ViT~\cite{dosovitskiy2020image} and its variants~\cite{liu2021swin,chu2021twins}, adopt the self-attention mechanism as aforementioned.
	In a vision task, self-attention performs spatial mixing computation $y_{SA}^{(i,c)}$ of $c^{th}$ output channel at location $i$, which can be written as:
	\begin{equation}
		y_{SA}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^CA(x)_{i\rightarrow j}W_V^{(c',c)}x^{(j,c')},
		\label{equ:self}
	\end{equation}
where $\Omega_i$ is the receptive field as instantiated to the attention window, $A(x)$ is the input-adaptive weight matrix calculated by a softmax dot-production of ``query'' ($Q$) and ``key'' ($K$) transformations of the input $x$, and $i$~$\rightarrow$~$j$ process denotes the relative position of location $i$ and $j$.
	Therefore, self-attention achieves channel-wise information interaction through its ``value'' ($V$) transformation of $W_V$ on $x^{(j,c')}$, and $(c',c)$ denotes the information interaction as manifested from input channel $c'$ to output channel $c$.
	As aforementioned, the multiplication of input-dependent weights $A(x)$ and input $x$ forms high-order interactions and thus corresponding expected cognition performance.

\begin{comment}
	% where  $\Omega_i$ is \JX{ the receptive field as} instantiated to the attention window, $A(x)$ \CX{is the input-adaptive weight matrix} calculated by a softmax dot-product of Query and Key transformations of input $x$, \CX{and $i\rightarrow j$ denotes the relative position of location $i$ and $j$}.
	%Self-attention \JX{performs} channel-wise information \JX{interaction}\sout{transportation} through \JX{its} Value transformation \JX{of} $W_V$ \JX{on $x^{(j,c')}$}, and $(c',c)$ denotes the information \JX{interaction as manifested}\sout{transportation} from input channel $c'$ to output channel $c$.
	%As aforementioned, the multiplication of input-dependent weights $A(x)$ and input $x$ generates a high-order interaction.
\end{comment}
\begin{comment}
	%In the past decade, researchers found the effectiveness of attention mechanism. The attention mechanism uses the data itself to generate a set of parameters, and then multiply them with the data itself or their transformation. So no matter what kinds of attention (spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self attention \cite{dosovitskiy2020image}) used, it can be formulated in a high-order computation:
	%This formulation that unifies with Equation \ref{equ:highorder} indicates self-attention is substantially a high-order interaction computation.
\end{comment}

Different from the self-attention approach shown in Eq.~\ref{equ:self}, HorNet \cite{rao2022hornet} performs high-order neural interactions with a recursive convolution design --- g$^n$Conv, which can be formulated as:
    % Specifically, HorNet proposes a g$^n$Conv operation to perform high-order interaction computation. The output of g$^n$Conv can be formulated as:
\begin{equation}
	\hspace{-3mm}y_{g^nConv}^{(i,c)} = p_n^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(p_{n-1})w_{n-1,i\rightarrow j}^cW_{\phi_{in}}^{(c',c)}x^{(j,c')}.
	\label{equ:gnconv}
\end{equation}
	Instead of generating high-order interaction directly input $x$, g$^n$Conv uses a channel increasing recursive formulation $g(p_{n-1})$ to perform high-order iteration of information, and therefore getting an input-adaptive weight. $W_{\phi_{in}}^{(c',c)}$ is an input projection.




\textbf{Higher-Order Interaction:}
Summarizing the above works, we find that both of them adopt an input-dependent weight matrix --- a channel-wise information transformation.
	Therefore, their working mechanism can be captured by the following unified formula for high-order interactions as:
\begin{equation}
	y_{highorder}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(x)_{ij}W^{(c',c)}x^{(j,c')},
	\label{equ:highorder}
\end{equation}
where $\Omega_i$ denotes mechanism's receptive field, $g(x)$ denotes an interactive weight which contains input's information, $W^{(c',c)}$ denotes a channel-wise information transformation from channel $c'$ to $c$.
	And the multiplication of $x$ and input-adaptive $g(x)$ forms the high-order neural interaction of data itself.
	Such an interaction represents leveraging the superposition of information between different feature dimensions of the input data itself.

\begin{comment}
	% As aforementioned, the computing mechanism of neural networks has evolved from low-density convolution into high-density attention-like mechanisms.
	% (e.g., spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self-attention \cite{dosovitskiy2020image})
	% These mechanisms could be formulated as follows:
	% \begin{equation}
		% Attention(x) = f(g(x),x),
	%\end{equation}
	%where $x$ denotes input data and $g(x)$ generate an input-adaptive weight, and compute the final output with rule $f(\cdot,\cdot)$.
	%\sout{These mechanisms can be generalized into an uniform high-order interaction formulation as:}
	%In such a formulation, usually, a high-order neural interaction can be observed as multiplication of data with itself or its transformation.
\end{comment}




\textbf{Computation Challenges:}
The computation of existing high-order interaction approaches (esp., self-attention) face multiple challenges in terms of memory consumption and computation cost.

\textbf{(1) \textit{Memory Consumption with Intermediate States:}}
As aforementioned, self-attention generation introduces a quadratic intermediate state space.
% ATTENTION!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
% !!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
% 尽管你后面分作training 和inference讲了很多heavy load，但是你会发现橙色字段跟后面没有一根毛的联系啊。。。你给的公式并没有利用好啊。你需要一方面把橙色字写清楚。另一方面把这些公式用到后面的描述中。
	\TD{Specifically, the transformation process of $Q$, $K$, and $V$ parameters in Transformer-like models generates $3C^2HW$ intermediate states, and the $softmax(QK^T/\sqrt{d_k})$ takes intermediate states as many as $2(HW)^2C/Patch\_area$, where $H$, $W$and $C$ denote the height, width, and channels of the input.}
	Due such a huge amount of data movement across intermediate states, conventional Transformer-like models usually suffer from excessive memory consumption.
	In the training stage, all the data in intermediate states must be saved for the backpropagation, leading considerable memory costs and design limits of model architecture volumes or batch tuning flexibility.
	In the inference stage, frequent and continuous generation and release of intermediate states during the forward propagation also cast inconsistency and interval of memory consumption in time flow.
\begin{comment}
	% When mapping to hardware, ViT suffers from excessive memory consumption.
	% This leads to a lot of memory usage on the accelerators (i.e. GPU), which limits the depth of trainable networks on accelerators or the batch size during training.
	% In the inference stage, \JX{please explain}\CX{the continuous generation and release of intermediate states causes} inconsistency and interval of memory consumption in time flow, which limits the parallelizability \CX{(depends on the moment that intermediate state occupies the most memory)} of models and sufficient usage of the computation resources.
\end{comment}


\textbf{\textit{(2) Computation Cost with Data Dependency:}}
In addition to the memory consumption, the complex computing logistic in self-attention also introduces considerable costs.
	For example, the computation of g$^n$Conv in HorNet makes use of a recursive design to achieve higher-order spatial interactions.
	\GR{Although its \TD{channel} increasing design limits the FLOPs to an acceptable range, the recursive design brings a strong data dependency.
	% 这里channel的用法跟上面接不上。我不确认channel这个词是对的。总之我改到这里，channel这个词在我脑海里没啥感觉。
	When mapping to hardware, there exists a insufficient utilization of computation units in the g$^n$Conv operator due to the mandatory synchronization caused by the data dependencies.}
	% 这一段话，写的也不清楚，问题跟上面的差不多，就只是一些general 的描述。不太清楚到底是多少。

Such excessive intermediate states and data dependency bring new opportunities and challenges to design a novel efficient high-order interactive neural network.
	In this work, we will show that, quadratic neuron can play an important role.

\begin{figure}
	\centerline{\includegraphics[width=3.5in]{quadratic_perceptron_1}}
	\caption{XOR Representation Capability of Different Neurons \newline(Different colors reprensts xxx, dots and crosses are xxx)}
	%A perceptron with single quadratic neuron can solve a generalized XOR problem.}
	\label{fig:perceptron}
	\vspace{-3.4mm}
\end{figure}



\subsection{\textbf{\TD{Quadratic Neuron}}}

\textbf{Neural Format:}
In contrast to the conventional neuron represented by a inner product of weight vector $W \in \mathbb{R}^{1 \times n}$ and input vector $\mathbf{x} \in \mathbb{R}^{n \times 1}$ plus a bias $b$ and an activation, the quadratic neuron can be written by an quadratic polynomial of input $\mathbf{x}$:
	\begin{equation}
		y = \mathbf{x}^TW_q\mathbf{x} + W_c\mathbf{x} + b,
		\label{equ:quadratic_neuron}
	\end{equation}
where $W_q \in \mathbf{R}^{n \times n}$ denotes a quadratic term weight and $W_c \in \mathbf{R}^{1 \times n}$ denotes a linear term weight.

While the linear term promise a non-weaker learning ability than conventional CNNs, since the quadratic neuron includes a conventional neural network.
	Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, and thus rise the potential high-order interaction to mandatory, causing a performance deduction.
\begin{comment}
	%Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, and thus it will rise the dimension interaction in data to a mandatory high-order format.
	%Since the high-order interaction among dimension is potential, rise it to a mandatory high-order format will miss the.
\end{comment}



\textbf{Design Motivation:}
To avoid huge memory consumption caused by a $O(n^2)$ intermediate state space and data dependency caused by high-order interactive neural network architecture design, we try to reduce the granularity of high-order computation from the level of network architectures to the level of neurons.

A quadratic neuron brings more opportunities to discover nonlinear relations among data dimensions, because it performs a high-order interaction within the neuron for its quadratic computation.
	Therefore, with a shallower network, a quadratic neural network can learn a smoother and richer nonlinear representation than conventional neural networks.
	Fig.~\ref{fig:perceptron} shows that for a generalized XOR classification problem, a single layer perceptron with a quadratic neuron can solve it alone, and gives even a more clear classification boundary than a two-layer perceptron with 10 hidden neurons.

When embedding quadratic neurons into a network architecture that is well optimized for computation flow, we will no longer suffer from the computational bottleneck caused by network design, while performing high-order interaction.


\textbf{Neuron Design Challenges:}
\FN{Although embedding high-order interactions into neuron-level, conventional quadratic neurons also generate a quadratic parameter space ($w_q$).}
	\TD{Therefore, an inappropriate implementation of quadratic neural networks would still cause certain computing issues.}
	% 到底是个什么parameter space？这个问题其实非常重要，而不是一句话打法了。因为他是你后面设计的motivation。
	\FN{In this work, we will carefully examine the quadratic neural network from neuron to structural blocks and eventually to the overall model design to comprehensively optimize the parameter space dilation issue whiling maintaining quadratic neurons with powerful high-order neural interaction ability.}
	% The optimization of quadratic neural network's computation will thus be a challenge.
	% Luckily, there is still room for improvement in the design of quadratic neurons.




\subsection{\textbf{Hardware-aware Neural Architecture Search}}
\FN{Neural Architecture Search (NAS) has been extensively used in the computer vision tasks during past few years.
	% Although NAS has achieved a huge success in finding high-performance neural networks, directly deploying NAS-synthesized complex neural architecture in resource-limited mobile devices is infeasible.
	Particularly, hardware-aware NAS considers system execution latency, memory footprint, or energy footprint as one of the optimization objectives in algorithms, and thus synthesizing a model that is well balanced between cognition and computing performance.}

\FN{Earlier on, few attention from NAS area is given to high-order interactive neural networks due to complex search space and large evaluation cost.
	Only very recently, the popularity of Transformer-like modleds triggered some works to build a NAS synthesized ViT~\cite{gong2021nasvit,chen2021glit}.
	However, even these works only focused on the cognition performance without considering hardware awareness, not to mention the breakthrough to high-order neuron designs.}

\FN{In this work, we target to endorse hardware-awareness into the proposed \textit{QuadraNet} and expand its generalization capability.
	Therefore, we will incorporate mature NAS techniques into our design methodology to search adaptive high-order interactive neural network architecture for various deployment scenarios.}


==> _hist/2-Background_v6-XC-CX.tex <==
\section{\textbf{Motivation Analysis}}

\subsection{\textbf{High-Order Interactive Neural Networks}}

\textbf{Existing Approaches:}
To capture high-order neural interactions, Transformer-like neural network models, such as ViT~\cite{dosovitskiy2020image} and its variants~\cite{liu2021swin,chu2021twins}, adopt the self-attention mechanism as aforementioned.
	During model cognition, self-attention performs spatial mixing computation $y_{SA}^{(i,c)}$ of the $c^{th}$ output channel at the $i^{th}$ feature dimension:
	\begin{equation}
		y_{Self-Attention}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^CA(x)_{i\rightarrow j}W_V^{(c',c)}x^{(j,c')},
		\label{equ:self}
	\end{equation}
where $\Omega_i$ is the attention receptive field involving interactive neurons,
%where $\Omega_i$ is the receptive field as instantiated to the attention window,
$A(x)$ is the input-adaptive weight matrix calculated by a softmax dot-production of ``query'' ($Q$) and ``key'' ($K$) transformations of the input $x$, and $i$~$\rightarrow$~$j$ process denotes the relative position of the $i^{th}$ and $j^{th}$ feature dimension.
	Meanwhile, self-attention achieves channel-wise information transformation through its ``value'' ($V$) transformation of $W_V$ on $x^{(j,c')}$, and $(c',c)$ denotes the information transformation as manifested from the $c'^{th}$ input channel to the $c^{th}$ output channel.
	As aforementioned, the multiplication $A(x)$ and $x$ forms high-order neural interactions and thus expected cognition performance.

\begin{comment}
	% where  $\Omega_i$ is \JX{ the receptive field as} instantiated to the attention window, $A(x)$ \CX{is the input-adaptive weight matrix} calculated by a softmax dot-product of Query and Key transformations of input $x$, \CX{and $i\rightarrow j$ denotes the relative position of location $i$ and $j$}.
	%Self-attention \JX{performs} channel-wise information \JX{interaction}\sout{transportation} through \JX{its} Value transformation \JX{of} $W_V$ \JX{on $x^{(j,c')}$}, and $(c',c)$ denotes the information \JX{interaction as manifested}\sout{transportation} from input channel $c'$ to output channel $c$.
	%As aforementioned, the multiplication of input-dependent weights $A(x)$ and input $x$ generates a high-order interaction.
\end{comment}
\begin{comment}
	%In the past decade, researchers found the effectiveness of attention mechanism. The attention mechanism uses the data itself to generate a set of parameters, and then multiply them with the data itself or their transformation. So no matter what kinds of attention (spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self attention \cite{dosovitskiy2020image}) used, it can be formulated in a high-order computation:
	%This formulation that unifies with Equation \ref{equ:highorder} indicates self-attention is substantially a high-order interaction computation.
\end{comment}

Different from the self-attention approach shown in Eq.~\ref{equ:self}, HorNet~\cite{rao2022hornet} performs high-order neural interactions with a gated recursive convolution --- \textit{g$^r$Conv}, which can be formulated as:
	% Specifically, HorNet proposes a g$^r$Conv operation to perform high-order interaction computation. The output of g$^r$Conv can be formulated as:
\begin{equation}
	\hspace{-3mm}y_{g^nConv}^{(i,c)}=p_r^{(i,c)}=\sum_{j \in \Omega_i}\sum_{c'=1}^Cg(p_{r-1})w_{r-1,i\rightarrow j}^cW_{\phi_{in}}^{(c',c)}x^{(j,c')}.
	\label{equ:gnconv}
\end{equation}
Instead of generating high-order interactions directly from the input $x$, \textit{g$^r$Conv} uses a channel increasing recursive formulation $g(p_{r-1})$ to perform a high-order iteration of feature information, and thus getting an input-adaptive weight matrix. $W_{\phi_{in}}^{(c',c)}$ is an input projection.





\textbf{Higher-Order Neural Interaction:}
Summarizing the above works, we find that both approaches adopt an input-dependent weight matrix and channel-wise information transformation.
	It can be formulated as a generic high-order neural interaction mechanism:
\begin{equation}
	y_{high-order}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(x)_{ij}W^{(c',c)}x^{(j,c')},
	\label{equ:highorder}
\end{equation}
where $\Omega_i$ denotes the mechanism's receptive field, $g(x)$ denotes an interactive weight matrix that contains the input's information, $W^{(c',c)}$ denotes a channel-wise information transformation.
	The multiplication of $x$ and input-adaptive $g(x)$ forms the high-order neural interaction of data itself.
	Such an interaction represents leveraging the superposition of information between different feature dimensions.

\begin{comment}
	% As aforementioned, the computing mechanism of neural networks has evolved from low-density convolution into high-density attention-like mechanisms.
	% (e.g., spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self-attention \cite{dosovitskiy2020image})
	% These mechanisms could be formulated as follows:
	% \begin{equation}
		% Attention(x) = f(g(x),x),
	%\end{equation}
	%where $x$ denotes input data and $g(x)$ generate an input-adaptive weight, and compute the final output with rule $f(\cdot,\cdot)$.
	%\sout{These mechanisms can be generalized into an uniform high-order interaction formulation as:}
	%In such a formulation, usually, a high-order neural interaction can be observed as multiplication of data with itself or its transformation.
\end{comment}



\subsection{\textbf{High-Order Computation Problems}}
The computation of existing high-order interaction approaches (esp., self-attention) face multiple problems in terms of memory consumption and computing cost.

\textbf{Memory Consumption with Intermediate States:}
Conventional Transformer-like models usually suffer from excessive memory consumption:
	in the training stage, all the data in intermediate states must be saved for backpropagations;
	in the inference stage, frequent and continuous generation and release of intermediate states during forward propagations also cast inconsistency and interval of memory consumption in runtime.
	Such consumption significantly restricts model architecture design flexibility and optimization feasibility.

As aforementioned, those intermediate states are introduced by self-attention generation.
	Specifically, the transformation process of $Q$, $K$, and $V$ parameters in Transformer-like models generates 3$HWC$ intermediate states, and the $softmax$($QK^T$)$V$ takes intermediate states as many as ($HW$)$^2$+($HW$)$^2C$, where $H$, $W$ and $C$ denote the height, width, and channels of the input per layer, respectively.
	Compared with widely-used depthwise separable convolution, which generates only $HWC$ intermediate states, self-attention needs ($HW$+3)$\times$ more to finish its computation.
	Even if the attention space is restricted to a local receptive field as shown in~\cite{liu2021swin}, the self-attention computation still yields ($M^2$+3)$\times$ more intermediate states, where $M$ denotes the field size (usually $\geq$7~\cite{liu2021swin}).
\begin{comment}
	% When mapping to hardware, ViT suffers from excessive memory consumption.
	% This leads to a lot of memory usage on the accelerators (i.e. GPU), which limits the depth of trainable networks on accelerators or the batch size during training.
	% In the inference stage, \JX{please explain}\CX{the continuous generation and release of intermediate states causes} inconsistency and interval of memory consumption in time flow, which limits the parallelizability \CX{(depends on the moment that intermediate state occupies the most memory)} of models and sufficient usage of the computation resources.
\end{comment}



\textbf{Computing Cost with Data Dependency:}
In addition to memory consumption, the complex computing flow in self-attention also introduces considerable cost.
	For example, the computation of \textit{g$^r$Conv} in HorNet makes use of recursive convolutions to achieve higher-order neural interactions, as aforementioned.
	% before it can proceed, in other words, $n$ times interactions means $n$ times synchronizations.
	Although such ingenious design limits the FLOPs to an acceptable range, the recursive logic brings considerable data dependency issues.
	In other words, the next order of neural interactions in \textit{g$^r$Conv} must wait for the previous order of interactions to complete.
	Therefore, a series of convolution operators are forced to be serialized, which largely compromises the computing parallelism performance and exacerbates computing latency, especially with GPUs.

Although such excessive intermediate states and data dependency bring new challenges to high-order interactive neural networks, the above motivation analysis also demystifies the core cognition mechanism of Transformer-like models and the computation problems.
	To achieve a revolutionary design with both cognition and computation performance in this work, we will show that quadratic neurons can play an important role.

\begin{figure}
	\centerline{\includegraphics[width=3.3in]{quadratic_perceptron_1}}
	\caption{\TD{XOR Representation Capability of Different Neurons \newline(Different colors represents xxx, dots and crosses are xxx)}}
	%A perceptron with single quadratic neuron can solve a generalized XOR problem.}
	\label{fig:perceptron}
	\vspace{-3.5mm}
\end{figure}




\subsection{\textbf{Quadratic Neuron}}
A quadratic neuron brings more opportunities to discover nonlinear relations among data dimensions because it performs a high-order interaction within the neuron for its quadratic computation.
	Therefore, with a shallower network, a quadratic neural network can learn a smoother and richer nonlinear representation than conventional neural networks.
	For example, for a generalized XOR classification problem, as shown in Fig.~\ref{fig:perceptron}, a single-layer perceptron with a quadratic neuron can solve it alone and gives even clearer classification boundaries than a two-layer perceptron with ten hidden neurons.

\begin{figure*}[ht!]
	\centerline{\includegraphics[width = 7 in]{_fig/QuadraNet_3.pdf}}
	\caption{A bottom-up overview of QuadraNet, from neuron-level to system implementation-level.}
	\label{fig:QuadraNet}
\end{figure*}

\textbf{Neuron Format:}
In contrast to the conventional neuron represented by an inner product of input vector  $\mathbf{x} \in \mathbb{R}^{n \times 1}$ and weight vector $W \in \mathbb{R}^{1 \times n}$ plus a bias $b$ and activation, the quadratic neuron can be written as a quadratic polynomial of input $\mathbf{x}$ in the formulation:
	\begin{equation}
		\mathbf{y} = \mathbf{x}^TW_q\mathbf{x} + W_c\mathbf{x} + b,
		\label{equ:quadratic_neuron}
	\end{equation}
where $W_q$ and $W_c$ denote the quadratic- and linear-term weights, respectively.
	In Eq.~\ref{equ:quadratic_neuron}, $\mathbf{x}^TW_q$ can be regarded as an input-dependent weight of $\mathbf{x}$; thus, it is evident that high-order interaction is directly embedded in a quadratic neuron~\cite{mantini2021cqnn,bu2021quadratic}.
	This refines the granularity of high-order neural interactions and corresponding computation to the neural level, resulting in a more generic model architecture-agnostic generality.
	Therefore, we can leverage the neural-level high-order interaction as described in Eq.~\ref{equ:quadratic_neuron} to build high-order interactive neural networks with the mechanism in Eq.~\ref{equ:highorder}.

\begin{comment}
	% \CX{\sout{While}} The linear term promise a non-weaker learning ability than a conventional neural network, since it is included in the quadratic neural network.
	% Some previous works~\cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, and thus rise the potential high-order interaction to mandatory, causing a performance deduction.
\end{comment}
\begin{comment}
	%Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, and thus it will rise the dimension interaction in data to a mandatory high-order format.
	%Since the high-order interaction among dimension is potential, rise it to a mandatory high-order format will miss the.
\end{comment}


\textbf{Opportunities and Challenges:}
\begin{comment}
	% \TD{\sout{To avoid huge memory consumption caused by a large intermediate state space and data dependency caused by high-order interactive neural network architecture design, we try to reduce the granularity of high-order interaction computation from the level of network architectures to the level of neurons. Interaction within the quadratic neuron makes it possible. When embedding quadratic neurons into a network architecture that is well optimized for computation flow, we will no longer suffer from the computational bottleneck caused by network design, while performing high-order neural interaction.}}
	%\CX{Quadratic neuron provides a good opportunity to address both aforementioned high-order computation problems. Due to quadratic neuron's architecture-agnostic generality, %combining it with an efficient but effective, a combination of the quadratic neuron and network architecture that is well optimized for computation flow (i.e. Convolution) will avoid both lots of intermediate states and strong data dependency, while forming high-order neural interactive neural networks as Eq.\ref{equ:highorder} with outstanding cognition performance.
\end{comment}
Although embedding high-order interactions into the neuron level, ordinary quadratic neurons also generate a quadratic parameter space as large as ($W_q \in \mathbb{R}^{n\times n}$), its parameter volume rises to $O(n^2+n)$ compared with $O(n)$ with conventional neuron-based model implementations, since we now get an extra quadratic term weight matrix with $n^2$ learnable parameters.
	Therefore, an inappropriate implementation of quadratic neural networks would still cause certain computing issues, such as a significant parameter space dilation and thus an increase in the amount of computation.
	% 到底是个什么parameter space？这个问题其实非常重要，而不是一句话打法了。因为他是你后面设计的motivation。

In this work, we carefully examine the quadratic neural network from neuron to structural blocks and eventually to the overall model design to comprehensively optimize the parameter space dilation issue while maintaining quadratic neurons with powerful high-order neural interaction ability.
	% The optimization of quadratic neural network's computation will thus be a challenge.
	% Luckily, there is still room for improvement in the design of quadratic neurons.




\subsection{\textbf{Hardware-aware Neural Architecture Search}}
Neural Architecture Search (NAS) has been extensively used in neural network design and optimization.
	% Although NAS has achieved a huge success in finding high-performance neural networks, directly deploying NAS-synthesized complex neural architecture in resource-limited mobile devices is infeasible.
	Particularly, hardware-aware NAS considers computing cost, memory consumption, runtime latency, or energy footprint as one of the optimization objectives in algorithms, thus synthesizing a model that is well-balanced between cognition and computation performance.

Earlier on, little attention from the NAS area is given to high-order interactive neural networks due to complex search space and large evaluation cost.
	Only very recently, the popularity of Transformer-like models triggered some works to build a NAS synthesized ViT~\cite{gong2021nasvit,chen2021glit}.
	However, even these works only focused on cognition performance without considering hardware awareness, not to mention the breakthrough to high-order neuron designs.

In this work, we target to endorse hardware awareness into the proposed \textit{QuadraNet} and expand its generalization capability.
	Therefore, we will incorporate mature NAS techniques into our design methodology to search adaptive high-order interactive neural network architecture for various deployment scenarios.


==> _hist/2-Background_v6-XC.tex <==
\section{\textbf{Motivation Analysis}}

\subsection{\textbf{High-Order Interactive Neural Networks}}

\textbf{Existing Approaches:}
To capture high-order neural interactions, Transformer-like neural network models, such as ViT~\cite{dosovitskiy2020image} and its variants~\cite{liu2021swin,chu2021twins}, adopt the self-attention mechanism as aforementioned.
	During model cognition, self-attention performs spatial mixing computation $y_{SA}^{(i,c)}$ of the $c^{th}$ output channel at the $i^{th}$ feature dimension:
	\begin{equation}
		y_{Self-Attention}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^CA(x)_{i\rightarrow j}W_V^{(c',c)}x^{(j,c')},
		\label{equ:self}
	\end{equation}
where $\Omega_i$ is the attention receptive field involving interactive neurons,
%where $\Omega_i$ is the receptive field as instantiated to the attention window,
$A(x)$ is the input-adaptive weight set calculated by a softmax dot-production of ``query'' ($Q$) and ``key'' ($K$) transformations of the input $x$, and $i$~$\rightarrow$~$j$ process denotes the relative position of the $i^{th}$ and $j^{th}$ feature dimension.
	Therefore, self-attention achieves channel-wise information transformation through its ``value'' ($V$) transformation of $W_V$ on $x^{(j,c')}$, and $(c',c)$ denotes the information transformation as manifested from the $c'^{th}$ input channel to the $c^{th}$ output channel.
	As aforementioned, the multiplication $A(x)$ and $x$ forms high-order neural interactions and thus expected cognition performance.

\begin{comment}
	% where  $\Omega_i$ is \JX{ the receptive field as} instantiated to the attention window, $A(x)$ \CX{is the input-adaptive weight matrix} calculated by a softmax dot-product of Query and Key transformations of input $x$, \CX{and $i\rightarrow j$ denotes the relative position of location $i$ and $j$}.
	%Self-attention \JX{performs} channel-wise information \JX{interaction}\sout{transportation} through \JX{its} Value transformation \JX{of} $W_V$ \JX{on $x^{(j,c')}$}, and $(c',c)$ denotes the information \JX{interaction as manifested}\sout{transportation} from input channel $c'$ to output channel $c$.
	%As aforementioned, the multiplication of input-dependent weights $A(x)$ and input $x$ generates a high-order interaction.
\end{comment}
\begin{comment}
	%In the past decade, researchers found the effectiveness of attention mechanism. The attention mechanism uses the data itself to generate a set of parameters, and then multiply them with the data itself or their transformation. So no matter what kinds of attention (spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self attention \cite{dosovitskiy2020image}) used, it can be formulated in a high-order computation:
	%This formulation that unifies with Equation \ref{equ:highorder} indicates self-attention is substantially a high-order interaction computation.
\end{comment}

Different from the self-attention approach shown in Eq.~\ref{equ:self}, HorNet~\cite{rao2022hornet} performs high-order neural interactions with a recursive convolution --- \textit{g$^n$Conv}, which can be formulated as:
	% Specifically, HorNet proposes a g$^n$Conv operation to perform high-order interaction computation. The output of g$^n$Conv can be formulated as:
\begin{equation}
	\hspace{-3mm}y_{g^nConv}^{(i,c)}=p_n^{(i,c)}=\sum_{j \in \Omega_i}\sum_{c'=1}^Cg(p_{n-1})w_{n-1,i\rightarrow j}^cW_{\phi_{in}}^{(c',c)}x^{(j,c')}.
	\label{equ:gnconv}
\end{equation}
Instead of generating high-order interactions directly from the input $x$, \textit{g$^n$Conv} uses a channel increasingly recursive formulation $g(p_{n-1})$ to perform high-order iteration of feature information, and therefore getting an input-adaptive weight set. $W_{\phi_{in}}^{(c',c)}$ is an input projection.





\textbf{Higher-Order Neural Interaction:}
Summarizing the above works, we find that both approaches adopt an input-dependent weight set based on a channel-wise information transformation.
	It can be formulated as a generic high-order neural interaction mechanism:
\begin{equation}
	y_{high-order}^{(i,c)} = \sum_{j \in \Omega_i}\sum_{c'=1}^Cg(x)_{ij}W^{(c',c)}x^{(j,c')},
	\label{equ:highorder}
\end{equation}
where $\Omega_i$ denotes the mechanism's receptive field, $g(x)$ denotes an interactive weight set that contains the input's information, $W^{(c',c)}$ denotes a channel-wise information transformation.
	And the multiplication of $x$ and input-adaptive $g(x)$ forms the high-order neural interaction of data itself.
	Such an interaction represents leveraging the superposition of information between different feature dimensions.

\begin{comment}
	% As aforementioned, the computing mechanism of neural networks has evolved from low-density convolution into high-density attention-like mechanisms.
	% (e.g., spatial \cite{zhu2019empirical}, channel \cite{hu2018squeeze}, or self-attention \cite{dosovitskiy2020image})
	% These mechanisms could be formulated as follows:
	% \begin{equation}
		% Attention(x) = f(g(x),x),
	%\end{equation}
	%where $x$ denotes input data and $g(x)$ generate an input-adaptive weight, and compute the final output with rule $f(\cdot,\cdot)$.
	%\sout{These mechanisms can be generalized into an uniform high-order interaction formulation as:}
	%In such a formulation, usually, a high-order neural interaction can be observed as multiplication of data with itself or its transformation.
\end{comment}



\subsection{\textbf{High-Order Computation Problems}}
The computation of existing high-order interaction approaches (esp., self-attention) face multiple problems in terms of memory consumption and computing cost.

\textbf{Memory Consumption with Intermediate States:}
Conventional Transformer-like models usually suffer from excessive memory consumption:
	in the training stage, all the data in intermediate states must be saved for backpropagations;
	in the inference stage, frequent and continuous generation and release of intermediate states during forward propagations also cast inconsistency and interval of memory consumption in runtime.
	Such consumption significantly restricts model architecture design flexibility and optimization feasibility.

As aforementioned, those intermediate states are introduced by self-attention generation.
	Specifically, the transformation process of $Q$, $K$, and $V$ parameters in Transformer-like models generates 3$HWC$ intermediate states, and the $softmax$($QK^T$)$V$ takes intermediate states as many as ($HW$)$^2$+($HW$)$^2C$, where $H$, $W$ and $C$ denote the height, width, and channels of the input in this layer, respectively.
	Compared with widely-used depthwise separable convolution, which generates only $HWC$ intermediate states, self-attention needs ($HW$+3)$\times$ more to finish its computation.
	Even if the attention space is restricted to a local receptive field as shown in~\cite{liu2021swin}, the self-attention computation still yields ($M^2$+3)$\times$ more intermediate states, where $M$ denotes the field size (usually $\geq$7~\cite{liu2021swin}).
\begin{comment}
	% When mapping to hardware, ViT suffers from excessive memory consumption.
	% This leads to a lot of memory usage on the accelerators (i.e. GPU), which limits the depth of trainable networks on accelerators or the batch size during training.
	% In the inference stage, \JX{please explain}\CX{the continuous generation and release of intermediate states causes} inconsistency and interval of memory consumption in time flow, which limits the parallelizability \CX{(depends on the moment that intermediate state occupies the most memory)} of models and sufficient usage of the computation resources.
\end{comment}



\textbf{Computing Cost with Data Dependency:}
In addition to memory consumption, the complex computing flow in self-attention also introduces considerable cost.
	For example, the computation of \textit{g$^n$Conv} in HorNet makes use of recursive convolutions to achieve higher-order neural interactions as aforementioned.
	% before it can proceed, in other words, $n$ times interactions means $n$ times synchronizations.
	Although such ingenious design limits the FLOPs to an acceptable range, the recursive logic brings considerable data dependency issues.
	In other words, the next order of neural interactions in \textit{g$^n$Conv} must wait for the previous order of interactions to complete.
	Therefore, a series of convolution operators are forced to be serialized, which largely compromises the computing parallelism performance and exacerbates computing latency, especially with GPUs.

Although such excessive intermediate states and data dependency bring new challenges to high-order interactive neural networks, the above motivation analysis also demystify the core cognition mechanism of Transformer-like models and the computation problems.
	To achieve revolutionary design with both cognition and computation performance in this work, we will show that, quadratic neuron can play an important role.

\begin{figure}
	\centerline{\includegraphics[width=3.3in]{quadratic_perceptron_1}}
	\caption{XOR Representation Capability of Different Neurons \newline(Different colors reprensts xxx, dots and crosses are xxx)}
	%A perceptron with single quadratic neuron can solve a generalized XOR problem.}
	\label{fig:perceptron}
	\vspace{-3.5mm}
\end{figure}




\subsection{\textbf{Quadratic Neuron}}
A quadratic neuron brings more opportunities to discover nonlinear relations among data dimensions, because it performs a high-order interaction within the neuron for its quadratic computation.
	Therefore, with a shallower network, a quadratic neural network can learn a smoother and richer nonlinear representation than conventional neural networks.
	For example, for a generalized XOR classification problem as shown in Fig.~\ref{fig:perceptron}, a single layer perceptron with a quadratic neuron can solve it alone, and gives even clearer classification boundaries than a two-layer perceptron with 10 hidden neurons.


\textbf{Neuron Format:}
In contrast to the conventional neuron represented by an inner product of weight vector $W \in \mathbb{R}^{1 \times n}$ and input vector $\mathbf{x} \in \mathbb{R}^{n \times 1}$ plus a bias $b$ and an activation, the quadratic neuron can be written as a quadratic polynomial of input $\mathbf{x}$ in formulation:
	\begin{equation}
		\mathbf{y} = \mathbf{x}^TW_q\mathbf{x} + W_c\mathbf{x} + b,
		\label{equ:quadratic_neuron}
	\end{equation}
where $W_q$ and $W_c$ denote the quadratic- and linear-term weights, respectively.
	In Eq.~\ref{equ:quadratic_neuron}, $\mathbf{x}^TW_q$ can be regarded as an input-dependent weight of $\mathbf{x}$; thus, it is evident that high-order interaction is directly embedded in a quadratic neuron~\cite{mantini2021cqnn,bu2021quadratic}.
	This will therefore refines the granularity of high-order neural interactions and corresponding computation to the neural-level, resulting in a more generic model architecture-agnostic generability.

\begin{comment}
	% \CX{\sout{While}} The linear term promise a non-weaker learning ability than a conventional neural network, since it is included in the quadratic neural network.
	% Some previous works~\cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, and thus rise the potential high-order interaction to mandatory, causing a performance deduction.
\end{comment}
\begin{comment}
	%Some previous works \cite{mantini2021cqnn,bu2021quadratic} get rid of the linear term of a quadratic polynomial, and thus it will rise the dimension interaction in data to a mandatory high-order format.
	%Since the high-order interaction among dimension is potential, rise it to a mandatory high-order format will miss the.
\end{comment}


\textbf{Opportunities and Challenges:}
\TD{To avoid huge memory consumption caused by a large intermediate state space and data dependency caused by high-order interactive neural network architecture design, we try to reduce the granularity of high-order interaction computation from the level of network architectures to the level of neurons. Interaction within the quadratic neuron makes it possible. When embedding quadratic neurons into a network architecture that is well optimized for computation flow, we will no longer suffer from the computational bottleneck caused by network design, while performing high-order neural interaction.}


\FN{Although embedding high-order interactions into neuron-level, conventional quadratic neurons also generate a quadratic parameter space ($W_q \in \mathbb{R}^{n\times n}$)}\CX{, which means we now have $n^2$, instead of $n$ in conventional neuron, learnable parameters need updating.}
	\TD{Therefore, an inappropriate implementation of quadratic neural networks would still cause certain computing issues.}
	% 到底是个什么parameter space？这个问题其实非常重要，而不是一句话打法了。因为他是你后面设计的motivation。
	\FN{In this work, we will carefully examine the quadratic neural network from neuron to structural blocks and eventually to the overall model design to comprehensively optimize the parameter space dilation issue whiling maintaining quadratic neurons with powerful high-order neural interaction ability.}
	% The optimization of quadratic neural network's computation will thus be a challenge.
	% Luckily, there is still room for improvement in the design of quadratic neurons.




\subsection{\textbf{Hardware-aware Neural Architecture Search}}
Neural Architecture Search (NAS) has been extensively used in the computer vision tasks during past few years.
	% Although NAS has achieved a huge success in finding high-performance neural networks, directly deploying NAS-synthesized complex neural architecture in resource-limited mobile devices is infeasible.
	Particularly, hardware-aware NAS considers computing cost, memory consumption, runtime latency, or energy footprint as one of the optimization objectives in algorithms, and thus synthesizing a model that is well balanced between cognition and computation performance.

Earlier on, few attention from NAS area is given to high-order interactive neural networks due to complex search space and large evaluation cost.
	Only very recently, the popularity of Transformer-like modleds triggered some works to build a NAS synthesized ViT~\cite{gong2021nasvit,chen2021glit}.
	However, even these works only focused on the cognition performance without considering hardware awareness, not to mention the breakthrough to high-order neuron designs.

In this work, we target to endorse hardware-awareness into the proposed \textit{QuadraNet} and expand its generalization capability.
	Therefore, we will incorporate mature NAS techniques into our design methodology to search adaptive high-order interactive neural network architecture for various deployment scenarios.


==> _hist/3-1-Method_Overview_v1.tex <==
\section{\textbf{\textit{QuadraNet} Design Methodology}}
\subsection{\textbf{Overview}}
\begin{figure*}
    \centerline{\includegraphics[width = 7 in]{_fig/QuadraNet_4.pdf}}
    \caption{A bottom-up overview of QuadraNet, from neuron-level to system implementation-level.}
    \label{fig:QuadraNet}
\end{figure*}
\begin{comment}
Figure \ref{fig:QuadraNet} illustrates the overview of our proposed model.     From a bottom-up perspective, it is composed of five components: (a) efficient low rank quadratic neuron, (b) mapping quadratic neuron to convolution, (c) Quadratic Neural Block Design, (d) QuadraNet architecture, (e) Hardware-aware quadratic neural architecture search. 
    To be specific: 
        (a) provides a factorization of quadratic term weights, reduce the computation complexity and parameters space of quadratic term.
        In (b) quadratic convolution, (a) quadratic neurons are mapped to hardware-optimized convolution operators. 
        Using optimized (b) high-order quadratic convolution, a powerful (c) Quadratic network block is built to leverage the (a) quadratic neuron's high-order information superposition. 
        Using similar pyramid macroscopical network architecture and (c) QuadraBlock, QuadraNet achieves competitive performance while solving the computation bottleneck of high-order interactive neural networks. 
        To make hardware specific optimization, (d) QuadraNet defines a search space for (e) HW-NAS.
    In the following section, we will introduce these components in detail.
\end{comment}   

Figure \ref{fig:QuadraNet} illustrates the overview of our proposed model. (a) Efficient quadratic neuron gives a solution to the aforementioned neuron design challenge by a factorization of quadratic term.
    And then it is mapped into (b) quadratic convolution to build high-order interaction while avoiding $O(n^2)$ intermediate state space and recursive computation, and therefore provides an optimization on memory consumption and data dependency. (Section. III.B)
    
Leveraging efficient high-order interaction provide by (b) and the computational and representative properties of modern neural blocks, we design (c) QuadraBlock to improve the computational efficiency while maintain a high representation capacity of quadratic neuron. 
    Based on (c), we manually design (d) QuadraNet to achieve competitive performance with state-of-the-art while improve inference throughput, and utilize (e)HW-NAS to find hardware-aware efficient quadratic neural architecture. (Section. III.C)


==> _hist/3-1-Method_Overview_v2-XC.tex <==
\section{\textbf{\textit{QuadraNet} Design Methodology}}
\subsection{\textbf{Design Methodology Overview}}

Fig.~\ref{fig:QuadraNet} illustrates the overview of our proposed methodology, which consists following major tasks:

(a) An novel computing-friendly \textit{quadratic neuron} design is proposed.
	With factorized low-rank quadratic terms, the parameter volumes and corresponding workload could be significant optimized in the neuron level first.

(b) Based on quadratic neurons, a \textit{quadratic convolution} mechanism is built for high-order neural interactions.
	Different from conventional approaches (e.g., $g^rConv$), this mechanism could avoid large amount of intermediate state spaces and recursive data dependency, further retaining the computation complexity.

(c) \textit{QuadraBlock} is designed as the basic high-order neural network structural module.
	\textit{QuadraBlock} achieves high-order spatial interaction with quadratic depthwise convolution, and effectively unify quadratic neurons with elastic receptive fields for optimal cognition.

(d) A comprehensive high-order neural network architecture \textit{QuadraNet} integrates the proposed techniques above and leads a design revolution for Transformer-like models with outstanding cognition and computation performance.

(e) Hardware-aware NAS is further incorporated to improve the architecture generalization capability of \textit{QuadraNet} and therefore the adaptability to various hardware computing constraints.


==> _hist/3-2-Method_Part1_v1-XC.tex <==
\subsection{\textbf{Efficient Quadratic Neuron and Convolution Design}}

\textbf{Quadratic Neuron:}
	% We first solve the neuron design challenge by an efficient quadratic neuron.
As defined in Eq.~(\ref{equ:quadratic_neuron}), the quadratic term of a conventional quadratic neuron has a $n^2$ complexity in the parameter space, which limits its usage in terms of both algorithmic complexity and implementation difficulty.
	%To avoid huge computing workload and memory cost of conventional quadratic neuron, as illustrated in Fig.~\ref{fig:QuadraNet} (a), in stead of using a full rank quadratic weight matrix $W_q$, we build weight matrix with two n-dimensional vectors $W_a, W_b \in \mathbb{R}^{1\times n}$, which can been seen as a low rank factorization of the quadratic term weight matrix.
To address this issue, instead of using a full-rank quadratic weight matrix $W_q$, we propose to build the weight vectors $W_a$ and $W_b \in \mathbb{R}^{1\times n}$ as shown in Fig.~\ref{fig:QuadraNet} (a), which can be seen as a low-rank factorization of the quadratic term.
	Thus, the new quadratic neuron can be reformulated as:
\begin{equation}
	\mathbf{y} = \mathbf{x}^TW_a^TW_b\mathbf{x} + W_c\mathbf{x} + b\\
	=(W_a\mathbf{x})^T(W_b\mathbf{x}) + W_c\mathbf{x} + b.
	\label{equ:our_neuron}
\end{equation}

Such a factorization reduces the parameter space of quadratic neurons from $O$($n^2$+$n$) to $O(3n)$ and the computation complexity from $O$($n^2$+2$n$) to $O$(4$n$).

\textbf{High-Order Interactive Quadratic Convolution:}
Because quadratic neurons have powerful cognitive capacity and generalization ability, we can directly bring them into a simple way of information extraction.
In this work, we directly map optimized quadratic neurons to the widely-used convolution operation to achieve efficient high-order interactions.
    Specifically, we map the three groups of weights $W_a$, $W_b$, and $W_c$ from a single quadratic neuron to three convolutional filters and conduct a polynomial computation like in Eq.~\ref{equ:our_neuron}. With such a mapping, we obtain a quadratic convolution.
Considering a mostly used depthwise separable convolution, the computation of $i^{th}$ position of channel $c$ can be formulated as:
\begin{equation}
    \begin{aligned}
        y_{Quad}^{(i,c)} &=\sum_{j,k \in \Omega_i} \sum_{c'=1}^C(\omega_{a,i\rightarrow j}T_{a}^{(c,c')}x^{(j,c')})(\omega_{b,i\rightarrow k}T_{b}^{(c,c')}x^{(k,c')})\\
        &=\sum_{j \in \Omega_i}\sum_{c'=1}^C\omega_{a,i\rightarrow j}\sum_{k \in \Omega_i}\omega_{b,i\rightarrow k}x^{(k,c')}T_{q}^{(c,c')}x^{(j,c')}\\
        &=\sum_{j \in \Omega_i}\sum_{c'=1}^Cq(x)_{ij}T_{q}^{(c,c')}x^{(j,c')},
     \end{aligned}
     \label{equ:q_conv}
\end{equation}
where $\Omega_i$ denotes the convolution receptive field in the $i^{th}$ position, and $q(x)_{ij}=\omega_{a,i\rightarrow j}\sum_{k \in \Omega_i}\omega_{b,i\rightarrow k}x^{(k,c')}$ implicates an input-adaptive weight and when multiplying $x$, it captures the high-order spatial interaction.
    Notice that Eq.~(\ref{equ:q_conv}) forms a unified  expression for high-order interaction that well matches with Eq.~(\ref{equ:highorder}).
    This indicates that the quadratic convolution can capture the high-order spatial interaction, and therefore can be seen as an approximation computation of self-attention and \textit{g$^r$Conv}.

\begin{comment}
    % \CX{\sout{Convolutional neural networks have efficient computation flow and generalization ability, and convolution operators are also fully optimized on various devices. Combining convolution with quadratic neurons can effectively use these characteristics to build efficient and powerful networks.}}
\end{comment}
\begin{comment}
    % \sout{The optimized quadratic neuron is further utilized to form high-order convolution operation.}
	% In order to build high-order spatial interaction in a vision task, we map quadratic to convolution.
	% Since we propose a neuron-level high-order interaction computation, it will be easy to map the quadratic neuron to any neural operations (i.e. convolution and FC).
	%Because of useful inductive bias (e.g., Translation equivalence) of convolution neural networks, we map the quadratic neuron to a convolution operations.
\end{comment}




\textbf{Efficient High-Order Computation:}
Through the neuron- and convolution-level design, the primary high-order quadratic computation mechanism could be determined. 
From a tensor perspective, the computing of this mechanism could be formulated as: 
\begin{equation}
    X_{out} = f_a(X_{in})\odot f_b(X_{in})+f_c(X_{in}),
    \label{equ:tensor}
\end{equation}
    where $\odot$ denotes the Hadamard product; $f_a,f_b,f_c$ denote convolution operators (with weights of $W_a$, $W_b$, $W_c$); $X_{in}$ and $X_{out}$ denote the input and output tensors, respectively.
Different from~\cite{rao2022hornet}, such a mechanism goes through a straightforward computation flow without recursive logic, and thus no aforementioned data dependency and corresponding computing costs.

As for the problem of intermediate states, we need to examine the intermediate states generated in Eq.~(\ref{equ:tensor}).
    In the forward, four intermediate states are generated --- $f_a(X_{in})$,$f_b(X_{in})$,$f_a(X_{in})\odot f_b(X_{in})$, and $f_c(X_{in})$, all of which have the same volume and 4$HWC$ intermediate states in total.
    The size of the intermediate states of the quadratic convolution will therefore be $4\times$ compared with conventional convolution (versus  ($HW$+3)$\times$ in self-attention).
\CX{
Meanwhile, in the back propagation, this $4\times$ intermediate states can be further reduced to $2\times$. Because the intermediate states $f_a(X_{in})\odot f_b(X_{in})$ and $f_c(X_{in})$ can be released.
%don't play a role in the back propagation. 
    The update of the weight $W_a$ only rely on intermediate states $f_b(X_{in})$, because the gradient of the weight $W_a^l$ can be computed by:
\begin{equation}
    \begin{aligned}
    \frac{\partial \mathscr{L}}{\partial W_a^l} = &\frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot \frac{\partial X^{l+1}}{\partial (W_a^lX^l)(W_b^lX^l)}\cdot \frac{\partial (W_a^lX^l)(W_b^lX^l)}{\partial (W_a^lX^l)} \cdot \frac{\partial (W_a^lX^l)}{\partial W_a^l}\\
    = &\frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot (W_b^lX^l)\cdot X^l,
    \end{aligned}
    \label{equ:garident}
\end{equation}
where $X^l$ denotes the output of the $l^{th}$ layer. 
Similarly, the update of the weight $W_b$ only rely on intermediate states $f_a(X_{in})$. The update of the linear term weight $W_c$ does not rely on any intermediate states. Therefore, these intermediate states can be released during forward propagation.

In a word, quadratic convolution enables more efficient higher-order computation by avoiding a recursive design that eliminates strong data dependencies and further optimizations for intermediate states.
Quadratic convolution also offers the possibility of external acceleration by simply mapping quadratic neuron to the convolution operator, allowing us to directly leverage existing compilers~\cite{chen2018tvm} and quadratic computation library~\cite{xu2022quadralib} to optimize the computation.

}

\begin{comment}


\TD{        
    % are 4 generated intermediate states to complete the forward computation, all of which have volume HWC, and totally 4HWC intermediate states.
       % What we further optimize lies in the fact that, considering back-propagation, this $4\times$ intermediate state can be further reduced during the training stage.
        When updating the $l^{th}$ layer's weights, the gradient of the weight $W_a^l$ can be computed by
\begin{equation}
    \begin{aligned}
    \frac{\partial \mathscr{L}}{\partial W_a^l} = &\frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot \frac{\partial X^{l+1}}{\partial (W_a^lX^l)(W_b^lX^l)}\cdot \frac{\partial (W_a^lX^l)(W_b^lX^l)}{\partial (W_a^lX^l)} \cdot \frac{\partial (W_a^lX^l)}{\partial W_a^l}\\
    = &\frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot (W_b^lX^l)\cdot X^l,
    \end{aligned}
    \label{equ:garident}
\end{equation}
where $X^l$ denotes the output tensor of the $l^{th}$ layer.
    That means the backpropagation of the quadratic term does not rely on intermediate state $f_a(X_{in})\odot f_b(X_{in})$. 
Also, the back-propagation of the linear term does not rely on intermediate state $f_c(X_{in})$. 
Therefore, we can implement back-propagation without saving these intermediate states, which further compress the intermediate states to $2\times$.

In a word, quadratic convolution enables more efficient higher-order computation by avoiding a recursive design that eliminates strong data dependencies and further optimizations for intermediate states.

Quadratic convolution also offers the possibility of external acceleration by simply mapping quadratic neuron to the convolution operator, allowing us to directly leverage existing compilers~\cite{chen2018tvm} and quadratic computation library~\cite{xu2022quadralib} to optimize the computation.



%Through the neuron and convolution level design, the basic high-order computation mechanism could be determined.
% From a tensor perspective, the computing could be xxxxx as Eq. 7
%Different from HorNet, this is a xxxxx 计算流程，没有recursive。

% 而针对另一个问题IS，我们需要进一步的检验Eq7的iS状态
% 包含四个状态
% 我们的优化点在于
% 最终状态是xxxx，compared to sota，特别好

% 从而我们的设计特别好。

For the two main aforementioned high-order computation problems, the strong data dependency is solved naturally because there is no recursive design in the quadratic convolution.
As for the problem of intermediate states, if we put the view on the whole tensor computation flow level, the size of the intermediate state of the quadratic convolution operation will be $4\times$ compared with conventional neural networks (versus  ($HW$+3)$\times$ in self-attention).
To be specific, given the input tensor $X_{in}$, the output of quadratic convolution can therefore be computed with:
\begin{equation}
    X_{out} = f_a(X_{in})\odot f_b(X_{in})+f_c(X_{in}),
    \label{equ:tensor}
\end{equation}
    where $\odot$ denotes Hadamard product, and $f_a,f_b,f_c$ denote convolution operators.
The only intermediate states we need to save here are $f_a(X_{in})$,$f_b(X_{in})$,$f_a(X_{in})\odot f_b(X_{in})$, and $f_c(X_{in})$, all of which have volume HWC, and therefore 4HWC intermediate states.

This $4\times$ intermediate state can be further optimized during the training stage, in the back-propagation, when updating the $l$-th layer's weights, the gradient of the weight $W_a^l$ can be computed by
\begin{equation}
    \frac{\partial \mathscr{L}}{\partial W_a^l} = \frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot \frac{\partial X^{l+1}}{\partial (W_a^lX^l)(W_b^lX^l)}\cdot \frac{\partial (W_a^lX^l)(W_b^lX^l)}{\partial (W_a^lX^l)} \cdot \frac{\partial (W_a^lX^l)}{\partial W_a^l},
    \label{equ:garident}
\end{equation}
where $X^l$ denotes the output tensor of layer $l$. We can observe that, in Eq.~(\ref{equ:garident}), the second term equals to one, and the third and forth terms can be obtained immediately from the front-propagation stage.
Therefore, the gradient of $W_a^l$ can be greatly simplified as
\begin{equation}
    \frac{\partial \mathscr{L}}{\partial W_a^l} = \frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot (W_b^lX^l)\cdot X^l.
\end{equation}
That means, the back-propagation of the quadratic term does not rely on intermediate state $f_a(X_{in})\odot f_b(X_{in})$. Also, the back-propagation of the linear term does not rely on intermediate state $f_c(X_{in})$. Therefore, we can implement back-propagation without saving these intermediate states, which further compress the intermediate states to $2\times$.

Quadratic convolutions also offer the possibility of external acceleration by simply mapping quadratic neuron to the convolution operator, allowing us to directly leverage existing compilers~\cite{chen2018tvm} and quadratic computation library~\cite{xu2022quadralib} to optimize the computation.
}


\sout{\textbf{Data Dependency Optimization:}
%\textbf{Improve Hardware Friendliness:}
%\textbf{Improve Hardware Friendliness by Mapping Quadratic Neuron to Optimized Operators:}
Considering the computation at the tensor level, the memory consumption and data dependency issue can be naturally solved.
    Because we don't introduce a recursive design, quadratic convolution has \textbf{no strong data dependency} as \textit{g$^r$Conv}.
    At a tensor computation level, quadratic operations can leverage convolution operators that have been widely optimized on various computing platforms \cite{chen2018tvm}.
    %Going to tensor computation level, 
    Given the input tensor $X_{in}$, the output of quadratic convolution can therefore be computed with:}
\end{comment}
\begin{comment}
\begin{equation}
    X_{out} = f_a(X_{in})\odot f_b(X_{in})+f_c(X_{in}),
\end{equation}
\end{comment}
\begin{comment}
\sout{
    where $\odot$ denotes Hadamard product, and $f_a,f_b,f_c$ denote convolution operators. Since the Hadamard product takes an element-wise product, its intermediate state space is limited to $O(n)$, which significantly \textbf{reduces the memory consumption}. More importantly, for implementation, we can directly use hardware-optimized convolution operators in a well-optimized computation library to further accelerate the computation.
}
\textbf{Intermediate State Reduction:}
The factorization does not only optimize the computation complexity, but also provides an opportunity to boost the computation efficiency of quadratic neurons during the training stage. In the back-propagation, when updating the $l$-th layer's weights, the gradient of the weight $W_a^l$ can be computed by
\begin{equation}
    \frac{\partial \mathscr{L}}{\partial W_a^l} = \frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot \frac{\partial X^{l+1}}{\partial (W_a^lX^l)(W_b^lX^l)}\cdot \frac{\partial (W_a^lX^l)(W_b^lX^l)}{\partial (W_a^lX^l)} \cdot \frac{\partial (W_a^lX^l)}{\partial W_a^l},
    \label{equ:garident}
\end{equation}
where $X^l$ denotes the output tensor of layer $l$. In the training stage, without any optimization, all of the above intermediate states need to be stored in the memory. However, we can observe that, in Eq.~(\ref{equ:garident}), the second term equals to one, and the third and forth terms can be obtained immediately from the front-propagation stage. Therefore, the gradient of $W_a^l$ can be greatly simplified as
\begin{equation}
    \frac{\partial \mathscr{L}}{\partial W_a^l} = \frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot (W_b^lX^l)\cdot X^l.
\end{equation}
In other words, only $W_a^lX^l$ and $W_b^lX^l$ will be the extra intermediate states that we need to save for the back-propagation. When compared with conventional neural networks, we only generate 2$\times$ intermediate states (versus  ($HW$+3)$\times$ in self-attention). Therefore, we can optimize memory usage and accelerate the computation of gradients by skipping some intermediate states in training.
\end{comment}


==> _hist/3-2-Method_Part1_v1.tex <==
\subsection{\textbf{Efficient Quadratic Neuron and Convolution}}
\textbf{Efficient Quadratic Neuron:}
We first solve the neuron design challenge by an efficient quadratic neuron.
As defined in Equation \ref{equ:quadratic_neuron}, the quadratic term of a conventional quadratic neuron has a $n\times n$ complexity in the parameter space, which limits its usage in terms of both algorithm complexity and implementation difficulty. 
%To avoid huge computing workload and memory cost of conventional quadratic neuron, as illustrated in Figure \ref{fig:QuadraNet} (a), in stead of using a full rank quadratic weight matrix $W_q$, we build weight matrix with two n-dimensional vectors $W_a, W_b \in \mathbb{R}^{1\times n}$, which can been seen as a low rank factorization of the quadratic term weight matrix.
To address such an issue, in stead of using a full rank quadratic weight matrix $W_q$ as shown in Figure \ref{fig:QuadraNet} (a), we propose to build the weight matrix with two n-dimensional vectors $W_a$ and  $W_b \in \mathbb{R}^{1\times n}$, which can been seen as a low rank factorization of the quadratic term weight matrix.
Then the new quadratic neuron can be reformulated as
\begin{equation}
    \mathbf{y} = \mathbf{x}^TW_a^TW_b\mathbf{x} + W_c\mathbf{x} + b\\
    =(W_a\mathbf{x})^T(W_b\mathbf{x}) + W_c\mathbf{x} + b.
\end{equation}
Such a factorization reduces the parameter space of quadratic neuron from $O(n^2+n)$ to $O(3n)$ and number of Multiply Accumulate (MAC) operations from $O(n^2+2n)$ to $O(4n)$. 

\textbf{Build High-order Interaction with Quadratic Convolution:} 
In order to build high-order spatial interaction in a vision task, we map quadratic to convolution. Since we propose a neuron-level high-order interaction computation, it will be easy to map the quadratic neuron to any neural operations (i.e. convolution and FC). Because of useful inductive bias (e.g. translation equivalence) of convolution neural networks, we map the quadratic neuron to a convolution operations. 
With quadratic convolution, high-order spatial interaction can be captured easily. Consider a mostly used depthwise separable convolution, the computation of $i$-th position of channel $c$ can be formulated as:
\begin{equation}
\begin{aligned}
     y_{Quad}^{(i,c)} &=\sum_{j,k \in \Omega_i} \sum_{c'=1}^C(\omega_{a,i\rightarrow j}W_{a}^{(c,c')}x^{(j,c')})(\omega_{b,i\rightarrow k}W_{b}^{(c,c')}x^{(k,c')})\\
     &=\sum_{j \in \Omega_i}\sum_{c'=1}^C\omega_{a,i\rightarrow j}\sum_{k \in \Omega_i}\omega_{b,i\rightarrow k}x^{(k,c')}W_{q}^{(c,c')}x^{(j,c')}\\
     &=\sum_{j \in \Omega_i}\sum_{c'=1}^Cq(x)_{ij}W_{q}^{(c,c')}x^{(j,c')},
     \end{aligned}
     \label{equ:q_conv}
\end{equation}
where $\Omega_i$ denotes the convolution receptive field in $i$-th position, and $q(x)_{ij}=\omega_{a,i\rightarrow j}\sum_{k \in \Omega_i}\omega_{b,i\rightarrow k}x^{(k,c')}$ implicates an input-adaptive weight and when multiply $x$, it captures the high-order spatial interaction. Notice that Equation \ref{equ:q_conv} forms an unified formula expression of high-order interaction with Equation \ref{equ:highorder}, which indicates quadratic convolution capture the high-order spatial interaction and therefore can be seen as an approximation computation of self-attention and g$^n$Conv. 

%\textbf{Improve Hardware Friendliness:}
\textbf{Improve Hardware Friendliness by Optimized Operators:}
%\textbf{Improve Hardware Friendliness by Mapping Quadratic Neuron to Optimized Operators:}
When we consider the computation of the tensor level, the memory consumption and data dependency issue can be naturally solved.
    Because we don't introduce a recursive design, quadratic convolution has \textbf{no strong data dependency} as g$^n$Conv.    
    In a tensor computation level, quadratic can leverage convolution operators that have been widely optimized on various computing platforms \cite{chen2018tvm}. 
    Going to tensor computation level, given the input tensor $X_{in}$, the output of quadratic convolution can therefore be computed with:
\begin{equation}
    X_{out} = f_a(X_{in})\odot f_b(X_{in})+f_c(X_{in}),
\end{equation}
    where $\odot$ denotes Hadamard product, and $f_a,f_b,f_c$ denote convolution operators. Since the Hadamard product takes an element-wise product, it intermediate state space is limited to $O(n)$, which significantly \textbf{reduces the memory consumption}. Also, when implementing, we can directly use hardware-optimized convolution operators in computation library to further accelerate the computation.
    
\textbf{Training Stage Memory Optimization:}
The factorization does not only optimize the computation complexity, but also provide a opportunity to boost the computation efficiency of quadratic neuron during training stage. In the back-propagation, when updating the $l$-th layer's weights, the gradient of the weight $W_a^l$ can be computed with:
\begin{equation}
    \frac{\partial \mathscr{L}}{\partial W_a^l} = \frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot \frac{\partial X^{l+1}}{\partial (W_a^lX^l)(W_b^lX^l)}\cdot \frac{\partial (W_a^lX^l)(W_b^lX^l)}{\partial (W_a^lX^l)} \cdot \frac{\partial (W_a^lX^l)}{\partial W_a^l},
    \label{equ:garident}
\end{equation}
where $X^l$ denotes the output tensor of layer $l$. In the training stage, without any optimization, all of above intermediate states are needed to be stored in the memory. We can observe in Equation \ref{equ:garident}, the second term equals one and the third and forth term can be obtained immediately in the front-propagation stage, therefore the gradient of $W_a^l$ can be computed with: 
\begin{equation}
    \frac{\partial \mathscr{L}}{\partial W_a^l} = \frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot (W_b^lX^l)\cdot X^l.
\end{equation}
That means, only $W_a^lX^l$ and $W_b^lX^l$ will be the extra intermediate states we need to save for back-propagation compared with conventional neural networks, we only generates $2\times$ intermediate states compared with $(HW+3) \times$ in self-attention. Therefore, we can optimize the memory usage and accelerate the computation of gradient by skip some intermediate state in training.

==> _hist/3-2-Method_Part1_v2-XC.tex <==
\subsection{\textbf{Efficient Quadratic Neuron and Convolution Design}}

\textbf{Quadratic Neuron:}
As defined in Eq.~(\ref{equ:quadratic_neuron}), the quadratic term of a conventional quadratic neuron has a $n^2$ complexity in the parameter space, which limits its usage in terms of both algorithmic implementation difficulty.
	To address this issue, instead of using a full-rank quadratic weight matrix $W_q$, we propose to build the weight vectors $W_a$ and $W_b \in \mathbb{R}^{1\times n}$ as shown in Fig.~\ref{fig:QuadraNet} (a), which can be seen as a low-rank factorization of the quadratic term.
	Thus, the new quadratic neuron can be reformulated as:
\begin{equation}
	\mathbf{y} = \mathbf{x}^TW_a^TW_b\mathbf{x} + W_c\mathbf{x} + b\\
	=(W_a\mathbf{x})^T(W_b\mathbf{x}) + W_c\mathbf{x} + b.
	\label{equ:our_neuron}
\end{equation}

Such a factorization reduces the parameter space of quadratic neurons from $O$($n^2$+$n$) to $O(3n)$ and the computation complexity from $O$($n^2$+2$n$) to $O$(4$n$).

\begin{comment}
	% We first solve the neuron design challenge by an efficient quadratic neuron.
	%To avoid huge computing workload and memory cost of conventional quadratic neuron, as illustrated in Fig.~\ref{fig:QuadraNet} (a), in stead of using a full rank quadratic weight matrix $W_q$, we build weight matrix with two n-dimensional vectors $W_a, W_b \in \mathbb{R}^{1\times n}$, which can been seen as a low rank factorization of the quadratic term weight matrix.
\end{comment}




\textbf{High-Order Interactive Quadratic Convolution:}
Because quadratic neurons have powerful cognitive capacity and generalization ability, we can directly bring them into a simple way of information extraction.
	In this work, we directly project optimized quadratic neurons to the widely-used convolution operation to achieve efficient high-order interactions.
	Specifically, we map the three groups of weights $W_a$, $W_b$, and $W_c$ from a single quadratic neuron to three convolutional filters and conduct a polynomial computation like in Eq.~(\ref{equ:our_neuron}). With such a mapping, we obtain a quadratic convolution.
	Considering a mostly used depthwise separable convolution, the quadratic computation of $i^{th}$ position of channel $c$ is formulated as:
\begin{equation}
	\begin{aligned}
		y_{Quad}^{(i,c)} &=\sum_{j,k \in \Omega_i} \sum_{c'=1}^C(\omega_{a,i\rightarrow j}T_{a}^{(c,c')}x^{(j,c')})(\omega_{b,i\rightarrow k}T_{b}^{(c,c')}x^{(k,c')})\\
		&=\sum_{j \in \Omega_i}\sum_{c'=1}^C\omega_{a,i\rightarrow j}\sum_{k \in \Omega_i}\omega_{b,i\rightarrow k}x^{(k,c')}T_{q}^{(c,c')}x^{(j,c')}\\
		&=\sum_{j \in \Omega_i}\sum_{c'=1}^Cq(x)_{ij}T_{q}^{(c,c')}x^{(j,c')},
	\end{aligned}
	\label{equ:q_conv}
\end{equation}
where $\Omega_i$ denotes the convolution receptive field in the $i^{th}$ position, and $q(x)_{ij}=\omega_{a,i\rightarrow j}\sum_{k \in \Omega_i}\omega_{b,i\rightarrow k}x^{(k,c')}$ implicates an input-adaptive weight.
When multiplying $x$, it captures the high-order spatial interaction.
	Notice that Eq.~(\ref{equ:q_conv}) forms a unified  expression for high-order interaction that well matches with Eq.~(\ref{equ:highorder}).
	This indicates that the quadratic convolution can capture high-order spatial interactions, and therefore can be seen as an approximation computation of self-attention and \textit{g$^r$Conv}.

\begin{comment}
	% \CX{\sout{Convolutional neural networks have efficient computation flow and generalization ability, and convolution operators are also fully optimized on various devices. Combining convolution with quadratic neurons can effectively use these characteristics to build efficient and powerful networks.}}
\end{comment}
\begin{comment}
	% \sout{The optimized quadratic neuron is further utilized to form high-order convolution operation.}
	% In order to build high-order spatial interaction in a vision task, we map quadratic to convolution.
	% Since we propose a neuron-level high-order interaction computation, it will be easy to map the quadratic neuron to any neural operations (i.e. convolution and FC).
	%Because of useful inductive bias (e.g., Translation equivalence) of convolution neural networks, we map the quadratic neuron to a convolution operations.
\end{comment}




\textbf{Efficient High-Order Computation:}
Through the neuron- and convolution-level design, the primary high-order quadratic computation mechanism could be determined.
	From a tensor perspective, the computing of this mechanism could be formulated as:
\begin{equation}
	X_{out} = f_a(X_{in})\odot f_b(X_{in})+f_c(X_{in}),
	\label{equ:tensor}
\end{equation}
where $\odot$ denotes the Hadamard product; $f_a,f_b,f_c$ denote convolution operators (with weights of $W_a$, $W_b$, $W_c$); $X_{in}$ and $X_{out}$ denote the input and output tensors, respectively.
	Different from~\cite{rao2022hornet}, such a mechanism goes through a straightforward computation flow without a recursive logic, and thus eliminating aforementioned data dependency and corresponding computing costs.

As for the problem of intermediate states, we need to examine the intermediate states generated in Eq.~(\ref{equ:tensor}).
	During forward propagation, four intermediate states are generated --- $f_a(X_{in})$,$f_b(X_{in})$,$f_a(X_{in})\odot f_b(X_{in})$, and $f_c(X_{in})$, all of which require the same data volume and 4$HWC$ intermediate state workload in total.
	The corresponding workload of intermediate states in quadratic convolution will therefore be $4\times$ compared with conventional convolution (i.e., $HWC$) for better cognition performance, but much smaller compared with the self-attention (i.e., ($HW$+3)$\times$) for less computing costs.

Meanwhile, during backpropagation, this $4\times$ intermediate states can be further reduced to $2\times$, since two intermediate states of $f_a(X_{in})\odot f_b(X_{in})$ and $f_c(X_{in})$ can be immediately released during computing before causing dominant workload.
	For the rest two states --- $f_a(X_{in})$ and $f_b(X_{in})$, weight updates of $W_a$ (or $W_b$) only rely on intermediate states $f_b(X_{in})$ (or $f_a(X_{in})$), because the gradient of the weight $W_a^l$ (or $W_b^l$) can be computed by:

\-\vspace{-3.5mm}
\begin{equation}
	\begin{aligned}
		\frac{\partial \mathscr{L}}{\partial W_a^l} = &\frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot \frac{\partial X^{l+1}}{\partial (W_a^lX^l)(W_b^lX^l)}\cdot \frac{\partial (W_a^lX^l)(W_b^lX^l)}{\partial (W_a^lX^l)} \cdot \frac{\partial (W_a^lX^l)}{\partial W_a^l}\\
		= &\frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot (W_b^lX^l)\cdot X^l,
	\end{aligned}
	\label{equ:garident}
\end{equation}
where $X^l$ denotes the $l^{th}$ layer output.
	Similarly, the update of the weight $W_b$ only rely on intermediate states $f_a(X_{in})$. The update of the linear term weight $W_c$ does not rely on any intermediate states.
	Therefore, only two intermediate states --- $f_a(X_{in})$ and $f_b(X_{in})$ are actually counted for memory and computing costs.

In a word, quadratic convolution enables more efficient higher-order computation by avoiding a recursive design for less data dependencies and further optimizations for intermediate states.
	Quadratic convolution also offers the possibility of external acceleration by simply mapping quadratic neurons to the convolution operators, allowing us to directly leverage existing compilers~\cite{chen2018tvm} and quadratic computation library~\cite{xu2022quadralib} to optimize the computation.

\begin{comment}
	%are 4 generated intermediate states to complete the forward computation, all of which have volume HWC, and totally 4HWC intermediate states.
		%What we further optimize lies in the fact that, considering back-propagation, this $4\times$ intermediate state can be further reduced during the training stage.
		%When updating the $l^{th}$ layer's weights, the gradient of the weight $W_a^l$ can be computed by
		%\begin{equation}
			%\begin{aligned}
				%\frac{\partial \mathscr{L}}{\partial W_a^l} = &\frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot \frac{\partial X^{l+1}}{\partial (W_a^lX^l)(W_b^lX^l)}\cdot \frac{\partial (W_a^lX^l)(W_b^lX^l)}{\partial (W_a^lX^l)} \cdot \frac{\partial (W_a^lX^l)}{\partial W_a^l}\\
				%= &\frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot (W_b^lX^l)\cdot X^l,
			%\end{aligned}
			%\label{equ:garident}
		%\end{equation}
	%where $X^l$ denotes the output tensor of the $l^{th}$ layer.
	%That means the backpropagation of the quadratic term does not rely on intermediate state $f_a(X_{in})\odot f_b(X_{in})$.
	%Also, the back-propagation of the linear term does not rely on intermediate state $f_c(X_{in})$.
	%Therefore, we can implement back-propagation without saving these intermediate states, which further compress the intermediate states to $2\times$.
	%In a word, quadratic convolution enables more efficient higher-order computation by avoiding a recursive design that eliminates strong data dependencies and further optimizations for intermediate states.
	%Quadratic convolution also offers the possibility of external acceleration by simply mapping quadratic neuron to the convolution operator, allowing us to directly leverage existing compilers~\cite{chen2018tvm} and quadratic computation library~\cite{xu2022quadralib} to optimize the computation.

%Through the neuron and convolution level design, the basic high-order computation mechanism could be determined.
	% From a tensor perspective, the computing could be xxxxx as Eq. 7
	%Different from HorNet, this is a xxxxx 计算流程，没有recursive。

% For the two main aforementioned high-order computation problems, the strong data dependency is solved naturally because there is no recursive design in the quadratic convolution.
	% As for the problem of intermediate states, if we put the view on the whole tensor computation flow level, the size of the intermediate state of the quadratic convolution operation will be $4\times$ compared with conventional neural networks (versus  ($HW$+3)$\times$ in self-attention).
	% To be specific, given the input tensor $X_{in}$, the output of quadratic convolution can therefore be computed with:
% \begin{equation}
	% X_{out} = f_a(X_{in})\odot f_b(X_{in})+f_c(X_{in}),
	% \label{equ:tensor}
% \end{equation}
	% where $\odot$ denotes Hadamard product, and $f_a,f_b,f_c$ denote convolution operators.
% The only intermediate states we need to save here are $f_a(X_{in})$,$f_b(X_{in})$,$f_a(X_{in})\odot f_b(X_{in})$, and $f_c(X_{in})$, all of which have volume HWC, and therefore 4HWC intermediate states.

% This $4\times$ intermediate state can be further optimized during the training stage, in the back-propagation, when updating the $l$-th layer's weights, the gradient of the weight $W_a^l$ can be computed by
	% \begin{equation}
		% \frac{\partial \mathscr{L}}{\partial W_a^l} = \frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot \frac{\partial X^{l+1}}{\partial (W_a^lX^l)(W_b^lX^l)}\cdot \frac{\partial (W_a^lX^l)(W_b^lX^l)}{\partial (W_a^lX^l)} \cdot \frac{\partial (W_a^lX^l)}{\partial W_a^l},
		% \label{equ:garident}
	% \end{equation}
% where $X^l$ denotes the output tensor of layer $l$. We can observe that, in Eq.~(\ref{equ:garident}), the second term equals to one, and the third and forth terms can be obtained immediately from the front-propagation stage.
% Therefore, the gradient of $W_a^l$ can be greatly simplified as
% \begin{equation}
	% \frac{\partial \mathscr{L}}{\partial W_a^l} = \frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot (W_b^lX^l)\cdot X^l.
% \end{equation}
% That means, the back-propagation of the quadratic term does not rely on intermediate state $f_a(X_{in})\odot f_b(X_{in})$. Also, the back-propagation of the linear term does not rely on intermediate state $f_c(X_{in})$. Therefore, we can implement back-propagation without saving these intermediate states, which further compress the intermediate states to $2\times$.

% Quadratic convolutions also offer the possibility of external acceleration by simply mapping quadratic neuron to the convolution operator, allowing us to directly leverage existing compilers~\cite{chen2018tvm} and quadratic computation library~\cite{xu2022quadralib} to optimize the computation.
% }

% \sout{\textbf{Data Dependency Optimization:}
%\textbf{Improve Hardware Friendliness:}
%\textbf{Improve Hardware Friendliness by Mapping Quadratic Neuron to Optimized Operators:}
% Considering the computation at the tensor level, the memory consumption and data dependency issue can be naturally solved.
	% Because we don't introduce a recursive design, quadratic convolution has \textbf{no strong data dependency} as \textit{g$^r$Conv}.
	% At a tensor computation level, quadratic operations can leverage convolution operators that have been widely optimized on various computing platforms \cite{chen2018tvm}.
	%Going to tensor computation level,
	% Given the input tensor $X_{in}$, the output of quadratic convolution can therefore be computed with:}
\end{comment}
\begin{comment}
	%\begin{equation}
		%X_{out} = f_a(X_{in})\odot f_b(X_{in})+f_c(X_{in}),
	%\end{equation}
\end{comment}
\begin{comment}
	%\sout{where $\odot$ denotes Hadamard product, and $f_a,f_b,f_c$ denote convolution operators. Since the Hadamard product takes an element-wise product, its intermediate state space is limited to $O(n)$, which significantly \textbf{reduces the memory consumption}.
	%More importantly, for implementation, we can directly use hardware-optimized convolution operators in a well-optimized computation library to further accelerate the computation.}
\end{comment}
\begin{comment}
	%\textbf{Intermediate State Reduction:}
		%The factorization does not only optimize the computation complexity, but also provides an opportunity to boost the computation efficiency of quadratic neurons during the training stage. In the back-propagation, when updating the $l$-th layer's weights, the gradient of the weight $W_a^l$ can be computed by
		%\begin{equation}
			%\frac{\partial \mathscr{L}}{\partial W_a^l} = \frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot \frac{\partial X^{l+1}}{\partial (W_a^lX^l)(W_b^lX^l)}\cdot \frac{\partial (W_a^lX^l)(W_b^lX^l)}{\partial (W_a^lX^l)} \cdot \frac{\partial (W_a^lX^l)}{\partial W_a^l},
			%\label{equ:garident}
		%\end{equation}
	% where $X^l$ denotes the output tensor of layer $l$. In the training stage, without any optimization, all of the above intermediate states need to be stored in the memory. However, we can observe that, in Eq.~(\ref{equ:garident}), the second term equals to one, and the third and forth terms can be obtained immediately from the front-propagation stage. Therefore, the gradient of $W_a^l$ can be greatly simplified as
		%\begin{equation}
			%\frac{\partial \mathscr{L}}{\partial W_a^l} = \frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot (W_b^lX^l)\cdot X^l.
		%\end{equation}
	% In other words, only $W_a^lX^l$ and $W_b^lX^l$ will be the extra intermediate states that we need to save for the back-propagation.
	% When compared with conventional neural networks, we only generate 2$\times$ intermediate states (versus  ($HW$+3)$\times$ in self-attention).
	% Therefore, we can optimize memory usage and accelerate the computation of gradients by skipping some intermediate states in training.
\end{comment}


==> _hist/3-3-Method_Part2_v2.tex <==

\CX{
\subsection{\textbf{Efficient and Powerful \textit{QuadraBlock}}}
\textbf{\textit{QuadraBlock} Design:} Our QuadraBlock design is as shown in Fig.~\ref{fig:QuadraNet} (c). 
It is divided to a spatial feature mixing layer and a inter-channel information mixing layer. 
The spatial feature mixing layer is composed of a layer normalization and a quadratic depth-wise convolution, while the inter-channel information mixing layer is composed of a layer normalization, a 1$\times$1 convolution with channel expansion coefficient $R$, a GELU activation and another 1$\times$1 convolution.

\textbf{Efficiency of \textit{QuadraBlock}:} \textit{QuadraBlock} achieves high efficiency by using only quadratic convolutions in spatial information mixing.
Because in the modern CNNs design, the spatial feature mixing layers take less than 5\% of the parameters and MACs while performing important texture, outline and shape depicting. 
Therefore, inserting the secondary convolutions into the spatial information mixture has little effect on the overall number of parameters and computation.

\textbf{Improve Quadratic Neuron with \textit{QuadraBlock}:} The advantage of this design is not only that it adds a very small amount of parameters and computation, but also that the information transfer and activation operation between channels provides an approximate calculation of more group weights. 
        The quadratic term of the combination of quadratic neuron layers, $1\times 1$ convolution with expansion coefficient $R$ and activation function $\sigma(\cdot)$ can be formulated as:
\begin{equation}
    y_{term}^c=\sum_{c'=1}^{RC}\sigma(T_{q}^{(c,c')}\mathbf{x}^TW_a^TW_b\mathbf{x}).
    \label{equ:rank}
\end{equation}
Consider the non-linearity of activation function, Eq.~(\ref{equ:rank}) can be approximated as:
\begin{equation}
    y_{comb}^c\approx \sum_{c'=1}^{C}T_{q}^{(c,c')}\mathbf{x}^T(\sum_{r=1}^{R}W_{ar}^TW_{br})\mathbf{x},
    \label{equ:rank1}
\end{equation}
where $(\sum_{r=1}^{R}W_{ar}^TW_{br}) = W_a^TW_b, W_a,W_b \in \mathbb{R}^{n*R}$. 

        Therefore, the block design brings the representation capacity of quadratic weight matrix $W_q$ with $rank = 1$ to the same level as a $rank = R$ matrix, where $R$ denotes the channel expansion coefficient in the first $1\times 1$ convolution layers.

\subsection{\textbf{Pyramid Multi-Stage \textit{QuadraNet}}}
Figure~\ref{fig:QuadraNet}~(d) illustrates the macro design of \textit{QuadraNet}. 
We follow full-fledged four-stage pyramid architecture as \cite{liu2021swin,liu2022convnet}. 
At the beginning of each stage, STEM~\cite{liu2022convnet} is first utilized for downsampling while increasing the number of channels. 
Then the \textit{QuadraBlock} is repeated for $n_i$ times in stage$_i$.

Receptive field:

We take a $7 \times 7$ quadratic depth-wise convolution to obtain a large high-order interactive receptive field. 

Number of blocks:

To fairly compare it with the baselines~\cite{liu2021swin,liu2022convnet,rao2022hornet}, we set the number of blocks as [3,3,27,3] and [2,3,18,2] in each stage in all of the models and set the number of channels as [C,2C,4C,8C] following common practice, with C = 64, 96, 128 for \textit{QuadraNet36/25-T/S/B}.

To explore the information superposition capability of quadratic neuron and \textit{QuadraBlock} in a different scale, we also design three families of narrow and shallow \textit{QuadraNet36/24/12-XXS/XS/T} with C = 16, 32, 64.


\subsection{\textbf{Hardware-aware Quadratic Neural Architecture Search}}
(1) Search Space: The proposal of \textit{QuadraNet} provides a new search space for the NAS.
When we lift the restrictions on the number of layers, channels and receptive field of \textit{QuadraNet}, we can obtain a natural search space for high-order interaction networks. 
In this work, following the original ProxylessNAS~\cite{cai2018proxylessnas}, we allow a candidate set of QuadraBlock with different kernel sizes \{3, 5, 7\} and expansion coefficients \{2, 4\}. 
We also add an identity block which does nothing but provides a residual connection to the candidate set to search for a shallow network.

(2)Hardware Constraint: Just like in the previous section we analyzed the hardware friendliness of \textit{QuadraNet}, using quadratic neurons can relatively alleviate the hardware constraints encountered in building high-order interactive NAS models. Because different devices have different hardware architectures, resulting in different degrees of computational constraints. Some devices have limited memory resources, others are IO sensitive, and still others have a very limited number of process units.

(3)Search Method: In this work, we directly employ hardware-aware ProxylessNAS \cite{cai2018proxylessnas} while modifying its search space to find a best suited \textit{QuadraNet} for different devices. Specificly, we train a supernet in defined \textit{QuadraNet} Search Space and use gradient based search strategy, we also add hardware latency estimation to loss function to search hardware-aware \textit{QuadraNet} models.
}










\TD{\subsection{\textbf{High-Performance Quadratic Neural Networks}}
\textbf{Improve Efficiency and Representation Capacity with QuadraBlock:}

\textbf{1)Efficient High-order Spatial Interaction:}}
%While quadratic neuron brings richer representation, it also brings more parameters.
    %Simply replacing the convolutional neural network with a quadratic neural version does not achieve the optimal solution in the trade-off between accuracy improvement and model-size increasement. 
    The neural block design philosophy of modern CNNs \cite{liu2022convnet}, and Transformers \cite{liu2021swin,dosovitskiy2020image} is to divide the block into spatial feature mixing layers (i.e., depth-wise convolution and self-attention) to depict texture, outline and shape information and inter-channel information mixing layers (i.e., feed-forward network(FFN) and $1\times 1$ convolution) to transport information among channels.
    IN the modern CNNs design \cite{liu2022convnet}, the spatial feature mixing layers take less than 5\% of the parameters and MACs while conducting the features spatial information mixing, and the resource-consuming inter-channel information mixing layers focus on the transportation of information across the different channels. 
%            \sout{Since we focus on the high-order spatial interaction}
            Since \cite{xu2022quadralib} shows that quadratic neurons are more conducive to the extraction of spatial features, we only takes quadratic depth-wise convolution with little increase at computation and parameters as a drop-in replacement of the spatial mixing layer in transformer block. 
 
\textbf{2)Improve Representation Capacity by approximating high-rank quadratic weight matrix:}
    As illustrated in Figure \ref{fig:QuadraNet}(c), the QuadraBlock contains a high-order spatial interaction layer with quadratic depth-wise convolution and an inter-channel fusion layer with conventional $1\times 1$ convolution. 
        The advantage of this design is not only that it adds a very small amount of parameters and computation, but also that the information transfer and activation operation between channels provides an approximate calculation of more group weights. 
        The quadratic term of the combination of quadratic neuron layers, $1\times 1$ convolution with expansion coefficient $R$ and activation function $\sigma(\cdot)$ can be formulated as:
\begin{equation}
    y_{term}^c=\sum_{c'=1}^{RC}\sigma(W_{q}^{(c,c')}\mathbf{x}^TW_a^TW_b\mathbf{x}).
    \label{equ:rank}
\end{equation}
Consider the non-linearity of activation function, Eq.~(\ref{equ:rank}) can be approximated as:
\begin{equation}
    y_{comb}^c\approx \sum_{c'=1}^{C}W_{q}^{(c,c')}\mathbf{x}^T(\sum_{r=1}^{R}W_{ar}^TW_{br})\mathbf{x},
    \label{equ:rank1}
\end{equation}
where $(\sum_{r=1}^{R}W_{ar}^TW_{br}) = W_a^TW_b, W_a,W_b \in \mathbb{R}^{n*R}$. 
\begin{comment}
\begin{equation}
\begin{aligned}
    y^{(i,c)} & = \sum_{j,k \in \Omega_i} \sum_{c'=1}^{RC}\sigma(W_{q}^{(c,c')}(\omega_{a,i\rightarrow j}x^{(j,c')})(\omega_{b,i\rightarrow k}x^{(k,c')})) \\
    & = \sum_{j,k \in \Omega_i}\sum_{c'=1}^{C}\sum_{r=1}^{R}\sigma(W_{q}^{(c,c')}(\omega_{a,i\rightarrow j}x^{(j,c')})(\omega_{b,i\rightarrow k}x^{(k,c')}))
\end{aligned}
\end{equation}
\end{comment}
        Therefore, the block design brings the representation capacity of quadratic weight matrix $W_q$ with $rank = 1$ to the same level as a $rank = R$ matrix, where $R$ denotes the channel expansion coefficient in the first $1\times 1$ convolution layers.
 
\textbf{Pyramid Multi-Stage \textit{QuadraNet}:}
When constructing models, we follow full-fledged four-stage pyramid architecture as \cite{liu2021swin,liu2022convnet} for \textit{QuadraNet}'s macroscopical architecture to pursue state-of-the-art performance.
We also take a $7 \times 7$ quadratic depth-wise convolution to obtain a large high-order interactive receptive field. 
To fairly compare it with the baselines \cite{liu2021swin,liu2022convnet,rao2022hornet}, we set the number of blocks as [3,3,27,3] and [2,3,18,2] in each stage in all of the models and set the number of channels as [C,2C,4C,8C] following common practice, with C = 64, 96, 128 for \textit{QuadraNet36/25-T/S/B}.
To explore the information superposition capability of quadratic neuron and QuadraBlock in a different scale, we also design two families of narrow and shallow \textit{QuadraNet36/12-XXS/XS/T} with C = 16, 32, 64.



\textbf{Hardware-aware Quadratic Neural Architecture Search:}
Although with competitive cognition performance to the state-of-the-art model, manually designed \textit{QuadraNet} might achieve sub-optimal performance and latency trade-off because of the heterogeneity of devices.
    The introduction of QuadraBlock provides a new search space for the NAS. % neural architecture search.
        In this work, we directly employ hardware-aware ProxylessNAS \cite{cai2018proxylessnas} while modifying its search space to find  a best suited \textit{QuadraNet} for different devices. 

\textbf{1) \textit{QuadraNet} Search Space:}
We use \textit{QuadraNet} as the backbone to build the architecture search space. 
Following the original ProxylessNAS~\cite{cai2018proxylessnas}, we allow a candidate set of QuadraBlock with different kernel sizes \{3, 5, 7\} and expansion coefficients\{2, 4\}. 
We also add an identity block which does nothing but provides a residual connection to the candidate set to search for a shallow network.




==> _hist/3-3-Method_Part2_v3-XC-CX.tex <==
\subsection{\textbf{Efficient and Powerful \textit{QuadraBlock}}}

\textbf{\textit{QuadraBlock} Design:}
Our QuadraBlock design is as shown in Fig.~\ref{fig:QuadraNet} (c).
	It is divided into a spatial feature mixing layer and an inter-channel information mixing layer:
	the spatial feature mixing layer is composed of a layer normalization operator and a quadratic depth-wise convolution;
	the inter-channel information mixing layer comprises a layer normalization operator, a 1$\times$1 convolution operator with a channel expansion coefficient $R$, a GELU activation, and another 1$\times$1 convolution operator.

Such a design achieves high computing efficiency by using only quadratic convolutions in spatial information mixing.
	Because in the modern CNNs design, the spatial feature mixing layers take less than 5\% of the parameters and MACs while performing important texture, outline, and shape depicting~\cite{liu2022convnet}.
	Therefore, inserting the quadratic convolutions into the spatial information mixture has little effect on the overall number of parameters and computation.



\textbf{\textit{QuadraBlock} for Cognition Capacity:}
    \textit{QuadraBlock} also unifies multiple quadratic neurons using channle-wise information transportation and activation. It enhances the cognition ability of quadratic neurons by approximating a high-rank quadratic weight matrix within the \textit{QuadraBlock}.
    This enhancement approximation is achieved by leveraging the nonlinear activation function to construct a linearly independent quadratic term weights matrix as in Eq.~(\ref{equ:rank}).
	The quadratic term of the combination of quadratic neuron layers, 1$\times$1 convolution with expansion coefficient $R$ and activation function $\sigma(\cdot)$ can be formulated as follows:
	\begin{equation}
	\begin{aligned}
        y_{comb}^c&=\sum_{c'=1}^{RC}\sigma(T_{q}^{(c,c')}\mathbf{x}^TW_a^TW_b\mathbf{x})\\
        &\approx \sum_{c'=1}^{C}T_{q}^{(c,c')}\mathbf{x}^T(\sum_{r=1}^{R}W_{ar}^TW_{br})\mathbf{x},
        \end{aligned}
		\label{equ:rank}
	\end{equation}
where $(\sum_{r=1}^{R}W_{ar}^TW_{br}) = W_A^TW_B, W_A,W_B \in \mathbb{R}^{n*R}$.

Thus, \textit{QuadraBlock} enhances the representation capacity of quadratic weight matrix $W_q$ with $rank$=1 to a similar level as a $rank$=$R$, retaining both low-rank efficiency and cognition capability.
    %where $R$ denotes the channel expansion coefficient in the first 1$\times$1 convolution layers.

\begin{comment}
    Furthermore, consider the non-linearity of activation function, Eq.~(\ref{equ:rank}) can be approximated as:
	\begin{equation}
		y_{comb}^c\approx \sum_{c'=1}^{C}T_{q}^{(c,c')}\mathbf{x}^T(\sum_{r=1}^{R}W_{ar}^TW_{br})\mathbf{x},
		\label{equ:rank1}
	\end{equation}
\end{comment}
\begin{comment}
    % \sout{The advantage of this design is not only that it adds a very small amount of parameters and computation, but also that the information transfer and activation operation between channels provides an approximate calculation of more group weights.}
\end{comment}





\subsection{\textbf{\textit{QuadraNet} Architecture Design:}}
Figure~\ref{fig:QuadraNet}~(d) illustrates the macro design of \textit{QuadraNet}.
We follow full-fledged four-stage pyramid architecture as \cite{liu2021swin,liu2022convnet}. Pyramid architecture contains 4-stage with a increasing channels and decreasing resolution design.
In each stage, STEM~\cite{liu2022convnet} is first utilized for downsampling while increasing the number of channels.
Then the \textit{QuadraBlock} is repeated for $n_i$ times in stage i.


\newpage
\textbf{Receptive field:} We set the receptive field w.r.t convolution kernel size to $7 \times 7$ for quadratic depth-wise convolution. 
A large receptive field helps to capture high-order spatial interactions.

\textbf{Number of Channels:}
In each stage, we set the number of channels to [C, 2C, 4C, 8C] in each stage following common practice, where C denotes the basic number of channels.
We set the basic number of channels as C=[16, 32, 64, 96, 128] to construct  \textit{QuadraNet}L-XXS/XS/T/S/B model. 

\textbf{Number of Layers:}
To fairly compare it with the baselines~\cite{liu2021swin,liu2022convnet,rao2022hornet}, we set the number of blocks as [3,3,27,3] and [2,3,18,2] in each stage to construct \textit{QuadraNet}36/25-C.

%\textbf{Number of \textit{QuadraBlocks}:}
%To fairly compare it with the baselines~\cite{liu2021swin,liu2022convnet,rao2022hornet}, we set the number of blocks as [3,3,27,3] and [2,3,18,2] in each stage in all of the models and set the number of channels as [C,2C,4C,8C] following common practice, with C = 64, 96, 128 for \textit{QuadraNet36/25-T/S/B}.

%To explore the information superposition capacity of quadratic neuron and \textit{QuadraBlock} in a different scale, we also design three families of narrow and shallow \textit{QuadraNet36/24/12-XXS/XS/T} with C = 16, 32, 64.




\subsection{\textbf{Hardware-Aware Quadratic Neural Architecture Search}}
We further incorporate state-of-the-art NAS techniques to enhance \textit{QuadraNet}'s architecture generability and hardware adaptability.

\textbf{Search Space:}
Following a common NAS development approach, \textit{QuadraNet} first requires a new parameter search space.
	\TD{When we lift the restrictions on the number of layers, channels, and receptive field of \textit{QuadraNet}, we can obtain a natural search space for high-order interaction networks.}
	\CX{When we lift the restrictions on hyperparameters of manual designed \textit{QuadraNet}, we can therefore obtain an unique high-order interactive search space}
	In this work, following the original ProxylessNAS~\cite{cai2018proxylessnas}, we specify a candidate set of \textit{QuadraBlock} with different kernel sizes \{3, 5, 7\} and expansion coefficients \{2, 4\}.
	We also add an identity block which does nothing but provides a residual connection to the candidate set to search for a shallow network.

\textbf{Hardware Awareness:}
As demonstrated in previous sections, we have  analyzed the \textit{QuadraNet}'s memory and computing costs, as well as optimization factors.
	Given different systems' hardware profiling regarding different neural network operations, we can project different \textit{QuadraNet} model designs into particular resource consumption estimations.
	Therefore, the hardware-aware search feedback can be well established in the NAS process.
	% And hardware friendliness of \textit{QuadraNet}, using quadratic neurons can relatively alleviate the hardware constraints encountered in building high-order interactive NAS models.
	% Because different devices have different hardware architectures, resulting in different degrees of computational constraints. Some devices have limited memory resources, others are IO sensitive, and still others have a very limited number of process units.

\textbf{Search Method:}
Leveraging these efforts, we directly modify ProxylessNAS~\cite{cai2018proxylessnas} into a \textit{QuadraNet}-specified NAS framework.
	\TD{Specificly, we train a supernet in defined \textit{QuadraNet} Search Space and use a gradient based search strategy. We also add hardware latency estimation to the loss function to search for hardware-aware \textit{QuadraNet} models.}
	\CX{Firstly, we train a supernet in defined \textit{QuadraNet} Search Space. Then with a gradient based search strategy, considering hardware latency as a part of loss function, we train the branch weights to search appropriate architecture for target devices.}


==> _hist/3-3-Method_Part2_v3-XC.tex <==
\subsection{\textbf{Efficient and Powerful \textit{QuadraBlock}}}

\textbf{\textit{QuadraBlock} Design:}
Our QuadraBlock design is as shown in Fig.~\ref{fig:QuadraNet} (c).
	It is divided into a spatial feature mixing layer and an inter-channel information mixing layer:
	the spatial feature mixing layer is composed of a layer normalization operator and a quadratic depth-wise convolution;
	the inter-channel information mixing layer is composed of a layer normalization operator, a 1$\times$1 convolution operator with channel expansion coefficient $R$, a GELU activation, and another 1$\times$1 convolution operator.

%\textbf{Efficiency of \textit{QuadraBlock}:} \textit{QuadraBlock} 
Such a design approach achieves high efficiency by using only quadratic convolutions in spatial information mixing.
	Because in the modern CNNs design, the spatial feature mixing layers take less than 5\% of the parameters and MACs while performing important texture, outline, and shape depicting.
Therefore, inserting the secondary convolutions into the spatial information mixture has little effect on the overall number of parameters and computation.


\textbf{Improve Quadratic Neuron with \textit{QuadraBlock}:} The advantage of this design is not only that it adds a very small amount of parameters and computation, but also that the information transfer and activation operation between channels provides an approximate calculation of more group weights.
	The quadratic term of the combination of quadratic neuron layers, $1\times 1$ convolution with expansion coefficient $R$ and activation function $\sigma(\cdot)$ can be formulated as follows:
	\begin{equation}
		y_{term}^c=\sum_{c'=1}^{RC}\sigma(T_{q}^{(c,c')}\mathbf{x}^TW_a^TW_b\mathbf{x}).
		\label{equ:rank}
	\end{equation}
Consider the non-linearity of activation function, Eq.~(\ref{equ:rank}) can be approximated as:
	\begin{equation}
		y_{comb}^c\approx \sum_{c'=1}^{C}T_{q}^{(c,c')}\mathbf{x}^T(\sum_{r=1}^{R}W_{ar}^TW_{br})\mathbf{x},
		\label{equ:rank1}
	\end{equation}
where $(\sum_{r=1}^{R}W_{ar}^TW_{br}) = W_a^TW_b, W_a,W_b \in \mathbb{R}^{n*R}$.

Therefore, the block design brings the representation capacity of quadratic weight matrix $W_q$ with $rank = 1$ to the same level as a $rank = R$ matrix, where $R$ denotes the channel expansion coefficient in the first $1\times 1$ convolution layers.



\subsection{\textbf{Pyramid Multi-Stage \textit{QuadraNet}}}
Figure~\ref{fig:QuadraNet}~(d) illustrates the macro design of \textit{QuadraNet}.
We follow full-fledged four-stage pyramid architecture as \cite{liu2021swin,liu2022convnet}.
At the beginning of each stage, STEM~\cite{liu2022convnet} is first utilized for downsampling while increasing the number of channels.
Then the \textit{QuadraBlock} is repeated for $n_i$ times in stage$_i$.

Receptive field:

We take a $7 \times 7$ quadratic depth-wise convolution to obtain a large high-order interactive receptive field.

Number of blocks:

To fairly compare it with the baselines~\cite{liu2021swin,liu2022convnet,rao2022hornet}, we set the number of blocks as [3,3,27,3] and [2,3,18,2] in each stage in all of the models and set the number of channels as [C,2C,4C,8C] following common practice, with C = 64, 96, 128 for \textit{QuadraNet36/25-T/S/B}.

To explore the information superposition capability of quadratic neuron and \textit{QuadraBlock} in a different scale, we also design three families of narrow and shallow \textit{QuadraNet36/24/12-XXS/XS/T} with C = 16, 32, 64.



\subsection{\textbf{Hardware-Aware Quadratic Neural Architecture Search}}
(1) Search Space: The proposal of \textit{QuadraNet} provides a new search space for the NAS.
When we lift the restrictions on the number of layers, channels and receptive field of \textit{QuadraNet}, we can obtain a natural search space for high-order interaction networks.
In this work, following the original ProxylessNAS~\cite{cai2018proxylessnas}, we allow a candidate set of QuadraBlock with different kernel sizes \{3, 5, 7\} and expansion coefficients \{2, 4\}.
We also add an identity block which does nothing but provides a residual connection to the candidate set to search for a shallow network.

(2)Hardware Constraint: Just like in the previous section we analyzed the hardware friendliness of \textit{QuadraNet}, using quadratic neurons can relatively alleviate the hardware constraints encountered in building high-order interactive NAS models. Because different devices have different hardware architectures, resulting in different degrees of computational constraints. Some devices have limited memory resources, others are IO sensitive, and still others have a very limited number of process units.

(3)Search Method: In this work, we directly employ hardware-aware ProxylessNAS \cite{cai2018proxylessnas} while modifying its search space to find a best suited \textit{QuadraNet} for different devices. Specificly, we train a supernet in defined \textit{QuadraNet} Search Space and use gradient based search strategy, we also add hardware latency estimation to loss function to search hardware-aware \textit{QuadraNet} models.


==> _hist/3-3-Method_Part2_v4-XC.tex <==
\subsection{\textbf{Efficient and Powerful \textit{QuadraBlock}}}

\textbf{\textit{QuadraBlock} Design:}
Our QuadraBlock design is as shown in Fig.~\ref{fig:QuadraNet} (c).
	It is divided into a spatial feature mixing layer and an inter-channel information mixing layer:
	the spatial feature mixing layer is composed of a layer normalization operator and a quadratic depth-wise convolution;
	the inter-channel information mixing layer comprises a layer normalization operator, a 1$\times$1 convolution operator with a channel expansion coefficient $R$, a GELU activation, and another 1$\times$1 convolution operator.

Such a design achieves high computing efficiency by using only quadratic convolutions in spatial information mixing.
	Because in the modern CNNs design, the spatial feature mixing layers take less than 5\% of the parameters and MACs while performing important texture, outline, and shape depicting~\cite{liu2022convnet}.
	Therefore, inserting the quadratic convolutions into the spatial information mixture has little effect on the overall number of parameters and computation.



\textbf{\textit{QuadraBlock} for Cognition Capacity:}
    \textit{QuadraBlock} also unifies multiple quadratic neurons using channle-wise information transportation and activation. It enhances the cognition ability of quadratic neurons by approximating a high-rank quadratic weight matrix within the \textit{QuadraBlock}.
    This enhancement approximation is achieved by leveraging the nonlinear activation function to construct a linearly independent quadratic term weights matrix as in Eq.~(\ref{equ:rank}).
	The quadratic term of the combination of quadratic neuron layers, 1$\times$1 convolution with expansion coefficient $R$ and activation function $\sigma(\cdot)$ can be formulated as follows:
	\begin{equation}
	\begin{aligned}
        y_{comb}^c&=\sum_{c'=1}^{RC}\sigma(T_{q}^{(c,c')}\mathbf{x}^TW_a^TW_b\mathbf{x})\\
        &\approx \sum_{c'=1}^{C}T_{q}^{(c,c')}\mathbf{x}^T(\sum_{r=1}^{R}W_{ar}^TW_{br})\mathbf{x},
        \end{aligned}
		\label{equ:rank}
	\end{equation}
where $(\sum_{r=1}^{R}W_{ar}^TW_{br}) = W_A^TW_B, W_A,W_B \in \mathbb{R}^{n*R}$.

Thus, \textit{QuadraBlock} enhances the representation capacity of quadratic weight matrix $W_q$ with $rank$=1 to a similar level as a $rank$=$R$, retaining both low-rank efficiency and cognition capability.
    %where $R$ denotes the channel expansion coefficient in the first 1$\times$1 convolution layers.

\begin{comment}
    Furthermore, consider the non-linearity of activation function, Eq.~(\ref{equ:rank}) can be approximated as:
	\begin{equation}
		y_{comb}^c\approx \sum_{c'=1}^{C}T_{q}^{(c,c')}\mathbf{x}^T(\sum_{r=1}^{R}W_{ar}^TW_{br})\mathbf{x},
		\label{equ:rank1}
	\end{equation}
\end{comment}
\begin{comment}
    % \sout{The advantage of this design is not only that it adds a very small amount of parameters and computation, but also that the information transfer and activation operation between channels provides an approximate calculation of more group weights.}
\end{comment}





\subsection{\textbf{\textit{QuadraNet} Architecture Design:}}
Figure~\ref{fig:QuadraNet}~(d) illustrates the macro design of \textit{QuadraNet}.
We follow full-fledged four-stage pyramid architecture as \cite{liu2021swin,liu2022convnet}. which contains 4-stage with increasing channels and decreasing resolutions.
    In each stage, STEM~\cite{liu2022convnet} is first utilized for downsampling while increasing the number of channels, then the \textit{QuadraBlock} is repeated for $n_i$ times in stage i.
    And following configurations will be considered:


\input{_tab/acc_through}

\textbf{Receptive field:}
We set the receptive field regarding convolution kernel size to 7$\times$7 for a quadratic depth-wise convolution. 
    A large receptive field helps to capture high-order spatial interactions.

\textbf{Number of Channels:}
In each stage, we set the number of channels to [C, 2C, 4C, 8C] in each stage following common practice, specifically, C=[16, 32, 64, 96, 128] to construct  \textit{QuadraNet}~L-XXS/XS/T/S/B models (for different layers and scales). 

\textbf{Number of Layers:}
To fairly compare it with baselines~\cite{liu2021swin,liu2022convnet,rao2022hornet}, we can set the number of blocks as [3,3,27,3] and [2,3,18,2] in each stage to construct \textit{QuadraNet}~36/25-C with similar model volumes.

%\textbf{Number of \textit{QuadraBlocks}:}
%To fairly compare it with the baselines~\cite{liu2021swin,liu2022convnet,rao2022hornet}, we set the number of blocks as [3,3,27,3] and [2,3,18,2] in each stage in all of the models and set the number of channels as [C,2C,4C,8C] following common practice, with C = 64, 96, 128 for \textit{QuadraNet36/25-T/S/B}.

%To explore the information superposition capacity of quadratic neuron and \textit{QuadraBlock} in a different scale, we also design three families of narrow and shallow \textit{QuadraNet36/24/12-XXS/XS/T} with C = 16, 32, 64.




\subsection{\textbf{Hardware-Aware Quadratic Neural Architecture Search}}
We further incorporate state-of-the-art NAS techniques to enhance \textit{QuadraNet}'s architecture generability and hardware adaptability.

\textbf{Search Space:}
Following a common NAS development approach, \textit{QuadraNet} first requires a new parameter search space.
	When we generalize the above configuration options into automation search, we can therefore obtain a unique high-order interactive search space.
	Following the original ProxylessNAS~\cite{cai2018proxylessnas}, we specify a candidate set of \textit{QuadraBlock} with different kernel sizes \{3, 5, 7\} and expansion coefficients \{2, 4\}.
	We also add an identity block that does nothing but provides a residual connection to the candidate set to search for a shallow network.

\textbf{Hardware Awareness:}
As demonstrated in previous sections, we have  analyzed the \textit{QuadraNet}'s memory and computing costs, as well as optimization factors.
	Given different systems' hardware profiling regarding different neural network operations, we can project different \textit{QuadraNet} model designs into particular resource consumption estimations.
	Therefore, the hardware-aware search feedback can be well established in the NAS process.
	% And hardware friendliness of \textit{QuadraNet}, using quadratic neurons can relatively alleviate the hardware constraints encountered in building high-order interactive NAS models.
	% Because different devices have different hardware architectures, resulting in different degrees of computational constraints. Some devices have limited memory resources, others are IO sensitive, and still others have a very limited number of process units.

\textbf{Search Method:}
Leveraging these efforts, we directly modify ProxylessNAS~\cite{cai2018proxylessnas} into a \textit{QuadraNet}-specified NAS framework.
	Specifically, we train a supernet in defined \textit{QuadraNet} Search Space and use a gradient-based search strategy. We also add hardware latency estimation to the loss function to search for hardware-aware \textit{QuadraNet} models.
	Firstly, we train a supernet in defined \textit{QuadraNet} Search Space. Then with a gradient-based search strategy, considering hardware latency as a part of the loss function.
    And eventually, we train the branch weights to search for an appropriate architecture for the target device with particular hardware constraints.

==> _hist/3-Method_v1.tex <==
\section{\textbf{Method}}
\subsection{\textbf{Overview}}
\begin{figure*}
    \centerline{\includegraphics[width = 7 in]{fig/QuadraNet.pdf}}
    \caption{A bottom-up overview of QuadraNet, from neuron-level to system implementation-level.}
    \label{fig:QuadraNet}
\end{figure*}
Figure \ref{fig:QuadraNet} illustrates the overview of our proposed model.     From a bottom-up perspective, it is composed of five components: (a) efficient low rank quadratic neuron, (b) mapping quadratic neuron to convolution, (c) Quadratic Neural Block Design, (d) QuadraNet architecture, (e) Hardware-aware quadratic neural architecture search. 
    To be specific: 
        (a) provides a factorization of quadratic term weights, reduce the computation complexity and parameters space of quadratic term.
        In (b) quadratic convolution, (a) quadratic neurons are mapped to hardware-optimized convolution operators. 
        Using optimized (b) high-order quadratic convolution, a powerful (c) Quadratic network block is built to leverage the (a) quadratic neuron's high-order information superposition. 
        Using similar pyramid macroscopical network architecture and (c) QuadraBlock, QuadraNet achieves competitive  performance while solving the computation bottleneck of high-order interactive neural networks. 
        To make hardware specific optimization, (d) QuadraNet defines a search space for (e) HW-NAS.
    In the following section, we will introduce these components in detail.
    
    
\subsection{\textbf{Efficient Quadratic Neuron \& Quadratic Convolution}}
\textbf{Efficient Low Rank Quadratic Neuron:}
As defined in Equation \ref{equ:quadratic_neuron}, the quadratic term of a conventional quadratic neuron is with a $n\times n$ parameter space, which limits the usage of quadratic neuron from both algorithm complexity and implementation difficulty perspective. 
    To avoid huge computing workload and memory cost of conventional quadratic neuron,as illustrated in Figure \ref{fig:QuadraNet} (a), in stead of using a full rank quadratic weight matrix $W_q$, we build weight matrix with two n-dimensional vectors $W_a, W_b \in \mathbb{R}^{1\times n}$, which can been seen as a low rank factorization of the quadratic term weight matrix.
    Then the quadratic neuron can be written in the format:
\begin{equation}
    y = \mathbf{x}^TW_a^TW_b\mathbf{x} + W_c\mathbf{x} + b\\
    =(W_a\mathbf{x})^T(W_b\mathbf{x}) + W_c\mathbf{x} + b
\end{equation}

The factorization reduces the parameter space of quadratic neuron from $O(n^2+n)$ to $O(3n)$ and number of Multiply Accumulates (MACs) from $O(n^2+2n)$ to $O(4n)$. 

%\textbf{Improve Hardware Friendliness:}
\textbf{Improve Hardware Friendliness by Optimized Operators:}
%\textbf{Improve Hardware Friendliness by Mapping Quadratic Neuron to Optimized Operators:}
    Since we propose a neuron-level high-order interaction computation, it will be easy to map the quadratic neuron to convolution (or any other neural operations).
        To leverage convolution operators that have been widely optimized on various computing platforms \cite{chen2018tvm} and useful inductive bias (e.g. translation equivalence) of convolution neural networks, we map the quadratic neuron to a convolution operations. 
    To map single quadratic neuron to a tensor computation level, given the input tensor $X_{in}$, the output of quadratic convolution can therefore be computed with:
\begin{equation}
    X_{out} = f_a(X_{in})\odot f_b(X_{in})+f_c(X_{in}),
\end{equation}
    where $\odot$ denotes Hadamard product, and $f_a,f_b,f_c$ denote convolution operators. Thus, when implementing a quadratic convolution, we can directly use hardware-optimized convolution operators in computation library to accelerate the computation. Also, the Hadamard product takes an element-wise product, it intermediate state space is limited to $O(n)$, which significantly reduce the memory consumption.
    
\textbf{Build High-order Spatial Interaction with Quadratic Convolution:}  
With quadratic convolution, high-order spatial interaction can be captured easily. Consider a mostly used depthwise separable convolution, the computation of $i$-th position of channel $c$ can be formulated as:
\begin{equation}
\begin{aligned}
     x_{Quad}^{(i,c)} &=\sum_{j,k \in \Omega_i} \sum_{c'=1}^C(\omega_{a,i\rightarrow j}W_{a}^{(c,c')}x^{(j,c')})(\omega_{b,i\rightarrow k}W_{b}^{(c,c')}x^{(k,c')})\\
     &=\sum_{j \in \Omega_i}\sum_{c'=1}^C\omega_{a,i\rightarrow j}\sum_{k \in \Omega_i}\omega_{b,i\rightarrow k}x^{(k,c')}W_{q}^{(c,c')}x^{(j,c')}\\
     &=\sum_{j \in \Omega_i}\sum_{c'=1}^Cq(x)_{ij}W_{q}^{(c,c')}x^{(j,c')},
     \end{aligned}
     \label{equ:q_conv}
\end{equation}
where $\Omega_i$ denotes the convolution receptive field in $i$-th position, and $q(x)_{ij}=\omega_{a,i\rightarrow j}\sum_{k \in \Omega_i}\omega_{b,i\rightarrow k}x^{(k,c')}$ implicates an input-adaptive weight and when multiply $x$, it captures the high-order spatial interaction between a feature $x_i$ and its neighbor $x_j,j \in \Omega_i$. Notice that Equation \ref{equ:q_conv} forms an unified formula expression of high-order interaction with Equation \ref{equ:self} and \ref{equ:gnconv}, which indicates quadratic convolution can been seen as an approximation computation of self-attention and g$^n$Conv. 

\textbf{Training Stage Memory Optimization:}
The factorization does not only optimize the computation complexity, but also provide a opportunity to boost the computation efficiency of quadratic neuron during training stage. In the back-propagation, when updating the $l$-th layer's weights, the gradient of the weight $W_a^l$ can be computed with:
\begin{equation}
    \frac{\partial \mathscr{L}}{\partial W_a^l} = \frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot \frac{\partial X^{l+1}}{\partial (W_a^lX^l)(W_b^lX^l)}\cdot \frac{\partial (W_a^lX^l)(W_b^lX^l)}{\partial (W_a^lX^l)} \cdot \frac{\partial (W_a^lX^l)}{\partial W_a^l},
    \label{equ:garident}
\end{equation}
where $X^l$ denotes the output tensor of layer $l$. In the training stage, without any optimization, all of above intermediate states are needed to be stored in the memory. We can observe in Equation \ref{equ:garident}, the second term equals one and the third and forth term can be obtained immediately in the front-propagation stage, therefore the gradient of $W_a^l$ can be computed with: 
\begin{equation}
    \frac{\partial \mathscr{L}}{\partial W_a^l} = \frac{\partial \mathscr{L}}{\partial X^{l+1}}\cdot (W_b^lX^l)\cdot X^l
\end{equation}
That means, we can optimize the memory usage and accelerate the computation of gradient by skip some intermediate state in training.


\subsection{\textbf{Build Powerful and Efficient High-Order Neural Interaction with QuadraBlock}}
%\subsection{\textbf{Improve Representation Capacity with QuadraBlock}}
\subsubsection{principle}
\subsubsection{formulation}
\subsubsection{trade-off?}

%While quadratic neuron brings richer representation, it also brings more parameters.
    %Simply replacing the convolutional neural network with a quadratic neural version does not achieve the optimal solution in the trade-off between accuracy improvement and model-size increasement. 
    Modern CNNs \cite{liu2022convnet} and Transformers \cite{liu2021swin,dosovitskiy2020image} divide network block design into spatial feature mixing layers (i.e. depth-wise convolution and self-attention) and inter-channel information mixing layers (i.e. feed-forward network(FFN) and $1\times 1$ convolution). 
    IN the modern CNNs design \cite{liu2022convnet}, the spatial feature mixing layers take less than 5\% of the parameters and MACs while finishing the features spatial information mixing and the resource-consuming inter-channel information mixing layers focus on the transportation of information across different channel. 
        In vision tasks, spatial interaction helps to depict texture, outline and shape. 
            Since we focus on the high-order spatial interaction, we only takes quadratic depth-wise convolution with little increasement at computation and parameters as a drop-in replacement of the spatial mixing layer in transformer block. 
    
    As illustrated in Figure \ref{fig:QuadraNet}(c) the QuadraBlock contains a high-order spatial interaction layer with quadratic depth-wise convolution and an inter-channel fusion layer with conventional $1\times 1$ convolution. 
        The advantage of this design is not only that it adds a very small amount of parameters and computation, but also that the information transfer and activation operation between channels provides an approximate calculation of more group weights. 
        Therefore, the block design brings the representation capacity of quadratic weight matrix with $rank=1$ to the same level as a $rank = r$ matrix, where $r$ denotes the channel expansion coefficient in the first $1\times 1$ convolution layers.
 
\subsection{Manual and Automatic QuadraNet Construction}
\subsubsection{Pyramid Multi-Stage QuadraNet}
When constructing models, we follows full-fledged four-stage pyramid architecture as \cite{liu2021swin,liu2022convnet} for QuadraNet's macroscopical architecture to pursue approximate to state-of-the-art performance.
We also takes a $7 \times 7$ quadratic depth-wise convolution to obtain a large high-order interactive receptive field. 
To fairly compare with baseline \cite{liu2021swin,liu2022convnet,rao2022hornet}, we set the number of blocks as [3,3,27,3] in each stage in all of the models and set the number of channels as [C,2C,4C,8C] following common practice, with C = 64,96,128 for QuadraNet36-T/S/B.
To explore the information superposition capability of quadratic neuron and QuadraBlock, we also design two families of narrow and shallow QuadraNet, with 25 and 12 total blocks and reduced channels.
We set the number of blocks as [2,3,18,2] and [2,2,6,2] in each stage and C = 16,32,64 for QuadraNet25/12-XXS/XS/T.

\subsubsection{Hardware-aware Quadratic Neural Architecture Search}


==> _hist/4-Experiment_v1.tex <==
\section{\textbf{Experiment}}

\input{_tab/acc_through}
We conduct experiments on ImageNet-1K image classification~\cite{deng2009imagenet} which contains 1.28M training images and 50K validation images from 1000 classes. 
    We report ImageNet-1K top-1 accuracy on the validation set. In the following, we first compare the proposed \textit{QuadraNet} with  state-of-the-art models in terms of cognition performance and computation.
\subsection{\textbf{Analyses of Manually Designed Models}}
\textbf{Settings:} We train \textit{QuadraNets} for 300 epochs (20 of which are warmup) with AdamW~\cite{loshchilov2018decoupled} optimizer and a learning rate of 4e-3. 
    We use a weight decay of 0.05 and the same data augmentations as in~\cite{rao2022hornet}. 
    The resolution of the input images is 224$\times$224. 
    To stabilize the training, we apply gradient clipping which limits the maximum value of gradient to 5 instead of the superabundant batch normalization as in~\cite{xu2022quadralib}, which will hurt the generalization ability of networks. 
    We use ``Channel Last'' memory layout following~\cite{liu2022convnet}.

Table~\ref{tab:acc} shows the comparison of \textit{QuadraNet} with other state-of-the-art models at comparable FLOPs and parameters.
    We observe that our models achieve competitive performance for both Transformers- and CNNs-based models. 
        We measure inference throughputs on an A100 GPU, and results show that, with a similar image classification accuracy, \textit{QuadraNets} achieve 1.35$\times$ to 1.57$\times$ higher inference throughputs than other baseline high-order interactive neural networks~\cite{liu2021swin,rao2022hornet}. 
Compared with ConvNeXt~\cite{liu2022convnet},
%(one-order state-of-the-art), 
\textit{QuadraNets} achieve higher cognitive performance due to its high-order neural interactions, but with 
higher throughputs most of the time. % relatively little slowdown.

\subsection{\textbf{Memory Footprint Analysis}}
\input{_tab/memory}
To analyze the memory usage of different models, we build a series of networks with a similar configuration except
the types of computation blocks.
%The number of blocks is set to [2, 2, 18, 2] in each stage and the batch size is set to 64. 
The batch size is set as 64 and 128, respectively.
The SkipBlock completely removes the spatial interaction and related residual connection, and the ConvBlock uses the same block design but only with the conventional depth-wise convolution. 

Table~\ref{tab:mem} shows that, under the same configuration, \textit{QuadraBlock} achieves high-order information interaction with a relatively smaller extra memory footprint than SwinBlock and HorBlock. 
When coupled with  QuadraLib~\cite{xu2022quadralib} that further optimizes the intermediate state, \textit{QuadraBlock} results in a even smaller memory footprint.
%\subsubsection{Layer Compression of Quadratic Neuron}
%Measure Layer Compression Ability Quadratic Neuron with shallow Network
\subsection{\textbf{Hardware-Aware Models Analysis}}
We conduct hardware-aware NAS with the help of nn-Meter~\cite{zhang2021nn}, which provides powerful latency estimation for different devices. We set the maximum latency for mobile CPU (CortexA76), VPU (Intel Myriad VPU), and GPU (A100) to 300ms, 30ms, and 3ms, respectively.
    With the help of ProxylessNAS~\cite{cai2018proxylessnas}, we compare its ordinary search space with \textit{QuadraNet}-defined search space, the results are shown in Tab.~\ref{tab:nas}. We observe that NAS can identify almost always better \textit{QuadraNets} models in the \textit{QuadraNet} defined search space in terms of  accuracy, FLOPs, and computation time. Fig~\ref{fig:Nas} gives an example of searched model with less than 10ms latency on VPU.
    
\begin{figure}[t]
    \centering
    \includegraphics{_fig/NAS_architecture_2.pdf}
    \caption{Visualization of Searched \textit{QuadraNet\_VPU\_10ms}}
    \label{fig:Nas}
\end{figure}

\input{_tab/NAS_result}


==> _hist/4-Experiment_v2-XC.tex <==
\section{\textbf{Experiment}}
As most state-of-the-art high-order interactive neural networks are designed for image classification, we also adopt the proposed \textit{QuadraNet} methodology in the same task.
	Specifically, we conduct experiments on ImageNet-1K dataset~\cite{deng2009imagenet}, which contains 1.28M training images and 50K validation images from 1000 classes.
	We report ImageNet-1K's Top-1 accuracy on the validation set.
	In the following, we compare the proposed \textit{QuadraNet} with state-of-the-art models regarding both cognition and computation performance.



\subsection{\textbf{\textit{QuadraNet} Evaluation with Manually Designed Models}}

\textbf{Model Initialization:}
We train \textit{QuadraNets} for 300 epochs (20 of which are warmup) with AdamW~\cite{loshchilov2018decoupled} optimizer and a learning rate of 4e-3.
	We use a weight decay of 0.05 and the same data augmentations as in~\cite{rao2022hornet}.
	The resolution of the input images is 224$\times$224.
	To stabilize the training, we apply gradient clipping that limits the maximum value of gradient to 5, instead of the superabundant batch normalization as in~\cite{xu2022quadralib}, which will hurt the generalization ability of networks.
	We use the ``Channel Last'' memory layout following~\cite{liu2022convnet}.


\textbf{Cognition Performance and Computing Costs:}
Table~\ref{tab:acc} evaluates the performance of several manually designed \textit{QuadraNet} models with other state-of-the-art models at comparable FLOPs and parameters.
	We observe that our models achieve competitive performance for both Transformers- and CNN-like models.
	With such a cognition performance baseline, we measure their inference throughputs on an A100 GPU\@.
	And results show that, with a similar image classification accuracy, \textit{QuadraNets} achieve 1.35$\times$ to 1.57$\times$ higher inference throughputs than high-order works~\cite{liu2021swin,rao2022hornet}.
Compared with ConvNeXt~\cite{liu2022convnet},
%(one-order state-of-the-art),
\textit{QuadraNets} achieve higher cognitive performance and even higher throughputs most of the time. % relatively little slowdown.


\textbf{Memory Consumption Analysis:}
\input{_tab/memory}
We further compare another set of models with a similar configuration except for different types of computation blocks to evaluate \textit{QuadraNet}'s memory consumption with 64 batch size, 24 layers, and 64/128 channels.
	Two non-high-order models are also involved in examining the trade-off between high-order performance and costs.
	To make a fair comparison, SkipBlock completely removes the spatial interaction and related residual connection, and ConvBlock uses the same block design but only with the conventional depth-wise convolution.

Table~\ref{tab:mem} shows that, under the same configuration, \textit{QuadraBlock} achieves high-order information interaction with a relatively smaller extra memory footprint than SwinBlock and HorBlock.
	When coupled with  QuadraLib~\cite{xu2022quadralib} that further optimizes the intermediate state, \textit{QuadraBlock} results in an even smaller memory footprint.
%\subsubsection{Layer Compression of Quadratic Neuron}
%Measure Layer Compression Ability Quadratic Neuron with shallow Network



\input{_tab/NAS_result}
\subsection{\textbf{Hardware-Aware QuadraNet Model Generalization}}
We conduct hardware-aware NAS with the help of nn-Meter~\cite{zhang2021nn} for its powerful latency estimation for different devices.
	We set the maximum latency for mobile CPU (CortexA76), VPU (Intel Myriad VPU), and GPU (A100) to 300ms, 30ms, and 3ms, respectively.
	Therefore, we compare the NAS models from regular ProxylessNAS~\cite{cai2018proxylessnas} and hardware-aware \textit{QuadraNet}.
	The results are shown in Table~\ref{tab:nas}.
	We observe that, given different hardware constraints, \textit{QuadraNet} models always perform better in terms of accuracy, FLOPs, and computation time.
	Fig~\ref{fig:Nas} also gives an example of a searched model with less than 10ms latency on VPU.

\begin{figure}[t]
	\centering
	\includegraphics{_fig/NAS_architecture_2.pdf}
	\caption{Visualization of Searched \textit{QuadraNet\_VPU\_10ms}}
	\label{fig:Nas}
\end{figure}


==> _hist/5-AblationStudy_v1.tex <==
\subsection{\textbf{Ablation Study}}
\textbf{Receptive Field:}
We explore the receptive field's influence on \textit{QuadraBlock}. As shown in Table~\ref{tab:receptive},
the large receptive fields indeed improves accuracy, but at the cost of significantly increased  training time because of the inflated computational scale. We observe that a kernel size of 7*7 seems to achieve a good trade-off balance between computation and performance.


\textbf{Cognitive capacity in different model volumes:}
Fig.~\ref{fig:my_label} shows that, with different number of channels and layers, the additional parameters introduced by quadratic neurons can be well reflected in the cognitive performance improvement, which further demonstrates the effectiveness of higher-order interactions.
\begin{figure}[t]
    \centering
    \includegraphics{_fig/FIg5.pdf}
    \caption{Outstanding Quadratic Performance w/ Various Configurations}
    \label{fig:my_label}
    \vspace{-4mm}
\end{figure}

\textbf{Channel-wise quadratic neurons:}

\input{_tab/receptive_field}
\input{_tab/FC}
Because of the generalization ability of quadratic neurons, we further study the effect of channel-wise higher-order interactions using quadratic neurons. As shown in Table~\ref{tab:fc}, we incrementally bring quadratic neurons into the channel-wise information transport layer, but the performance improvement is very limited while the amount of parameters and computation increase quickly.




==> _hist/5-AblationStudy_v2-XC.tex <==
\begin{figure}[b]
	\vspace{-5mm}
	\centering
	\includegraphics{_fig/FIg5.pdf}
	\caption{Outstanding Quadratic Performance w/ Various Configurations}
	\label{fig:my_label}
\end{figure}

\subsection{\textbf{Ablation Study}}
\textbf{Receptive Field:}
We explore the receptive field's influence on \textit{QuadraBlock}. As shown in Table~\ref{tab:receptive},
the large receptive fields indeed improves accuracy, but at the cost of significantly increased  training time because of the inflated computational scale. We observe that a kernel size of 7*7 seems to achieve a good trade-off balance between computation and performance.

\textbf{Cognitive capacity in different model volumes:}
Fig.~\ref{fig:my_label} shows that, with different number of channels and layers, the additional parameters introduced by quadratic neurons can be well reflected in the cognitive performance improvement, which further demonstrates the effectiveness of higher-order interactions.


\textbf{Channel-wise quadratic neurons:}
Because of the generalization ability of quadratic neurons, we further study the effect of channel-wise higher-order interactions using quadratic neurons. As shown in Table~\ref{tab:fc}, we incrementally bring quadratic neurons into the channel-wise information transport layer, but the performance improvement is very limited while the amount of parameters and computation increase quickly.


==> _hist/6-Conclusion_v1.tex <==
\section{Conclusion}

%We also notice that, in searched hybrid models, \textit{QuadraBlock} tends to appear in the final stage of the model. 

%A very interesting point is that, in contrast to GhostNet~\cite{han2020ghostnet} which generates more channels of feature maps with less filters, quadratic convolution essentially generates fewer channels of feature maps with more filters by means of higher-order interactions. Relation between the number of filters and the number of channels. The relationship between the number of filters and the number of channels, and what kind of interaction can exist between filters, will therefore be an open question. In this work, we gives a solution to embedding high-order interaction to quadratic neurons, but there are still many more ways of interaction waiting to be explored.

In this work, we have presented the \textit{QuadraNet} that performs efficient and powerful high-order interaction with quadratic neurons. 
    \textit{QuadraNet} avoids the computational problems of existing high-order interaction models by optimizing the intermediate states and eliminates strong data dependency in the computation process down to the neuron design level. Based on the design of efficient quadratic neurons, we construct a new family of generic backbone networks \textit{QuadraNets}, and provide a new search space for high-order interactions for hardware-aware NAS. Experiments demonstrate the superior cognitive capacity, high throughputs and low training memory footprints of the proposed \textit{QuadraNet}. Hardware-aware NAS further identifies better quadratic neural network architecture under this new  search space with quadratic neurons.
    
    % It combines hardware characteristics and uses the hardware friendliness of quadratic neurons to construct a hardware-aware network architecture search for quadratic neural networks

==> _hist/6-Conclusion_v2-XC.tex <==
\section{Conclusion}


In this work, we have presented \textit{QuadraNet} --- a revolutionary neural network design framework that incorporates efficient and powerful high-order neural interaction interactions.
	\textit{QuadraNet} solves the computational problems of existing high-order interaction models by optimizing the intermediate states and eliminating strong data dependency in the computation process down to the neuron design level.
	Based on the design of efficient quadratic neurons, we construct a new family of generic backbone \textit{QuadraNets} models and provide a new search space for high-order interactions for hardware-aware NAS.
	Experiments demonstrate the superior cognitive capacity, high throughputs, and low training memory footprints of the proposed \textit{QuadraNet}.
	Hardware-aware NAS further identifies better quadratic neural network architecture under this new  search space with quadratic neurons.
\input{_tab/receptive_field}
\input{_tab/FC}
